Astrophysics with the Laser Interferometer Space Antenna

The Laser Interferometer Space Antenna (LISA) will be a transformative experiment for gravitational wave astronomy, and, as such, it will offer unique opportunities to address many key astrophysical questions in a completely novel way. The synergy with ground-based and space-born instruments in the electromagnetic domain, by enabling multi-messenger observations, will add further to the discovery potential of LISA. The next decade is crucial to prepare the astrophysical community for LISA's first observations. This review outlines the extensive landscape of astrophysical theory, numerical simulations, and astronomical observations that are instrumental for modeling and interpreting the upcoming LISA datastream. To this aim, the current knowledge in three main source classes for LISA is reviewed; ultracompact stellar-mass binaries, massive black hole binaries, and extreme or intermediate mass ratio inspirals. The relevant astrophysical processes and the established modeling techniques are summarized. Likewise, open issues and gaps in our understanding of these sources are highlighted, along with an indication of how LISA could help making progress in the different areas. New research avenues that LISA itself, or its joint exploitation with upcoming studies in the electromagnetic domain, will enable, are also illustrated. Improvements in modeling and analysis approaches, such as the combination of numerical simulations and modern data science techniques, are discussed. This review is intended to be a starting point for using LISA as a new discovery tool for understanding our Universe.

==> astroWP_01ucb_BACKUP.tex <==
% Set page counter to 3 (no reset after the title pages)
\setcounter{page}{3}

\section{Stellar Compact Binaries and Multiples}

\textbf{Section coordinators: Silvia Toonen, Tassos Fragos, Thomas Kupfer, Thomas Tauris}%\\
 \newpage
%########Introduction and Summary
%###################################################
\subsection	{Introduction and Summary}
\noindent \contr{Silvia Toonen, Tassos Fragos, Thomas Kupfer, Thomas Tauris}\\
\input{ucb_s1_intro}

\newpage

%###################################################
\subsection	{Classes of LISA binaries}\label{subsec:classes-binaries} % 
\input{ucb_s2.1_VerificationSources}

\bigskip

\input{ucb_s2.2_DetachedBinaries}

\bigskip

\input{ucb_s2.3_InteractingBinaries}

\bigskip

\input{ucb_s2.4_OtherSources}

\subsection	{Formation of LISA binaries }\label{subsec:formation-binaries} 
\noindent \coord{Katie Breivik} 

\noindent \contr{Michela Mapelli (1.3.2-3), Simone Bavera, Katie Breivik, Martyna Chruslinska, Gijs Nelemans,  Pau Amaro Seoane (1.3.2), Manuel Arca Sedda (1.3.2-3), Thomas Tauris,  Silvia Toonen (1.3.2-3), Jeff Andrews, Tassos Fragos (1.3.1), Luca Graziani, Daryl Haggard (1.3.2), Melvyn B. Davies (1.3.2-3)}% \\
\input{ucb_S3_FormationOfSources}


\subsection	{Expected LISA observations: numbers and rates}\label{subsec:rates}
\noindent \coord{Abbas Askar,Simone Bavera}\\
\noindent \contr{Abbas Askar,  Quentin Baghi, Simone Bavera, Tassos Fragos, Valeriya Korol, Kyle Kremer,  Manuel Arca Sedda}\\

\input{ucb_s4_Rates}

\subsection	{Synergies}
\input{ucb_s6.1_EMSynergies}

\input{ucb_s6.2_GWSynergies}

\bigskip
\subsection	{Technical aspects} 
\input{ucb_s7_Technical}

\subsection	{Scientific objectives} 
\label{subsec:scientificQ}

\input{ucb_s5.1_InteractionPhysics}

\bigskip
\input{ucb_s5.2_GalacticProbes}



==> ucb_S3_FormationOfSources.tex <==

\vspace{1.0cm}
{\color{blue}In the following section, we discuss the formation of LISA binaries. For a review and broader description of the many physical aspects of stellar evolution and binary star interactions that are referred to below in the context of the formation of compact object binaries, we refer to the textbooks by, for example, \citet{slv94,2001icbs.book.....H,2006epbm.book.....E,10.1088/2514-3433/ac595f,TvdH23}.}

\subsubsection{Isolated binaries}\label{subsubsec:isolated-binaries}
The formation pathways of isolated binaries observable by LISA are marked with several phases of mass loss or exchange. In the following Section, we refer to the initially more massive star as the primary and the initially less massive star as the secondary. Stable mass transfer can occur either through wind mass loss/accretion or RLO. Wind mass loss is generally assumed to be non-conservative across all phases of stellar evolution, with mass accretion efficiency ranging from $\lesssim 10\%$ for the Bondi--Hoyle--Lyttleton mechanism and $20\text{--}50\%$ if the accretion is focused \citep{2017MNRAS.468.3408D}. In this case, the orbit widens as the mass lost from the system causes an increase of the remaining specific angular momentum. In practice, the dynamics are  complicated and dependent on physics related to the geometry and structure of the wind, tidal effects, orbital characteristics and in some cases magnetic fields and radiation transport, thus calling for three-dimensional, multi-physics, hydrodynamical simulations \citep[e.g.][]{2018A&A...618A..50S, 2019A&A...626A..68S}. 

RLO occurs when the donor star expands to the point that its radius exceeds the Roche radius \citep{1983ApJ...268..368E}. RLO mass transfer can proceed in a dynamically stable or unstable fashion, depending on the structure of the donor and accretor as well as their mass ratio. The stability of RLO mass transfer is commonly described using the Webbink radius--mass exponents \citep{1985ibs..book...39W} that determine the timescales on which mass transfer will become unstable. In the case of dynamically stable mass transfer, the orbital evolution depends strongly on the mass ratio of the binary: if $M_{\rm donor}/M_{\rm accretor} > 1$,  the orbit tightens (for fully conservative mass-transfer), while in the converse case the orbit widens. Mass-transfer efficiency, as well as the assumed specific angular momentum carried away from mass lost from the system, play a crucial role in mass-transfer stability and the orbital evolution of the binary.

Dynamically unstable mass transfer is believed to generate a CE phase where the donor star's core and companion are enshrouded in the donor's envelope \citep[for a review see][]{2013A&ARv..21...59I}. The precise dynamics of how CE proceeds are still not fully understood. In the context of compact object binary formation and population synthesis studies, energy budget arguments are most often employed to estimate the post-CE properties of a binary. In the ``$\alpha_{\rm CE}$'' prescription, it is assumed that a fraction $\alpha_{\rm CE}$ of the released orbital energy is used to unbind the donor's envelope and eject it from the system \citep{1976IAUS...73...35V, 1984ApJ...277..355W}. Several recent studies have suggested that other sources of energy may be needed to successfully eject the envelope, including recombination energy \citep[e.g.][]{2014A&A...568A..68Z, 2016MNRAS.460.3992N} or jets launched by the companion \citep[e.g.][]{2019MNRAS.488.5615S}. Each of these will change the overall energy budget of the CE evolution and lead to differences in the final orbital separation \citep[e.g.][]{2018MNRAS.477.2349I}. Alternatively, in the ``$\gamma_{\rm CE}$'' prescription, angular momentum conservation arguments, which lead to less dramatic inspiral, have been considered to explain the orbital period distribution of WD+WDs \citep{2000A&A...360.1011N}. 



\paragraph{WD+WD systems and AM~CVn binaries }\label{paragr:DWD-formation} 

\phantom{text}

\begin{figure*}
    \begin{center}
  \includegraphics[width=0.60\textwidth, angle=0]{./img_ucb/fig_LISA_WP_WDWD.png}
\caption{Illustration of the formation of an AM~CVn system and a detached WD+WD binary. LISA sources are indicated with waves. Acronyms. ZAMS: zero-age main sequence; RLO: Roche-lobe overflow (mass transfer); CE: common envelope; He star: helium star; WD: white dwarf; CV: cataclysmic variable; AM~CVn: AM Canum Venaticorum binary \citep[Figure from][]{TvdH23}.
}
 \label{fig:DWD}
  \end{center}
\end{figure*}

The progenitors of isolated WD+WD and AM~CVn binaries begin with zero age main sequence stars with masses below $8-10\,M_{\odot}$. The formation pathways of close WD+WD and AM~CVn binaries contain several stages of stable and unstable mass transfer, or CE (see Fig.\,\ref{fig:DWD}). The uncertain outcomes of these interactions determine whether the progenitor binary continues on in its evolutionary path toward becoming a LISA source or if it merges with its companion. Conversely, LISA observations of the populations of WD+WD and AM~CVn sources will constrain these interactions.

Virtually all close WD+WD and AM~CVn progenitors experience an interaction as the primary star advances off the main sequence and fills its Roche lobe. This interaction can either proceed stably or unstably on dynamical timescales. In either case, the orbit will shrink because of the donor's higher mass relative to the accretor. For systems with late red giant and asymptotic giant branch donors, initially dynamically stable but thermally unstable mass transfer can produce mass loss from the L2 Lagrange point, which leads to a delayed dynamical instability and a CE phase \citep{2020ApJS..249....9G, 2020A&A...642A.174M}. In the rare case of close WD+WDs where the more massive WD forms second (converse to stellar lifetime expectations), a phase of stable mass transfer, followed by a CE generated by the initially lower mass star could be necessary \citep{2012ApJ...744...12W}. 

After each interaction, the star which donates mass becomes stripped leaving behind a He core that can have varying structure depending on the evolutionary phase at which the donor filled its Roche lobe. Such stripped stars orbiting main sequence companions have been widely observed throughout the Galaxy \citep{2007MNRAS.382.1377R} and been used to constrain CE ejection efficiencies \citep{2010A&A...520A..86Z, 2013A&A...557A..87T}. 

Since the previous interaction brings the two stars together, further interactions are likely. Interactions can occur while the secondary is still on the main sequence. In this case, if the mass transfer is stable, a cataclysmic variable is formed \citep{2011A&A...536A..42Z}. Conversely, mass transfer can also occur as the secondary advances up the giant branch. Due to previous envelope stripping, the mass ratio of the secondary donor to the WD accretor can be either greater or less than one. If the secondary is already less massive than the WD, stable mass transfer will occur and widen the orbit, removing the possibility of detection by LISA. However, if the secondary is more massive than the WD companion, the mass exchange will lead to orbital tightening. If the mass transfer is unstable, another CE phase takes place, potentially bringing the stars even closer together and leaving behind a WD with a stripped He core companion. The structure of the He core again depends on the evolutionary phase at which the secondary overflows its Roche lobe. At this point, a close WD+WD binary is assured and the slow evolution due to GW  emission brings the WD+WD toward the LISA band.

A key uncertainty in the formation pathways of AM~CVn binaries is the nature of the donor star. AM~CVn binaries consist of a WD accreting He-rich material originating from a WD, semi-degenerate helium star, or evolved MS donor  \citep{2010PASP..122.1133S}. Indeed, it could be the case that the observed AM~CVn population is a combination of all three with different relative contributions \citep{2004MNRAS.349..181N}. 
If the donor star is a non-degenerate evolved star, magnetic braking is required, along with GW emission, to maintain the ultra-short periods of observed AM~CVn systems \citep{2005A&A...440..973V}. 
{\color{blue}Magnetic braking is a process in which orbital angular momentum in a tight synchronized binary is converted into spin angular momentum via a magnetic stellar wind (a process that therefore requires a low-mass stellar component with a convective envelope).}
The ultra-compact orbital configuration is less problematic for semi-degenerate and fully-degenerate donors which originate from the ejection of a second CE, with tighter orbits allowed by more degenerate donors \citep{2008AstL...34..620Y}. In the case of fully-degenerate He-core~WD donors, the orbit can become so small that the mass lost from the donor directly impacts the accretor leading to a rapid decrease in orbital size followed by a long-lived phase of accretion which widens the orbit \citep{2004MNRAS.349..181N,2004MNRAS.350..113M, 2006ApJ...649L..99D, 2017ApJ...846...95K}. Regardless of the donor, a significant uncertainty still remains in how much He-rich material the accretor can handle until novae erupt on the WD's surface. While detailed binary evolution calculations \citep[e.g.][]{2018PhRvL.121m1105T} have shown that RLO mass transfer in WD+WD can be stable, it has been suggested that interactions of the donor star with the expanding nova shells will likely lead to a rapid orbit shrinkage and eventually a merger \citep{2015ApJ...805L...6S}.




\paragraph{White-dwarf binaries with neutron-star or black-hole companions}

\phantom{text}


\begin{figure*}
    \begin{center}
  \includegraphics[width=0.60\textwidth, angle=0]{./img_ucb/fig_LISA_WP_UCXB.png}
\caption{Illustration of the formation of a detached NS+WD binary and an UCXB system. See Fig.~\ref{fig:DWD} for details. Additional acronyms: SN: supernova; NS: neutron star; LMXB: low-mass X-ray binary; BH: black hole \citep[Figure from][]{TvdH23}. }
 \label{fig:UCXB}
  \end{center}
\end{figure*}

\begin{figure*}
    \begin{center}
   \includegraphics[width=0.60\textwidth]{./img_ucb/Formation-UCXB-EM+GW_detection.png}
\caption{Evolutionary sequence showing how ultra-compact X-ray binaries (prime LISA source candidates) are formed from merging NS+WD binaries, descending from LMXBs. Plotted here is mass-transfer rate of the donor star as a function of stellar age. The initial MS star\,+\,NS binary has components of $1.40\;M_\odot$ and $1.30\;M_\odot$, respectively. The system evolves through two observable stages of mass transfer:
an LMXB for 4~Gyr, followed by a detached phase lasting about 3~Gyr where the system is detectable as a radio millisecond pulsar orbiting the helium WD remnant of the donor star, until GW radiation brings the system into contact again, producing a UCXB. The colour bars indicate detectability in different regimes resulting in synergies between LISA and EM detectors \citep[Figure from][]{2018PhRvL.121m1105T}.}
 \label{fig:LMXB-UCXB-link}
  \end{center}
\end{figure*}


Compared to WD+WDs, the formation of detached binaries with WD and NS or BH companions occur in binaries with stars that are massive enough to explode in a SN (see Fig.~\ref{fig:UCXB}). Similar to WD+WD formation, the more massive primary evolves first and, because of the relatively large mass ratio, begins RLO mass transfer that is  often expected to be unstable and lead to a CE. Soon after, the primary evolves to become a compact object, through either a supernova explosion (NS or BH) or  direct collapse (BH only). Since a NS is thought to receive a kick during its formation, there is a significant  probability that the binary disrupts at this point.

The subsequent evolution, of a lower-mass non-degenerate star with a NS or BH, will typically go through a phase of stable mass transfer in which the binary becomes observable as X-ray binary, due to the strong heating of the accretion disc in the deep potential of the NS or BH. When the onset of the mass-transfer occurs after the secondary star has evolved past its main sequence, the core of the star has already contracted. Thus after the X-ray binary phase, when the envelope of the expanding star has been completely transferred, the NS or BH is left with a WD companion that was the core of the donor star.

In some cases, the NS/BH+WD binary is tight enough that angular momentum loss due to GW emmission will bring the two objects together as LISA sources (Fig.~\ref{fig:LMXB-UCXB-link}). At periods of $\sim 10\text{--}20\;{\rm min}$, i.e. within the LISA band, the WD will start to transfer mass to the NS/BH, forming an X-ray binary again, but now of ultra-short period, called an UCXB. Detailed numerical calculations, including finite-temperature (entropy) effects, have shown that UCXBs can indeed form via stable RLO from post-LMXBs systems \citep{2017MNRAS.470L...6S,2018PhRvL.121m1105T}.




\paragraph{Double neutron star/black hole binaries } \label{subsec:1313}

\phantom{text}


\begin{figure*}
    \begin{center} \label{fig:1.9}
  \includegraphics[width=0.60\textwidth, angle=0]{./img_ucb/fig_LISA_WP_BHNS.png}
\caption{Illustration of the formation of a tight BH+NS binary that evolves towards a merger. See Figs.~\ref{fig:DWD} and \ref{fig:UCXB} for explanation of acronyms \citep[Figure from][]{TvdH23}.}
 \label{fig:BHNS}
  \end{center}
\end{figure*}


NS+NS formation has been extensively discussed in the literature \citep[see][for a review]{2017ApJ...846..170T}. The standard scenario (see Fig.~\ref{fig:BHNS} for a schematic diagram) involves several phases of interaction, starting with a stable RLO, during which the primary loses part of its envelope before it undergoes a SN to form a NS. The newly formed NS HMXB is likely too dim to be detectable in X-rays, as the orbital separation is still large and the NS may only be able to capture an appreciable fraction of the companion's stellar wind when the latter evolves to the giant phase. During the subsequent evolution the orbital separation needs to decrease from $\sim 10^3\;R_{\odot}$ to a few $R_\odot$ for the final binary to merge within the Hubble time.
Significant tightening is typically achieved through a CE phase that occurs when the secondary this time fills its Roche lobe. The post-CE binary is expected to encounter another phase of mass transfer, initiated by a {\color{blue}stripped helium-burning secondary \citep[i.e. so-called Case~BB mass transfer, often initiated when a $\sim 2.5-3.5\;M_\odot$ helium star expands during shell-helium burning,][]{1986A&A...165...95H}}. This leads to further orbital tightening, stripping of the secondary's envelope, and NS spin-up. If this last mass-transfer episode is unstable and leads to a second CE phase, a fast merging NS+NS will be formed; a scenario invoked to explain r-process
element enrichment observed in some stellar systems \citep{2019ApJ...872..105S,2019ApJ...886....4Z}.
Such NS+NSs would be  effectively unobservable with current radio surveys, and if they exist within the Galaxy, their presence will be revealed by LISA \citep{2019MNRAS.483.2615K,2020ApJ...892L...9A}. However, recent detailed binary evolution calculations have shown that this last phase of Case~BB mass transfer is expected to be stable \citep{2015MNRAS.451.2123T,2018MNRAS.481.4009V} and do not support the existence of the aforementioned fast-merging channel \citep[in contrast to earlier works][]{2003ApJ...592..475I,2003MNRAS.344..629D}.

Besides the pre-HMXB evolution, the most important and uncertain aspects of our current understanding of NS+NS and mixed BH+NS formation are related to: 
i) CE evolution and spiral-in of the NS, ii) momentum kicks (magnitude and direction) imparted onto newborn NSs, and iii) the mass distribution of NSs. 

From an energetics point of view, it has been shown that an inspiralling NS may indeed be able to eject the
envelope of its massive star companion \citep[e.g.][]{ 2010ApJ...716..114X,2011ApJ...743...49L, 2016RAA....16..126W,  2016A&A...596A..58K}. However, predicting the final post-CE
separation is difficult for several reasons, including: estimating the location of the bifurcation point  within the massive star \citep{2001A&A...369..170T}, separating the remaining core from the ejected envelope \citep{2001A&A...369..170T, 2019ApJ...883L..45F}, additional energy sources such as accretion energy \citep{2015ApJ...798L..19M, 2020ApJ...901L..24M}, energy and radiation transport during the CE inspiral \citep{2019ApJ...883L..45F} and the effect of an inflated envelope of the exposed naked helium core \citep[][see also Section~\ref{paragr:CE}]{2015A&A...580A..20S}.




Newly formed NSs gain velocity \citep[natal kicks; e.g.][] {1970ApJ...160..979G,2005MNRAS.360..974H,2017A&A...608A..57V} due to asymmetries arising during their formation  \citep[e.g.][]{2012ARNPS..62..407J}. The properties of the modelled NS+NS population (e.g. number of systems formed, orbital parameters, merger locations relative to formation site) are highly dependent on the adopted natal kick prescription  \cite[e.g.][]{1998A&A...332..173P,1999MNRAS.305..763B, 2018MNRAS.474.2937C,2018MNRAS.480.2011G,2019MNRAS.486.3213A}. To match the current observational constraints on the NS+NS merger rate and parameters of several of the observed systems \cite[e.g.][]{2007AIPC..924..598V}, it is necessary to assume that a fraction of NS forms with natal kicks smaller than typically found for young single pulsars. Some scenarios involve low-mass NS progenitors and electron-capture triggered explosions \cite[e.g.][]{2006ApJ...644.1063D,2013ApJ...772..150J}. Others postulate a link between the natal kick magnitude and the mass of the NS progenitor and SN ejecta  \citep[e.g.][]{2016MNRAS.456.4089B,2016MNRAS.461.3747B,2017ApJ...837...84J}. 
These claims have been supported by 3D NS simulations of ultra-stripped stars \citep{2019MNRAS.484.3307M}.
In fact, it has been demonstrated that close-orbit, low-eccentricity NS+NS and BH+NS systems most likely form via ultra-stripped SNe when the last star explodes \citep{2013ApJ...778L..23T,2015MNRAS.451.2123T}. The reason being that the last Case~BB RLO mass-transfer phase causes the NS to significantly strip its evolved helium-star companion, almost to a naked metal core prior to its explosion, and thus there is very little SN ejecta (see also Section~\ref{paragr:ccSNe}).

 

Finally, a clear correlation has been predicted between the spin period of the recycled pulsar and the orbital period of the system after the second SN \citep{2017ApJ...846..170T}. This correlation can be tested in LISA binaries, if the spin period is measured, since only short orbit systems will enter the LISA band within a Hubble time, and these binaries should therefore contain the most rapidly spinning NSs of this population. Another hypothesis that can be tested by LISA, is the resulting mass distribution among NS+NS systems \cite[e.g.][and references therein]{2016ARA&A..54..401O}. 




Merging BH+BHs and NS+BHs in the field are thought to occur under some specific binary interactions which either (i) bring the parent stars closer together during their evolution or (ii) prevent stars in close obits from expanding. 

The former one (i) occurs in a similar manner to the formation of NS+NSs described above, and involves many of the main uncertainties. In contrast to NS+NS formation, BH+BHs and to a lesser degree BH+NSs are sensitive to the metallicity of the progenitor stars, and they favor low-metallicity environments. In addition the second mass transfer episode, after the first compact object formation, can be either dynamically stable \citep[e.g.][]{2017MNRAS.471.4256V,2017MNRAS.468.5020I,2019MNRAS.490.3740N} or unstable \citep[e.g.,][]{1976ApJ...207..574S,1976IAUS...73...35V,1993MNRAS.260..675T,2007PhR...442...75K,2014LRR....17....3P,2016Natur.534..512B}. In the latter case this leads to a CE phase. The resulting tight system composed of a compact object and a Wolf--Rayet star can eventually undergo a tidal spin up of the star \citep{2018A&A...616A..28Q,2020A&A...635A..97B}. On the other end, if the second mass transfer is stable the binary will result in wider orbits compared to the evolution through CE and avoid a subsequent tidal spin up phase \citep{2020arXiv201016333B}. Eventually, following wind-driven mass loss, the secondary will collapse to a compact object. This leave us with either a BH+BH system or a NS+BH system with either a first- or second-born NS. 

The latter possibility (ii) occurs when two massive stars are born in a tight orbit (orbital periods less than 4 days) in low-metallicity environments which due to their tidal interactions can maintain the stars at almost critical rotation. Such rapidly rotating stars develop a temperature gradient between the poles and the equator leading to chemical homogeneous evolution \citep[e.g.,][]{2009A&A...497..243D,2016MNRAS.458.2634M,2016A&A...588A..50M,2020arXiv200211630D}. In these stars meridional circulation transport hydrogen from the surface into the core and helium out into the envelope until nearly all the hydrogen in the star is fused into helium. At the end of their main sequence these stars are essentially Wolf--Rayet stars and do not expand, hence, avoiding any additional mass-transfer phase.

LISA may answer whether or not mixed binaries of BHs and NSs, in which the NS formed first, are produced in the Galaxy. It is possible that the in-spiralling NS is unable to eject the envelope of the relatively massive BH progenitor star \citep{2018MNRAS.481.1908K}. 
Since we currently do not know of the existence of mixed BH+NS systems in the Galacy, any LISA detections of such systems, as well as double BH systems, will provide crucial information about their formation process. 



\subsubsection{Sources in clusters}\label{subsubsec:cluster-sources} 

\begin{figure*}
    \begin{center}
  \includegraphics[width=0.60\textwidth, angle=0]{./img_ucb/fig_LISA_WP_dynamical.png}
\caption{Illustration of the formation of LISA sources via examples of exchange encounters. See Figs.~\ref{fig:DWD} and \ref{fig:UCXB} for explanation of acronyms \citep[Figure from][]{TvdH23}.}
 \label{fig:dynamical}
  \end{center}
\end{figure*}




The inner regions of stellar clusters are cosmic factories of compact binaries (i.e.\,binaries containing two compact objects; BHs,  NSs or WDs), owing to the dominant role played by stellar dynamics in such environments. Massive stars in stellar clusters lose kinetic energy to lighter stars and accumulate into the cluster centre. In just a few Myr, these stars evolve into stellar BHs and NSs. 

The production of compact binaries can take one of two routes. If only a small fraction of BHs are retained within a cluster, encounters between BHs and binary stars  lead to dynamical exchanges, where the BH  replaces a less massive star within the binary \citep{1980AJ.....85.1281H}. Globular clusters have a considerably-enhanced population of X-ray binaries \citep{2003ApJ...598..501H}, which might have formed when a NS or a BH exchanges into a binary star \citep[e.g.,][]{1976MNRAS.175P...1H}. After the first exchange, evolution of the stellar companion (which might also become a BH or a NS)  or a second dynamical exchange can produce a compact binary.  Binary-single interactions represent an efficient mechanism to harden these binaries  \citep{1975MNRAS.173..729H} to the point where they can merge via the emission of gravitational radiation (see Fig.~\ref{fig:dynamical} for a schematic representation).  

Alternatively, if a large fraction of
BHs are retained in the cluster, they can form a BH subsystem 
\citep[][but see \citealt{2013MNRAS.432.2779B}]{1969ApJ...158L.139S,2007MNRAS.379L..40M,2008MNRAS.386...65M,2018MNRAS.479.4652A,2020ApJS..247...48K}. BHs in the subsystem tend to strongly interact with each other, undergoing frequent pairing, exchanges, and ejections. The most efficient mechanism driving binary formation in globular clusters is via three-body scatterings \citep[e.g.,][]{2015ApJ...800....9M}. After formation, a binary can undergo dozens of interactions with passing stars and binaries, which can lead to the production of  very hard binaries, capable of merging via the action of GW  emission \citep{2000ApJ...528L..17P}. 
If the star cluster centre harbours a BH subsystem, the BHs dominate the dynamics, quenching mass segregation and preventing the formation of binaries containing other compact objects \citep[see e.g.][]{2020ApJ...888L..10Y}. However, dynamically evolved clusters can lose a substantial fraction of the BHs. In these BH-poor clusters, binary-single interactions can allow the formation of binary NS and BH+NS binaries. Furthermore, it has been proposed that a parabolic encounter between two compact objects could potentially lead to the formation of a binary due to an abrupt loss of energy emitted as gravitational radiation \cite[e.g.][]{1972PhRvD...5.1021H,1989ApJ...343..725Q,2006ApJ...648..411K,2015MNRAS.448..754H}. However, the event rate of this mechanism, which is often referred to as the ``gravitational brake'' capture, is very likely to be negligible due to the small cross-section \citep{1990ApJ...358...81K}.




Old BH-poor clusters may also be ideal for dynamical formation of WD+WD binaries as well as BH/NS+WD binaries \citep{2020ApJS..247...48K}, see Fig.~\ref{fig:dynamical}. In old globular clusters, WDs are by far the most abundant type of compact object (roughly $10^5$ WDs are expected in a $10^6\,M_{\odot}$ cluster). A number of analyses have studied ways WD binaries,  both accreting and detached, may be dynamically assembled in stellar clusters \citep{1995ApJ...455L..47G,2006MNRAS.372.1043I,2016MNRAS.462.2950B,2018ApJ...852...29K}. Furthermore, a handful of the stellar-mass BH binary candidates observed in Galactic globular clusters are suspected to be ultra-compact accreting BH+WD binaries \citep{2012Natur.490...71S,2017MNRAS.467.2199B,2017ApJ...851L...4C}. Overall, up to a few dozen dynamically formed WD binaries are expected to be resolved by LISA in the Galactic globular clusters, likely constituting the largest class of dynamically-formed LISA sources in the Galaxy \citep{Willems2007,2019PhRvD..99f3003K}. Currently two candidates to AM CVns in globular clusters have been identified \citep{ 2016MNRAS.460.3660Z,2018MNRAS.475.4841R} and several more are expected to be discovered in upcoming globular cluster surveys.

Comparing nuclear stellar clusters with globular clusters, the former tend to have somewhat larger escape speeds \citep[due in part to the presence of a central massive BH, MBH:][]{2009MNRAS.397.2148G}. This means that a larger fraction of BHs are likely to be retained \cite[e.g.][]{2009ApJ...692..917M}, while the higher dispersion velocity inhibits both exchange encounters and the dynamical formation of binaries \citep[e.g.][]{2003gmbp.book.....H}. The presence of a dense nuclear cluster surrounding the MBH can significantly affect the formation process of compact binaries in a number of ways. Dynamical three body encounters can form at least one compact BH+BH if the nuclear cluster-to-MBH mass ratio exceeds 10, whereas at lower values the reservoir of compact binaries might be replenished via star cluster inspiral \citep[e.g.][]{2020ApJ...891...47A}. The presence of an MBH can leave significant imprints on the BH+BH evolution, owing to the possible development of von Zeipel--Kozai--Lidov cycles \citep{1910AN....183..345V,1962AJ.....67..591K,1962P&SS....9..719L}, which can boost the rate of BH+BH mergers \citep{2002ApJ...578..775B,2012ApJ...757...27A,2018ApJ...856..140H,2019MNRAS.488...47F,2020ApJ...891...47A} and significantly affect the BH mass spectrum in these extreme environments \citep[e.g.][]{2020ApJ...891...47A}. 


Young star clusters and open clusters, because of their relatively low total masses ($10^2\text{--}10^5$~M$_\odot$), host a smaller population of BHs with respect to globular and nuclear clusters \citep[e.g.,][]{2000ApJ...528L..17P,2010MNRAS.402..371B,2017MNRAS.467..524B,2021MNRAS.500.3002B}. BH+BHs in young/open star clusters mostly originate from dynamical exchanges or even from the evolution and hardening of primordial binaries \citep{2014MNRAS.441.3703Z,2019MNRAS.487.2947D,2020MNRAS.498..495D,2019MNRAS.486.3942K,2020MNRAS.495.4268K}. Furthermore, dynamical exchanges favour the formation of BH+NS binaries in young and open clusters \citep{2020MNRAS.497.1563R}.

Finally, hierarchical mergers in globular/nuclear clusters \citep[e.g.][]{2002ApJ...576..894M,2019PhRvD.100d3027R,2019MNRAS.486.5008A,2020ApJ...891...47A,2020ApJ...894..133A} or runaway collisions of massive stars \citep[e.g.][]{2004Natur.428..724P,2015MNRAS.454.3150G,2016MNRAS.459.3432M,2020arXiv200809571R} and binary star mergers in young star clusters \citep{2020MNRAS.497.1043D} might even lead to the formation of intermediate-mass BHs \citep{2019MNRAS.484..814G} and BHs with mass in the pair-instability gap \citep[e.g.][]{2020ApJ...894..133A}, similar to GW190521 \citep[][]{2020PhRvL.125j1102A,2020ApJ...900L..13A}.

\subsubsection{Triple stellar systems}\label{subsubsec:triples_formation}

\begin{figure*}
    \begin{center}
  \includegraphics[width=0.60\textwidth, angle=0]{./img_ucb/fig_LISA_WP_triple.png}
\caption{Illustration of the formation of a LISA source in a triple system. See Figs.~\ref{fig:DWD} and \ref{fig:UCXB} for explanation of acronyms \citep[Figure from][]{TvdH23}.}
 \label{fig:triple}
  \end{center}
\end{figure*}




Some of the LISA sources may form as part of triples and higher-order multiples. This includes sources in the Galactic disc (formed through e.g.\,isolated triple evolution) as well as those in dense environments. Three-body (or more) interactions are important in the formation of compact sources in two ways: during short-lived dynamical interactions and in hierarchical triple systems.


Hierarchical triples, in which two bodies orbit each other, and a third body orbits the centre of mass of the inner orbit, can remain stable for secular timescales, and therefore stay intact for Hubble times \citep{1994MNRAS.270..936K,1999ASIC..522..385M,2008CeMDA.100..151G,2018MNRAS.474...20H}. They may form in clusters (where they may interact with interloper stars in the densest environments) or exist in the Galactic disc (and evolve in pure isolation). Their evolution differs from that of isolated binaries due to three-body effects. Hence, triples that live their lives in isolation bridge the gap between classically isolated LISA sources and dynamically-evolving sources (often used to mean cluster sources). The importance of three-body interactions in hierarchical systems has been recognised for the evolution of stellar triples \citep{2011ApJ...741...82T,2013MNRAS.430.2262H,2017ApJ...836...39S,2017ApJ...841...77A,2017ApJ...846L..11L,2018A&A...610A..22T,2019MNRAS.486.4443F,2019MNRAS.486.4781F,2020A&A...640A..16T}, triples that consists of a combinations of stars and planets \citep{2016MNRAS.462L..84H,2017MNRAS.466.4107H,2018MNRAS.481.2180V,2018AJ....156..128S,2020ApJ...889...45S}, as well as stellar binaries in dense environments \citep{2012ApJ...757...27A,2016ApJ...816...65A,2017ApJ...846..146P,2016MNRAS.460.3494S,2019ApJ...878...58S, 2019MNRAS.488.5489H, 2019ApJ...881L..13H,2020ApJ...900...16F,2020arXiv200908468M,2020ApJ...900...16F}. 

The general formation of binaries and multiples (compact and wide) in clusters is boosted during the  collapse of the dense cluster core, which is halted by frequent stellar interactions \citep{1987degc.book.....S,1992PASP..104..981H}. The formation of the first binaries takes place most likely via three-body scatterings, involving three initially unbound objects \citep{1993ApJ...403..271G,1995MNRAS.272..605L}. As soon as binaries start forming, binary--single \citep{1983ApJ...268..319H,1993ApJ...415..631S} and binary-binary \citep{1983MNRAS.203.1107M,2002ApJ...576..894M} interactions take over and become the dominant dynamical processes at play. Even for relatively low triple fractions, dynamical interactions involving triples occur roughly as often as encounters involving either single or binary stars alone, particularly in low-mass star clusters \citep{2013MNRAS.432.2474L}. When the objects involved in the interaction cross their mutual sphere of influence, a strong interaction can trigger the formation of a short-lived bound triple system \citep{1993ApJ...403..271G}. During these chaotic resonances, a pair of objects has a non-negligible probability of experiencing a very close passage, triggering the formation of a compact binary and subsequent merger \citep{2014ApJ...784...71S}. Depending on the cluster structure, binary mergers developing through resonant interactions can be highly eccentric at LISA frequencies and even still when entering the frequency range typical of ground-based detectors \citep{2018PhRvD..97j3014S,2018MNRAS.481.5445S,2018arXiv180506458A}. Binary--binary interactions \citep{1984MNRAS.207..115M,1991ApJ...372..111M,2002ApJ...576..894M} represent another  efficient mechanism to form triples, either 
in the form of short lived, resonant unstable triples \citep{1983ApJ...268..319H,2019ApJ...871...91Z,2018arXiv180506458A}, or in a hierarchical configuration \citep{2016ApJ...816...65A,2019ApJ...871...91Z,2018arXiv180506458A,2020arXiv200908468M, 2020ApJ...900...16F}.


The best known manifestation of three-body dynamics are the von Zeipel--Kozai--Lidov cycles \citep{1910AN....183..345V, 1962P&SS....9..719L,1962AJ.....67..591K} regime in which the inner orbit eccentricity and the inclination between the two orbits vary periodically. Strictly speaking this applies to the (inner) test particle regime, an axisymmetric outer potential and the lowest-order expansion of the Hamiltonian (i.e.\,quadrupole). Relaxing either one of these assumptions leads to qualitative different dynamical evolution, which include extreme eccentricity variations and orbital flips \citep[see][for a review]{2016ARA&A..54..441N}. The high eccentricities can lead to close passages between the bodies, mass transfer, and enhancement of dissipative processes such as from tides or by GW  emission. Over time, the latter can lead to a significant reduction of the inner orbital separation during the nuclear burning stages or during the compact object phase of the stars \citep{1979A&A....77..145M,1998MNRAS.300..292K,2007ApJ...669.1298F,2011ApJ...741...82T}. Through the internal stellar evolution, a triple may transition from one dynamical regime to another, enhancing (or diminishing) the three-body effects \citep{2013ApJ...766...64S,2014ApJ...794..122M,2016ComAC...3....6T}. 






==> ucb_s1_intro.tex <==

Detection of GW emission from binary compact stars is one of the key drivers for the LISA mission. There are already at the time of writing {\color{blue}(July~2022) about two dozen known Galactic sources, most of which} are guaranteed to be detectable with LISA within a few years of its operation (Section~\ref{subsec:classes-binaries}). These are tight binaries (typically with orbital periods of $P_{\rm orb}\simeq 5-30\;{\rm min}$) of WD+WDs which give rise to continuous emission of GWs. 
Unlike binaries consisting of NSs and BHs, WD binaries (with their larger radii and thus lower orbital frequencies at merger) are not readily detectable by ground-based high-frequency (Hz--kHz) GW observatories, such as LIGO/Virgo/KAGRA, nor by the planned third generation of such detectors. These high-frequency detectors can observe the final a few - a few thousands orbits of inspiral (lasting a fraction of a second - minutes) and the merger event itself for NSs and BHs. Such merger events, however, are rare (of order a dozen events ${\rm Myr}^{-1}$ for a Milky~Way equivalent galaxy) and therefore they are only anticipated to be detected as extra-galactic sources, across volumes that encompass large numbers of galaxies. 
A major advantage of LISA is that the inspiral phase (due to orbital GW damping in the compact binaries) of the vast population of tight Galactic double WDs, NSs and BHs is in the low-frequency ($\sim$~mHz) GW window  for up to $\sim 10^6\;{\rm yr}$ prior to their merger event. Thus a significant number of such local sources are anticipated to be detected by LISA, even though their emitted GW luminosity is relatively small compared to that of the final merger process. The possibility that LISA can measure sky locations of its sources will allow for EM follow-up observations which may result in much more precise compact object component masses, e.g. compared to high-frequency GW mergers.

Binary population synthesis studies and early data-analysis work predicts of order $10^4$ resolved Galactic WD+WD may be detected with LISA. This population includes both detached WD+WD and those undergoing mass transfer (the so-called AM Canum Venaticorum binaries or AM~CVns, see Section~\ref{paragr:AM-CVns}). NS+NS systems are also expected to be detected by LISA. Based on the known Galactic population of tight-orbit radio pulsar binaries in combination with population synthesis predictions, an estimated number of $10^1-10^2$ NS+NS systems with a significant signal-to-noise ratio (SNR) may be detected by LISA within a 4-year mission (Section~\ref{paragr:DNS}). An even larger number of NS+WD systems is expected to be detected too, including ultra-compact X-ray binaries (UCXBs, see Section~\ref{paragr:UCXBs}, a sub-class of low-mass X-ray binaries, LMXBs). Binary BHs (BH+BH) detectable by LISA are strong candidates to become the first discoveries of such systems in the Milky Way.  
Given that LISA’s volume sensitivity for a constant SNR scales with chirp mass to the fifth power, $\mathcal{M}^5_{\rm chirp}$, BH+BH sources may be detected in distant galaxies, located several hundreds of megaparsecs away (see examples in Fig.~\ref{fig:horizons}). Interestingly enough, this fortuitous condition will therefore allow LISA to discover extra-galactic BH+BHs several years before the final merger events that LIGO/Virgo/KAGRA or Einstein Telescope/Cosmic Explorer will detect. Finally, LISA is also expected to detect rare Galactic systems such as (see Section~\ref{subsubsec:other_sources}): triple stellar systems, tight systems of WDs with exoplanets, or helium star binaries.

The LISA mission will provide  opportunities to learn new physics and answer key scientific questions related to formation and evolutionary processes of tight binary and multiple stellar systems containing compact objects. This includes questions related to the stability and efficiency of mass transfer, common envelopes (CEs), tides and stellar angular momentum transport, irradiation effects, as well as details of their formation and destruction in core-collapse supernovae (SNe) and Type~Ia SNe (and related transients), respectively. Furthermore, information about the environments of these sources will be available too, and the number and Galactic distribution of LISA sources are excellent probes to gain new knowledge on the star formation history and the structure of the Milky~Way. Finally, the sheer numbers of LISA sources will provide crucial knowledge concerning their formation and evolution processes and help to place constraints on key physical parameters related to binary (and triple-star) interactions.

The current catalogue of known LISA {\color{blue}``guaranteed sources''} consists of detached WD+WDs, accreting AM~CVn binaries, a hot subdwarf binary, and an UCXB. Although the sample is still small and inhomogeneous, binary population synthesis predicts a large population of multi-messenger sources that are EM bright and also detectable by LISA. This includes up to a few thousand detectable WD+WDs as well as a few tens of NS
or BH binaries, with a population strongly peaking towards the Galactic Plane/Bulge. Many sources will be detected across different EM bands. Detached WD+WDs and NS+WDs are typically seen in optical and UV bands, whereas AM~CVn systems and UCXBs are also seen in X-rays. NSs in compact binaries can potentially be detected as pulsars in the radio band. Therefore, in parallel with the LISA mission, we expect an EM bright future of thousands of resolved Galactic LISA binaries.

Systems with orbital periods $<20\;{\rm min}$ will be the strongest Galactic LISA sources and will be detected by LISA within weeks after science operations begin. These verification binaries, {\color{blue}as well as other so far unknown loud sources,} are crucial in facilitating the functional tests of the instrument and maximize LISAs scientific output. Combined GW and EM multi-messenger studies of UCXBs will allow us to derive population properties of these systems with unprecedented quality including for the first time the effects of tides compared to GW  radiation. Tides are predicted to contribute up to $10\,\%$ of the orbital decay. For accreting WDs as well as NS binaries, multi-messenger observations give us the possibility to study the angular momentum transport due to mass transfer. In particular for monochromatic GW sources, EM observations are required to break degeneracies in the GW data (e.g. between masses and distance).

\begin{figure*}[h!]
    \begin{center}
   \includegraphics[width=0.60\textwidth]{./img_ucb/LISA_horizons_v4.png}
\caption{Distance to which LISA binaries can be detected as a function of GW frequency. The coloured lines represent the SNR threshold of 7 (here computed assuming a mission duration of 4~yr with 100\% duty cycle) for (quasi-)stationary equal-mass circular binaries of different total masses in the distance--GW frequency parameter space. The shaded range represents angle-averaged curve limits for the optimal and worst binary orientation. The ticks on the curves represent binary merger times: for merger times $\gg 4\;{\rm yr}$ the binary will be seen by LISA as a monochromatic GW source, whereas for merger times $< 4\;{\rm yr}$ the binary will be seen as evolving. Note in particular that evolving sources like GW190521 and GW150914 remain within the LISA band for less than the mission lifetime. Figure credit: Antoine Klein \& Valeriya Korol.}
 \label{fig:horizons}
  \end{center}
\end{figure*}


==> ucb_s2.1_VerificationSources.tex <==
\subsubsection{Known binaries --- LISA verification sources}\label{subsec:verification sources}

\noindent \coord{Thomas Kupfer, Thomas Tauris}\\
\noindent \contr{Thomas Kupfer, Thomas Tauris, Silvia Toonen, Tassos Fragos}\\

The most abundant sources in the LISA band will be binary stars with orbital periods $<60$\,min, so-called ultra-compact binaries (UCBs). They are a class of binary stars with ultrashort orbital periods, consisting of a WD or NS primary and a compact helium-star/WD/NS secondary. A subset of the known UCBs have predicted GW strains high enough that they will be individually detected due to their strong GW signals \citep[e.g.][]{2020ApJ...905...32B}. These LISA guaranteed sources are termed {\it verification binaries} with some being expected to be detected on a timescale of weeks or a few months \citep{2006CQGra..23S.809S}. Currently, we know of only about two dozen of these systems although hundreds are predicted by theory to be detectable in our Galaxy \citep[e.g.][]{2004MNRAS.349..181N,2006PhRvD..73l2001T,2013MNRAS.429.2361L,2017MNRAS.470.1894K, 2017ApJ...846...95K, 2018MNRAS.480..302K, 2019MNRAS.490.5888L}.

At present, the catalogue of verification binaries include 13 WD+WDs, 11 semi-detached accreting WDs (AM\,CVn binaries, a subclass of Cataclysmic Variables, CVs), one hot subdwarf star with a WD companion, and one semi-detached UCXB. Table\,\ref{tab:verif_systems} and \ref{tab:verif_systems1} present an overview of the known systems with observed EM properties. Figure\,\ref{fig:strain} shows the characteristic strain of the known verification binaries which reach a predicted ${\rm SNR}\geq5$ in LISA assuming an optimistic 10~year mission with an 80\% duty cycle. So far large-scale searches for verification binaries have been conducted almost exclusively in the northern hemisphere, because large-scale survey instruments (e.g. the Sloan Digital Sky Survey, SDSS, and the Zwicky Transient Facility, ZTF) are located in the Northern Hemisphere, and mostly at high Galactic latitudes, to avoid stellar crowding. Fig.\,\ref{fig:skylocation} shows the sky location of the known verification systems which presents the strong bias towards sources in the Northern Hemisphere.

\begin{figure*}[h!]
    \begin{center}
  \includegraphics[width=0.73\textwidth,]{./img_ucb/verification_systems_10years.pdf}
\caption{Sensitivity plot for LISA assuming 10~yr of observation with an 80\% duty cycle showing the known binaries which reach a ${\rm SNR}\geq5$. Filled symbols represent eclipsing sources and open symbols represent non-eclipsing sources from \citet{2018MNRAS.480..302K}. The black lack solid line represents the LISA sensitivity curve. Acronyms for binaries: AM Canum Venaticorum (AM~CVns), WD+WD (DWDs), subdwarf B-star (sdB) and ultracompact X-ray binary (UCXB). Figure credit: Thomas Kupfer.}
 \label{fig:strain}
  \end{center}
\end{figure*}


In 2018, Gaia data release 2 \citep{2018A&A...616A...1G} announced parallaxes for $\approx1.3$ billion sources. The Gaia catalogue contains the distances of many of the known LISA verification binaries, allowing accurate prediction of their GW strains. Using the Gaia distances, \citet{2018MNRAS.480..302K} found 13 sources will exceed an SNR of 5 after 4~yr of LISA observations. This  sample consists of 13 verification binaries from the current, known list; it is strongly biased and incomplete. It includes AM\,CVn, CR~Boo, V803~Cen and ES~Cet, which were all found as outliers in surveys for blue, high-Galactic latitude stars. HM~Cnc and V407~Vul are the most compact known AM\,CVn systems and were discovered during the course of the ROSAT All-Sky Survey showing an on/off X-ray profile modulated on a period of 321 and 569~s respectively. The known WD+WD verification binaries, such as SDSS J0651 and SDSS J0935, were found as part of the extremely low-mass (ELM) WD survey (\citealt{2020ApJ...889...49B} and references therein). 


More recently, more systematic searches for UCBs were performed. UCBs show up in lightcurves with variations on timescales of the orbital period (e.g.\, due to eclipses or tidal deformation of the components). Therefore, photometric surveys are well suited to identify UCBs in a homogeneous way. A number of fast cadence ground-based surveys, including the Rapid Temporal Survey (RATS; \citealt{2005MNRAS.360..314R,2011MNRAS.413.2696B}), OmegaWhite (\citealt{2015MNRAS.454..507M}) survey as well as the ZTF high-cadence Galactic plane survey \citep{2019PASP..131a8003M,2021MNRAS.505.1254K}, have been executed to study the variable sky down to a few minute period aiming to find UCBs and increase the number of known verification binaries. The ELM survey targets a colour-selected sample of B-type hypervelocity candidates from SDSS \citep[][]{2005AJ....130.2230A,2007MNRAS.382..685R}, which are being followed up systematically (\citealt{2020ApJ...889...49B} and references therein). ELM~WDs can be separated efficiently from the bulk of WDs with a colour selection \citep{2010ApJ...723.1072B}.

Over the last few years the number of known verification binaries has almost doubled thanks to these large scale surveys. The two most significant contributors were the ELM survey (\citealt{2020ApJ...889...49B} and references therein) and ZTF \citep{2019Natur.571..528B, 2020ApJ...905...32B,2020arXiv201003555B}. The ELM survey discovered six WD+WD verification binaries including SDSS\,J0651: a detached eclipsing system with an orbital period of 12~min. Most recently ZTF released seven new WD+WD verification binaries, five systems found as eclipsing sources. Remarkably, one of the first ZTF discoveries was the shortest orbital period eclipsing WD+WD known to date, ZTF~J1539+5027, with an orbital period of just 6.91~min \citep{2019Natur.571..528B}. 

\begin{figure*}[h!]
    \begin{center}
  \includegraphics[width=0.95\textwidth,]{./img_ucb/sky_coord_verif.pdf}
\caption{Sky position of the verification binaries. The sky positions show a clear bias towards the northern hemisphere and to higher Galactic latitudes. The black line indicates the Galactic equator and $|b| = 10$\,deg, with the Galactic Centre located at the black cross. See caption in Fig.~\ref{fig:strain} for explanation of acronyms. Figure credit: Thomas Kupfer.}
 \label{fig:skylocation}
  \end{center}
\end{figure*}

\begin{table*}[ht]
\begin{center}
\caption{Physical properties (orbital periods, component masses, inclination angles) of the known verification binaries which reach a ${\rm SNR}>5$ after a 10~yr LISA mission with 80\% duty cycle. Masses and inclination angles in brackets are assumed and based on evolutionary stage and mass ratio estimations.}
\begin{tabular}{lrllll}
\hline
\hline
Source         & $P_{\rm orb}$ &  $M_1$ & $M_2$ & $\iota$ & Refs.  \\
             &   (s)          &  (M$_\odot$) &    (M$_\odot$)  &  ($\deg$)    \\
                      \hline
\multicolumn{2}{l}{{\bf AM\,CVn type}}      &     \\
HM Cnc                     &   321.5  &   0.55     &  0.27  & $\approx$38 & 1, 2  \\
V407 Vul                   &   569.4  &   [0.8$\pm$0.1]   & [0.177$\pm$0.071]   & [60]  & 3  \\
ES Cet                     &   620.2  & [0.8$\pm$0.1]  &  [0.161$\pm$0.064] &  [60] & 4  \\ 
SDSS J135154.46$-$064309.0 &   943.8  &    [0.8$\pm$0.1]     &  [0.100$\pm$0.040]  & [60]  & 5  \\
AM CVn                     &  1028.7  &  0.68$\pm$0.06 &  0.125$\pm$0.012  & 43$\pm$2 & 6, 7  \\
SDSS J190817.07+394036.4   &  1085.7  & [0.8$\pm$0.1]  & [0.085$\pm$0.034]  & 10 - 20 & 8, 9  \\
HP Lib                     &  1102.7  &  0.49-0.80 & 0.048-0.088 & 26-34 & 10,11  \\
PTF1 J191905.19+481506.2   &  1347.3  & [0.8$\pm$0.1] & [0.066$\pm$0.026] & [60] & 12  \\
CXOGBS J175107.6$-$294037  &  1375.0  & [0.8$\pm$0.1] &  [0.064$\pm$0.026] & [60]  & 13  \\
CR Boo                     &  1471.3  & 0.67-1.10 &  0.044-0.088 & 30  & 10,14  \\
V803 Cen                   &  1596.4  &  0.78-1.17 & 0.059-0.109 & 12 - 15 & 11  \\
     \noalign{\smallskip}
 \multicolumn{3}{l}{{\bf Detached double WDs}}         & \\
 ZTF J1539+5027            &  414.8  &    $0.610^{+0.017}_{-0.022}$ &	$0.210\pm0.015$	& $84.15^{+0.64}_{-0.57}$   &   15    \\
 ZTF J2243+5242            &  527.9  &   $0.349^{+0.093}_{-0.074}$ & $0.384^{+0.114}_{-0.074}$ & $81.88^{+1.31}_{-0.69}$ &   16   \\
SDSS J065133.34+284423.4   &  765.5  &  0.247$\pm$0.015 &  0.49$\pm$0.02 & ${86.9^{+1.6}_{-1.0}}$  & 17, 18  \\
 ZTF J0538+1953            &  866.6  &    $0.45\pm0.05$  &	$0.32\pm0.03$   &  $85.43^{+0.07}_{-0.09}$  &   19 \\
SDSS J093506.92+441107.0   & 1188.0  &  0.312$\pm$0.019 &  0.75$\pm$0.24 &  [60]  & 20, 21  \\
SDSS J2322+0509            & 1201.4  &  $0.34\pm0.02$   & $>0.17$ &  [60]    & 22 \\
 PTF J0533+0209            & 1234.0  &   $0.652^{+0.037}_{-0.040}$ &  $0.167\pm0.030$  & $72.8^{+0.8}_{-1.4}$ & 19, 23 \\
 ZTF J2029+1534            & 1252.0  &   $0.32\pm0.04$  &   $0.3\pm0.04$   &  $86.64^{+0.70}_{-0.40}$ &   19 \\
 ZTF J0722$-$1839          & 1422.5  &   $0.38\pm0.04$  & $0.33\pm0.03$   & $89.66\pm0.22$   &  19  \\
 ZTF J1749+0924            & 1586.0  &  $0.40^{+0.07}_{-0.05}$  &  $0.28^{+0.05}_{-0.04}$  &	$85.45^{+1.40}_{-1.15}$  &  19   \\
SDSS J163030.58+423305.7   & 2389.8  &  0.298$\pm$0.019 &  0.76$\pm$0.24 & [60]  & 20, 24 \\
SDSS J1235+1543            & 3172.6  &  $0.35\pm0.01$ &  $0.27^{+0.06}_{-0.02}$  &	$27\pm3.8$ &  25, 26  \\
SDSS J092345.59+302805.0   & 3883.7  &  0.275$\pm$0.015 &  0.76$\pm$0.23 & [60] & 20, 27 \\
      \noalign{\smallskip}
  \multicolumn{3}{l}{{\bf Hot subdwarf binaries}}      & \\
  CD$-$30$^\circ$11223       & 4231.8   &   0.54$\pm$0.02     &  0.79$\pm$0.01  & 82.9$\pm$0.4 & 28 \\
        \noalign{\smallskip}
  \multicolumn{3}{l}{{\bf Ultracompact X-ray binaries}}      & \\
  4U1820$-$30                &  685.0  &   [1.4]	&  [0.069]	&  [60]  &  29, 30 \\  
\hline
 \hline
 \end{tabular}
\begin{flushleft}
[1] \citet{2005ApJ...627..920S}, [2] \citet{2010ApJ...711L.138R}, [3] \citet{2002MNRAS.331L...7M}, [4] \citet{2005PASP..117..189E}, [5] \citet{2018MNRAS.477.5646G}, [6] \citet{1999PASP..111.1281S}, [7] \citet{2006MNRAS.371.1231R}, [8] \citet{2011ApJ...726...92F}, [9] \citet{2015MNRAS.453..483K}, [10] \citet{2007MNRAS.379..176R}, [11] \citet{2021MNRAS.500.1222S}, [12] \citet{2014ApJ...785..114L}, [13] \citet{2016MNRAS.462L.106W}, [14] \citet{1997ApJ...480..383P}, [15] \citet{2019Natur.571..528B}, [16] \citet{2020arXiv201003555B}, [17] \citet{2011ApJ...737L..23B}, [18] \citet{2012ApJ...757L..21H}, [19] \citet{2020ApJ...905...32B}, [20] \citet{2016ApJ...824...46B},  [21] \citet{2014MNRAS.444L...1K}, [22] \citet{2020ApJ...892L..35B}, [23] \citet{2019ApJ...886L..12B}, [24] \citet{2011MNRAS.418L.157K}, [25] \citet{2017MNRAS.468.2910B}, [26] \citet{2017MNRAS.471.4218K}, [27] \citet{2010ApJ...723.1072B}, [28] \citet{2013A&A...554A..54G}, [29] \citet{1987vgex.conf..157S}, [30] \citet{2020ApJ...900L...8C}
 \label{tab:verif_systems}
\end{flushleft}
\end{center}
\end{table*}


\begin{table*}[ht]
\begin{center}
\caption{Measured EM properties (Galactic coordinates, GW frequency, magnitudes and parallaxes from Gaia early data  release 3 \citep{2020arXiv201201533G} of the known verification binaries which reach a ${\rm SNR}>5$ after a 10~yr LISA mission with 80\% duty cycle.}
\begin{tabular}{lrrrrc}
\hline
\hline
Source              & $f_{\rm GW}$    &  $l_{\rm Gal}$   &  $b_{\rm Gal}$ &  Gaia G &  $\varpi$   \\
                   & (mHz)    & (deg)  & (deg) & mag    &   (mas)      \\
                      \hline
\multicolumn{3}{l}{{\bf AM\,CVn type}}      &     \\
HM Cnc                     &  6.22  &  206.9246 &	23.3952 &	20.92 &  ---  \\
V407 Vul                   &  3.51  &  57.7281	&  6.4006   &  19.36  & 0.0978$\pm$0.2384 \\
ES Cet                     &  3.22  &  168.9684 & $-$65.8632	 & 16.80 & 0.5606$\pm$0.0677  \\ 
SDSS J135154.46$-$064309.0 &  2.12  &  328.5021 & 53.1240 &	18.72  & 0.6584$\pm$0.2197 \\
AM CVn                     &  1.94  &  140.2343 & 78.9382  & 14.06  & 3.3106$\pm$0.0303 \\
SDSS J190817.07+394036.4   &  1.84  &  70.6664 & 13.9349 & 16.22 & 1.0232$\pm$0.0335 \\
HP Lib                     &  1.81  & 352.0561 & 32.5467 & 13.60 & 3.5674$\pm$0.0313 \\
PTF1 J191905.19+481506.2.  &  1.48  & 79.5945 & 15.5977 & 19.75 & 0.6229$\pm$0.2385 \\
CXOGBS J175107.6$-$294037  &  1.45  &  359.9849 & $-$1.4108 & 16.27 & 0.8591$\pm$0.1733 \\
CR Boo                     &  1.34  & 340.9671 & 66.4884 &  15.47 & 2.8438$\pm$0.0367  \\
V803 Cen                   &  1.25  & 309.3671 & 20.7262 & 15.73 & 3.4885$\pm$0.0599 \\
     \noalign{\smallskip}
 \multicolumn{3}{l}{{\bf Detached double WDs}}         & \\
 ZTF J1539+5027            &  4.82  & 80.7746 & 50.5819 & 20.40 & $-$0.4926$\pm$0.5726 \\
 ZTF J2243+5242            &  3.79  & 104.1514 & $-$5.4496 & 20.55 & $-$1.2372$\pm$0.6578 \\
SDSS J065133.34+284423.4   &  2.61  & 186.9277 & 12.6886 & 19.28 & 1.0071$\pm$0.3091    \\
 ZTF J0538+1953            &  2.31  & 186.8104 & $-$6.2213 & 18.80 & 0.9617$\pm$0.2866 \\
SDSS J093506.92+441107.0   &  1.68  & 176.0796 & 47.3776 & 17.80 & 2.7034$\pm$0.6648  \\
 SDSS J2322+0509           &  1.66  & 85.9507 & $-$51.2104 & 18.75 & 1.1558$\pm$0.2244 \\
 PTF J0533+0209            &  1.62  & 201.8012 & $-$16.2238 & 19.05 & 0.7902$\pm$0.2396  \\
 ZTF J2029+1534            &  1.60  & 58.5836 & $-$13.4655 & 20.47 & 0.1240$\pm$0.9893   \\
 ZTF J0722$-$1839          &  1.40  & 232.9930 & $-$1.8604 & 19.05 & 0.6996$\pm$0.2457 \\
 ZTF J1749+0924            &  1.26  & 34.5093 & 17.9025 & 20.47 & $-$0.2961$\pm$0.8222 \\
SDSS J163030.58+423305.7   &  0.84  & 67.0760 & 43.3604 & 19.18 & 1.1748$\pm$0.1952 \\
SDSS J1235+1543            &  0.63  & 284.5186 & 78.0320 & 17.52 &  2.2504$\pm$0.1389  \\
SDSS J092345.59+302805.0   &  0.51  & 195.8199 & 44.7754 & 15.92 & 3.4795$\pm$0.0648 \\
      \noalign{\smallskip}
  \multicolumn{3}{l}{{\bf Hot subdwarf binaries}}      & \\
  CD--30$^\circ$11223       &   0.47  & 322.4875 & 28.9379 & 12.30 & 2.8198$\pm$0.0516 \\
        \noalign{\smallskip}
  \multicolumn{3}{l}{{\bf Ultracompact X-ray binaries}}      & \\
  4U1820$-$30                &  2.92  & 2.7896 & $-$7.9144 & 15.41 & $-$0.7676$\pm$0.2164 \\
\hline
 \hline
 \end{tabular}
\begin{flushleft}
 \label{tab:verif_systems1}
\end{flushleft}
\end{center}
\end{table*}

\clearpage

==> ucb_s2.2_DetachedBinaries.tex <==
\subsubsection{Detached binaries}\label{subsubsec:detached-binaries}

\noindent \coord{Ashley Ruiter, Ross Church}\\
\noindent \contr{Ashley Ruiter (1.2.2.1), Thomas Tauris (1.2.2.2--4), Jeff Andrews (1.2.2.3), Simone Bavera (1.2.2.4), Ross Church (1.2.2.2), Tassos Fragos (1.2.2.4), Gijs Nelemans (1.2.2.1), Milton Ruiz (1.2.2.3), Alberto Sesana (1.2.2.4), Antonios Tsokaros (1.2.2.3), Shenghua Yu (1.2.2.3)}

\paragraph{WD+WD systems}\label{paragr:DWD-detached} %  

\phantom{text}

For over three decades it has been known that WD+WD binaries will be the dominant contributor to signals detected by a space-based GW observatory \cite[][]{1990ApJ...360...75H}. While most extra-galactic sources \citep{2003MNRAS.346.1197F} as well as a significant fraction of those in the Galactic halo \citep{2009ApJ...705L.128R} are likely too distant to be individually detected by LISA, a large portion of the frequency band observed by LISA will be swamped with GWs from millions of WD+WDs existing in the Galactic disc and bulge. At low frequencies, the combined signal of these millions of WD+WDs will populate just a few frequency bins and merge to form an unresolved confusion foreground (often referred to as the galactic foreground or the galactic confusion noise), with louder resolvable sources standing out above the confusion (see also Section~\ref{subsubsec:GWforeground}). Together with high-frequency sources a large number these form $\sim 10^4$, (e. g., \citealt{2001A&A...365..491N,2003MNRAS.346.1197F,2010ApJ...717.1006R,2017MNRAS.470.1894K}) of resolved WD+WDs and we now discuss these key sources in more detail.

WD+WDs were discovered in the late 1980s and initially were dominated by low-mass ($\lesssim 0.4\;M_\odot$) helium-core (He-core)~WDs that cannot be formed in single-star evolution within a Hubble time, and, thus, were the targets for radial velocity searches for binarity amongst known WDs \citep{1995MNRAS.275..828M}. Later, (more) unbiased surveys were done, e.g. the Supernova Ia Progenitor surveY \citep[SPY, ][and references therein]{2020A&A...638A.131N} and studies using SDSS,
discovering also more massive WDs. Over the last decade, it has become more clear that previously-undetected WD+WD systems (and their progenitors, e.g. double-core planetary nebulae) are more easily detectable with today's sophisticated instrumentation \citep{2018MNRAS.480.4589W}. A dramatic increase in the number of WD+WDs has come from the ELM WD survey \citep{2012ApJ...751..141K,2017ApJ...835..180B,2020ApJ...889...49B} that targets a part of the parameter space in colour--colour diagrams that is occupied by (subdwarf) B-stars, but also by very low mass (below $\sim 0.3\;M_\odot$) proto-WDs that are still approaching the cooling track and are thus relatively large and bright \citep{2014A&A...571L...3I,2016A&A...595A..35I}. In total, the ELM survey alone has discovered 98 WD+WDs so far \citep{2020ApJ...889...49B}. 

Over the past couple of years, ZTF \citep[[]{2019PASP..131a8002B} has facilitated a rapid growth in the population of known WD+WDs with orbital periods under an hour. Three of the sources discovered by ZTF so far \citep{2020arXiv201003555B}, the eclipsing WD+WDs: ZTF~J1539+5027 ($P_b = 6.91\;{\rm min}$), ZTF~J2243+5242 ($P_b = 8.80\;{\rm min}$) and ZTF~J0538+1953 ($P_b = 14.4\;{\rm min}$),
should all be detected by LISA with a high SNR, enabling precise parameter estimation using GWs \citep{2019ApJ...881L..43L}.

The detached WD+WDs may consist of a pair of He-core WDs, carbon/oxygen-core (C/O-core) WDs, oxygen/neon/magnesium-core (O/Ne/Mg-core) WDs, or any mixed combination thereof. For some systems, LISA measurements of the orbital-decay rate will yield the chirp mass for a given system, which can be combined with EM observations to reveal individual WD component masses. The distribution of WD masses (and their mass ratios), along with the number of detectable sources in a local volume, will provide important information to help understand their formation history (see Section~\ref{subsec:formation-binaries}). 
With enough detached WD+WDs in a sample, it may even be possible to set limits on mass-transfer efficiencies and CE physics (Section~\ref{subsec:scientificQ}) through characterisation of chirp mass distributions \citep{2019MNRAS.484..698R}. 
Furthermore, the detected WD+WDs will provide unique information on the formation of progenitors of R~Coronae Borealis stars, thought to be formed by the merger of two WDs, e.g. \citep{2020A&A...635A..14T}, massive carbon-enhanced WDs \citep{2020MNRAS.491L..40K}, Type~Ia SNe (see Section~\ref{paragr:SNeIa}), and other transients. 
 
Over the last three decades, several works have made predictions about the scientific impact of LISA detections of Galactic WD+WDs. Different binary evolution population synthesis studies have uncovered how the WD+WD population will look to LISA in terms of characteristic strain amplitude \citep{2001A&A...375..890N,2004MNRAS.349..181N,2010A&A...521A..85Y,2019MNRAS.490.5888L,2020A&A...638A.153K}, spectral density \citep{2020ApJ...901....4B}, as well as how different populations of WD+WDs contribute to the spectral amplitude signal \citep{2009ApJ...705L.128R,2010ApJ...717.1006R}.

Detached WD+WD binaries that are resolvable with LISA are expected to be on par with or slightly outnumber the resolvable interacting WD+WD binaries \citep{2001A&A...368..939N,2004MNRAS.349..181N,2010ApJ...717.1006R}, and will be the sole WD+WD contributers to the LISA signal at GW frequencies below $\sim 2 \times 10^{-4}\;{\rm Hz}$. \cite{2017ApJ...846...95K} found that a number of {\em mass-transferring} WD+WDs (Section~\ref{subsubsec:interacting-binaries}) will be resolvable with LISA ($\sim 200-3000$ for SNRs between 10 and 5, respectively), many of which are likely to exhibit a negative chirp (caused by orbital widening) --- a diagnostic not applicable for detached WD+WDs. 
Finally, we expect that the number of detached WD+WDs, composed of a light He-core~WD and a more massive C/O-core~WD (or possibly an O/Ne/Mg-core~WD) detected by LISA must be in accordance with the number of similar interacting AM~CVn systems that LISA will detect, given their evolutionary connection (the detached systems being the precursors of the interacting WD+WDs, see Fig.~\ref{fig:DWD}). The transitional GW frequency between these two populations (detached and interacting) depends on the mass and temperature of the lighter (last-formed) WD, see examples in Figs.~\ref{fig:UCXB_strain+data} and \ref{fig:UCXB-AMCVn-detailed}. 


\paragraph{NS+WD and BH+WD systems}\label{paragr:WD+N} 

\phantom{text}

The known population of Galactic NS+WD systems can be divided into two classes. Systems with: i) massive WDs (O/Ne/Mg-core or C/O-core WDs, typically more massive than $0.7\,M_\odot$), and ii) low-mass He-core~WDs (typically less massive than $0.3\,M_\odot$). The massive NS+WD systems can again be subdivided into two populations, depending on the formation order of the WD and the NS. The NS+WD systems are observed as binary radio pulsars and the formation order can be clearly distinguished from the properties of the pulsar: if the pulsar has a strong B-field and an eccentric orbit \citep[e.g.][]{2000A&A...355..236T,2006MNRAS.372..715C}, it is the last-formed compact object, whereas if the pulsar is (mildly) recycled with a low-B-field and a fairly rapid spin, and in a near-circular orbit, it is the first-formed compact object \citep[][]{2012MNRAS.425.1601T}. 
For LISA detections, the formation order is irrelevant and among both types of systems examples are known to merge within a Hubble time, thus producing a bright LISA source well before their final merger.

Among the detached low-mass He-core~WDs with NS companions, the systems in relatively tight orbits are completely dominated by millisecond radio pulsars. 
According to the ATNF Pulsar Catalogue \citep{2005AJ....129.1993M}, there are about 120 such systems known in the MW disc, a handful of which will merge within a Hubble time, producing a bright detached LISA source (depending on their distance) for approximately the last several tens of Myr of the inspiral, before an UCXB is formed (Section~\ref{paragr:UCXBs}).
Based on the observed population of radio pulsars and their selection effects, \citet{2018PhRvL.121m1105T} argue that LISA could detect about 50 of these systems while still detached, before they become UCXBs and widen their orbits again, resulting in a negative chirp of the GW signal (see Figs.~\ref{fig:UCXB_strain+data} and \ref{fig:UCXB-AMCVn-detailed}). 

At present, we do not know of any detached BH+WD binaries. However, this is probably due to observational selection effects since the only EM radiation we would expect from such detached systems would be from the cooling of the WD companion --- unlike the situation for semi-detached systems or systems containing NSs, which can be detected in X-rays and radio waves, respectively. Nevertheless, several Galactic LMXBs are known with low-mass donor stars and BH accretors \citep{2006csxs.book..157M} and thus we expect many of these systems to leave detached BH+WD systems, possibly (although still to be proven) in tight orbits that LISA will detect. A more viable formation channel for more massive WDs in tight orbits with BHs is formation via a CE.
Optical follow-up observations of the WD companion, in combination with the measured chirp mass, will constrain the BH mass in these systems. Early simulations \citep{2001A&A...375..890N} predict a Galactic merger rate of BH+WD binaries of order $\sim 100\;{\rm Myr}^{-1}$ and thus roughly $\sim 100$ such systems detectable by LISA.


\paragraph{NS+NS systems}\label{paragr:DNS} 

\phantom{text}

The known population NS+NS systems so far only manifest themselves as radio pulsars. The first one of these (PSR~B1913$+$16, the {\it Hulse--Taylor Pulsar}) was discovered in 1974 \citep{1975ApJ...195L..51H}. According to the ATNF Pulsar Catalogue \citep{2005AJ....129.1993M}, there are currently about 20 NS+NS systems detected in our Galaxy. Except for one case, the {\it double pulsar} PSR~J0737$-$3039 \citep{2004Sci...303.1153L}, only one of the two NSs is detected --- usually the recycled pulsar \citep{2017ApJ...846..170T}. The other NS, is either not an active radio pulsar anymore or it is not beaming in our direction. 

Given the small merger rate of NS+NS systems in our Galaxy\footnote{The empirical rate and its uncertainty measured by the LIGO network of detectors is currently based on only two events (GW170817 and GW190425) but is anticipated to improve substantially in the coming decade.} (most likely somewhere in the range from a few events up to a hundred events per~Myr), it is statistically highly improbable that ground-based high-frequency detectors (LIGO--Virgo--KAGRA) will detect a NS+NS merger in the Local Group earlier than the LISA era. 
The advantage of LISA is that it can follow the inspiral of Galactic NS+NS systems up to $\sim 10^6\;{\rm yr}$ prior to their merger event, and thus a significant number of NS+NS sources are anticipated to be detected in GWs by LISA.

About half of the 20 known NS+NS systems have orbital periods small enough (or eccentricities sufficiently large) to merge within a Hubble time. As an example, a ``standard'' NS+NS system with NS masses of $1.35\;M_\odot$ and e.g. an orbital period of 16~hr will merge in: 11.8~Gyr, 4.4~Gyr or 0.35~Gyr for an initial eccentricity, $e_0$ of 0.1, 0.5 or 0.8, respectively. 
The number of NS+NS sources that LISA will detect can be evaluated, approximately to first order, from a combination of the Galactic NS+NS merger rate and the distribution of these sources within the Milky Way. The above three standard NS+NS systems will have a remaining lifetime of between $\sim 247\;{\rm kyr}$ ($\sim 243\;{\rm kyr}$ for $e_0=0.8$) and $1.57\;{\rm Myr}$ ($1.48\;{\rm Myr}$ for $e_0=0.8$) by the time they enter the LISA band, if this occurs at a GW frequency of about 2~mHz and 1~mHz, respectively. Thus, if the Galactic merger rate is, say, $10\;{\rm Myr}^{-1}$, we can roughly expect to detect between a few and a dozen LISA sources. Of course, the details depend on the Galactic distribution of these sources, the SNR required for a detection, and the duration of the LISA mission.
The merger rate can be estimated from population synthesis, but its value is uncertain by, at least, one or two orders of magnitude \citep{2010CQGra..27q3001A}. The merger rate derived from an extrapolation of the LIGO/Virgo empirical merger rate of NS+NSs still has very large error bars due to small number statistics.

Recent works by \citet{2020MNRAS.492.3061L,2020ApJ...892L...9A} suggest that LISA may even detect up to $\sim 50-200$ Galactic NS+NS sources with a SNR greater than 7 within a 4~yr mission. Given that LISA’s volume sensitivity for a constant SNR scales with $\mathcal{M}^5_{\rm chirp}$, unlike double BH sources, very few NS+NS sources are anticipated to be detected outside the Milky Way, although a few such binaries may be found in both the LMC and M31 \citep{2019MNRAS.489.4513S}. 
Applying a more conservative number, however, for the merger rate of Galactic NS+NS system of about $3-14\;{\rm Myr}^{-1}$ \citep{2018MNRAS.481.1908K} would lead to a substantial reduction in the predicted number of LISA detections. The Galactic merger rate is expected to be significantly better constrained in the coming decade such that we will have a clear idea about the expected number of NS+NS sources detected by LISA prior to its operation. Finally, an expected reduction in LISA SNR for detecting eccentric NS+NS systems, compared to circular NS+NS systems with similar orbital period and NS masses, should be noticed \citep{2021arXiv210316030R}.

LISA may give us the opportunity to probe a hidden subpopulation of NS+NS systems with different properties compared to those of the well-known radio pulsar NS+NSs.
The nature of GW190425, a presumed NS+NS merger detected by the LIGO/Virgo network with a total mass of $3.4\;M_\odot$ \citep{2020ApJ...892L...3A}, is still a mystery.
With such a large total mass, GW190425 stands at five standard deviations away from the total mass distribution of Galactic NS+NSs detected in the Milky Way as radio pulsars \citep{2019ApJ...876...18F}. If a subpopulation of heavy GW190425-like NS+NSs exists in our Galaxy, it is not yet clear why it should be radio-quiet \citep[e.g.][]{2020ApJ...900...13S}. Thus, LISA may actually be the most suited instrument for detecting the population of GW190425-like binaries \citep{2021ApJ...909L..19G, 2021MNRAS.502.5576K}. In particular, \citet{2021MNRAS.502.5576K} demonstrated that if GW190425-like binaries constitute a fraction larger than 10\% of the total Galactic population, LISA should be able to recover this fraction with better than $\sim 15$\% accuracy, assuming the merger rate of $42\;{\rm Myr}^{-1}$.

Additional recent investigations \citep{2020MNRAS.493.5408T,2019MNRAS.483.2615K} have discussed the importance of sky-localization on LISA NS+NS sources for multi-messenger follow-ups that may allow to impose constraints on the equation-of-state of NSs by measuring the Lense--Thirring precession \citep{2020MNRAS.493.5408T} or test general relativity through the detection of radio pulses from Galactic NS+NS binaries in a very tight orbit with the period shorter than 10~min \citep{2019MNRAS.483.2615K}. Sky-localization may also help disentangle NS+NS systems from others sources by either knowing their position in the Milky Way, or in nearby galaxies, thus enhancing the possibility of EM follow-ups~\cite[e.g.][]{2020MNRAS.492.3061L}. In particular, in addition to differences in chirp masses, it will allow us to distinguish between eccentric NS+NS and eccentric WD+WD systems --- the latter only expected to be formed in globular clusters and ejected into the Galactic halo via dynamical interactions, while the former systems have an eccentricity encoded from the last SN explosion.


\paragraph{BH+NS and BH+BH systems} 

\phantom{text}

For several decades, a number of high-mass X-ray binaries (HMXBs) containing BH accretors have been identified in the Milky Way and nearby galaxies \citep[e.g.\, Cyg~X-1, LMC~X-1, LMC~X-3, MCW~656, M33~X-7, see][]{2019IAUS..346....1V}.
It has been shown that a fraction of these known wind-accreting HMXBs may eventually form BH+BHs or BH+NS systems \citep[][see also Fig.~\ref{fig:BHNS}]{2012arXiv1208.2422B,2013ApJ...764...96B}, while others will merge in an upcoming CE phase (Section~\ref{paragr:CE}), once the companion star evolves to a giant-star size and possibly initiates dynamically unstable Roche-lobe overflow (RLO), depending on its stellar structure and the mass ratio between the two binary components. 
The masses of compact objects in X-ray binaries can be estimated with astrometry and the Galactic stellar-mass BHs are found to have masses between roughly $5-21\;M_{\odot}$ \citep{2019MNRAS.485.2642G,2021MNRAS.502.5455A,2019IAUS..346....1V,2021Sci...371.1046M}. The astrometric satellite Gaia, can also be used to detect optical emission from the HMXB companion stars  \citep{2014arXiv1407.6163B,2017IAUS..324...41K,2017MNRAS.470.2611M,2017ApJ...850L..13B,2018ApJ...861...21Y}. 
Finally, non-interacting binaries with a BH component have also been discovered by combining radial velocity measurements with photometric variability data \citep{2017ApJ...850L..13B,2019Sci...366..637T,2019Natur.575..618L}, although their interpretations can, in some cases, be subject to alternative explanations \citep{2020Sci...368.3282V}. 

The LIGO--Virgo GW detectors have detected BH+BH mergers in distant galaxies, out to $\sim 5\;{\rm Gpc}$. \citep{2020arXiv201014527A}. The inferred BH masses\footnote{Notice, the $2.6\;M_\odot$ compact object in GW190814 might well have been a massive NS rather than a BH.} of their inspiralling BH components potentially range all the way from $\sim 2.6\pm{0.1}\;M_\odot$ \citep{2020ApJ...896L..44A} to $\sim 95\pm{10}\;M_\odot$ \citep{2020arXiv201014527A}, thus significantly more massive than the known Galactic stellar-mass BHs. This difference is mainly attributed to the relatively high metallicity content of the Galaxy \citep{2016Natur.534..512B,2018MNRAS.481.1908K}.
The LIGO--Virgo GW detectors have also identified two sources in close proximity or within the mass ranges expected for BH+NS binaries: GW190426 and GW190814. 
The first event has marginal significance (i.e. a high false-alarm rate, ${\rm FAR}=1.4\;{\rm yr}^{-1}$) and the second is likely to be a BH+BH, not a BH+NS. Nevertheless, 
LISA like LIGO is much more sensitive to the masses (as opposed to matter content) of the binaries, so the presence of similar binaries suggests LISA will copiously find similar sources.

Interestingly enough, although the LIGO--Virgo GW sources are located in distant galaxies at Gpc distances, their low-frequency GWs during the last few years of inspiral prior to the merger event is often so luminous that it allows for detection with LISA \citep{2016PhRvL.116w1102S}. For example, the very first GW source (GW150914) would have been observable by LISA several years before its merger (see Fig.~\ref{fig:UCXB_strain+data}). Similarly, the extreme event GW190521 \citep{2020PhRvL.125j1102A,2020arXiv201006056T}, with a total stellar mass of $\sim 160\;M_\odot$ and located at a distance of about 5~Gpc, would also have been detected during its inspiral in the LISA band. 

\paragraph{Stochastic background}\label{subsec:SGWB}

\phantom{text}

As discussed above, stellar-mass compact binaries (BH+BH, BH+NS, NS+NS) are one of the primary targets for LISA, with expected detection rates of between a few and a few thousands per year, as summarized in Sec\,\ref{subsec:rates}. Nevertheless, many of these sources will not be detected, either because they are too distant and thus have a low SNR, or because the signals from multiple long-lived sources will overlap in time and will be difficult to disentangle. These unresolved signals will combine incoherently and produce a stochastic GW background (SGWB). Current predictions of the amplitude of this background typically rely on the merger rates measured in the local Universe by LIGO-Virgo \citep{2016PhRvL.116m1102A,2018PhRvL.120i1101A}, but since most of the unresolved sources reside at higher redshifts, these predictions depend on the detailed population synthesis and galaxy evolution models. 

The expected amplitude of the SGWB from BH+BH binaries in the LISA band (without source subtraction) varies in the range $\Omega_{\rm GW}(f)\sim 10^{-13}-10^{-11}$ at $f=3$ mHz \citep{2016PhRvL.116w1102S,2016PhRvD..94j3011D,2020MNRAS.493L...1C,2020arXiv200804890P}. Up to a few thousands of these binaries (likely responsible for about $10\%$ of the background) will be individually detected by LISA \citep{2016PhRvL.116w1102S,2020arXiv200804890P}.  The prediction for the background from NS+NS is significantly lower at $\Omega_{\rm GW}(f)\sim 10^{-14}$ at $f=3$ mHz \citep{2020arXiv200804890P}, and the background from BH+NS in the model of \citet{2020arXiv200804890P} is slightly higher but similar to that of NS+NS. The uncertainties on these rates will be significantly reduced in the coming years with more detections of stellar-mass binaries by ground-based detectors, and improved modelling of source formation and evolution. Detection of this background and in particular its shape, will provide important information about the population at periods too short to be directly observed, but before the merger phase probed by ground-based detectors (see Section~\ref{paragr:highFreqGW}).






==> ucb_s2.3_InteractingBinaries.tex <==
\subsubsection{Interacting binaries}\label{subsubsec:interacting-binaries}

\noindent \coord{Shenghua Yu, Thomas Tauris} \\
\noindent \contr{Ashley Ruiter(1.2.3.1), Thomas Kupfer(1.2.3.1), Thomas Tauris(1.2.3.1--2), Gijs Nelemans (1.2.3.1), Shenghua Yu (1.2.3.2)}

\paragraph{AM~CVn binaries (AM Canum Venaticorum binaries --- accreting WDs)}\label{paragr:AM-CVns}

\phantom{text}

AM~CVn binaries consist of a WD accreting from a hydrogen-deficient star (or WD) companion \citep{1995Ap&SS.225..249W,2010PASP..122.1133S}. In their formation history (Fig.~\ref{fig:DWD} and Section~\ref{paragr:DWD-formation}), AM~CVns form after at least one CE phase of their progenitor system. 
The current RLO is initiated, due to orbital damping caused by GW radiation, at orbital periods of typically $5-20\;{\rm min}$ (depending on the nature and the temperature of the companion star), and the mass-transfer rate is determined by a competition between orbital angular momentum loss through emission of GWs and orbital widening due to RLO from the less-massive donor star to the more-massive WD accretor. 

If the system survives the onset of the semi-detached phase, a stable accreting AM~CVn binary is formed in which the orbital separation widens shortly after onset of RLO (Fig.~\ref{fig:UCXB-AMCVn-detailed}), and the system evolves to longer orbital periods (see Fig.~\ref{fig:UCXB-AMCVn-detailed}). When they reach an orbital period of $\sim 60\;{\rm min.}$ (after a few Gyr), the donor star has been stripped down to about 5~Jupiter~masses \citep[$5~M_{\rm J}$,][]{2018PhRvL.121m1105T}. These systems have been hypothesised to be possible progenitors of faint thermonuclear explosions  \citep[flashes, or Type~``.Ia'' SNe,][]{2001A&A...368..939N,2007ApJ...662L..95B}.

Figure~\ref{fig:UCXB_strain+data} shows examples of computed evolutionary tracks of AM~CVn (and UCXB) systems in the characteristic strain amplitude vs GW frequency diagram. As can be seen, AM~CVn systems are indeed anticipated to be detected by LISA --- in some cases even with a ${\rm SNR}>100$ (for the sources located within 1~kpc).

\begin{figure*}
    \begin{center}
  \includegraphics[width=0.60\textwidth, angle=-90]{./img_ucb/UCXB_strain+data.jpg}
\caption{Characteristic strain amplitude vs GW frequency for LISA. Evolutionary tracks are for an UCXB (blue) and an AM~CVn system (magenta) at a distance of $d_{\rm L} = 1\;{\rm kpc}$. Their slope on the inspiral leg is $\propto\, f_{\rm gw}^{7/6}$. The stars along the tracks represent (with increasing GW frequency) onset LMXB/CV stage, termination LMXB/CV stage, and onset UCXB/AM CVn stage. The evolutionary timescales along these tracks are shown in Fig.~\ref{fig:UCXB-AMCVn-detailed}. The LISA sensitivity curve (red line, ${\rm SNR}=1$) is based on four years of observations. The grey curves are for the UCXB at $d_{\rm L} = 15\;{\rm kpc}$ and $780\;{\rm kpc}$ (M31), respectively. Comparison tracks are shown for an MBH merger (green) and GW150914 (orange). Their inspiral slopes are $\propto\, f_{\rm gw}^{-1/6}$. Data from LISA verification sources \citep{2018MNRAS.480..302K} include detached double WD binaries (solid squares), AM~CVn systems (open circles), and a hot subdwarf binary (solid triangle). Figure from \citet{2018PhRvL.121m1105T}.}
 \label{fig:UCXB_strain+data}
  \end{center}
\end{figure*}

Though there are currently $\sim 65$ AM~CVn binaries known in the Galaxy \citep{2018A&A...620A.141R}, their formation pathways are still a puzzle \citep{2018MNRAS.476.1663G}. Their compact orbits and the lack of hydrogen in their spectra, led to three different proposed formation channels: i) the donor is a low-mass (likely He-core) WD \citep{1967AcA....17..287P}; ii) the donor is a semi-degenerate hydrogen-stripped, helium-burning star (e.g. main-sequence helium star, or hot subdwarf); or iii) the donor is a helium-rich core of a main-sequence star that has not undergone helium-burning since it had a rather low mass to begin with \citep[see][]{2010PASP..122.1133S}. Further discussions on their formation is given in Section~\ref{paragr:DWD-formation}. 

Only for eclipsing AM~CVns is it possible to fully determine all binary parameters and put constraints on the donor type. Recent results from eclipsing systems revealed that the donor stars are likely larger and more massive than previously assumed \citep{2011MNRAS.410.1113C,2018A&A...620A.141R}, implying that a semi-degenerate donor is more likely for such systems, unless the donor star is a low-mass He-core~WD which can remain bloated on a Gyr timescale \citep{2014A&A...571L...3I}. If that is the norm rather than the exception, it will lead to more AM~CVn GW sources than previously predicted.

Based on binary population synthesis, \citet{2001A&A...368..939N} predicted a space density of AM~CVn stars in a range of $0.4-1.7\times10^{-4}\;{\rm pc}^{-3}$ and a number of resolvable AM~CVn systems for LISA roughly equal to the number of detached WD+WDs \citep{2004MNRAS.349..181N}. More recently, \cite{2017ApJ...846...95K} predicts that $\sim 2700$ systems will be observable by LISA with a negative chirp of $0.1\;{\rm yr}^{-2}$ (i.e. $\dot{f}_{\rm gw}<0$, resulting from orbital expansion due to mass transfer, see Figs.~\ref{fig:UCXB_strain+data} and \ref{fig:UCXB-AMCVn-detailed}). Until very recently, when ZTF reported a large number of eclipsing WD+WDs \citep{2019Natur.571..528B, 2020arXiv201003555B}, the majority of known LISA verification binaries was dominated by AM~CVn systems \citep{2007ApJ...666.1174R,2010ApJ...711L.138R,2015MNRAS.453..483K,2018MNRAS.477.5646G,2018MNRAS.480..302K}. However, observational space density estimates from SDSS data are in strong disagreement with theoretical predictions from these binary population studies. \citet{2007MNRAS.382..685R,2013MNRAS.429.2143C} derived an observed space density about an order of magnitude below the prediction by \cite{2001A&A...368..939N,2017ApJ...846...95K} which would result in only $\lesssim1000$ resolvable systems in the LISA band. The discrepancy could be real with the population synthesis predicting too many systems, related to assumptions in binary evolution physics (especially the treatment of mass transfer in close binaries), and/or possibly because some of the systems that are predicted to evolve into AM~CVn binaries in fact merge in a CE shortly after the less-massive star fills its Roche lobe. On the other hand, it could also be that AM~CVn stars are more difficult to find than expected (when not in outburst) or that they are distributed with relative high concentration in the thick disc \citep{2012ApJ...758..131N}. \citet{2018A&A...620A.141R} argued, based on Gaia data release 2 parallaxes, that a significant fraction of AM~CVn systems, even within 100~pc, could still be undiscovered. Future transient sky surveys, such as LSST using the Vera~C.~Rubin Observatory, could have great success in detecting short-period binary systems with the implementation of appropriate cadence intervals (e.g. very short, $\sim 15\;{\rm s}$ sub-exposures). Indeed already some AM~CVn systems are thought (or known) to be eclipsing \citep{2020ApJ...905...32B}. 

Nonetheless, AM~CVn binaries are expected to be extremely useful for LISA because they simultaneously provide EM information across different wavelengths, as well as being observable in LISA's GW frequency range. For this reason, AM~CVn systems have been cited as being important verification sources for LISA \citep[e.g.][]{2018MNRAS.480..302K}. In other words, AM~CVn binaries will be multi-messenger sources once LISA flies. See Section~\ref{subsec:synergies} for further discussion on the multi-messenger opportunities for LISA.



\paragraph{UCXBs (ultra-compact X-ray binaries)}\label{paragr:UCXBs} 

\phantom{text}

It has been known for many years that tight-orbit post-LMXB systems, leaving behind a NS+WD binary that spirals-in due to GW radiation, may avoid a catastrophic event, once the WD fills its Roche lobe. The outcome is expected to be a long-lived UCXB \citep[][]{1979ApJ...227..178W,1986ApJ...304..231N,2002ApJ...565.1107P,2010MNRAS.401.1347N,2012A&A...537A.104V,2013ApJ...768..184H}.      
These sources are tight X-ray binaries observed with an accreting NS and a typical orbital period of less than 60~min. 
Because of the compactness of UCXBs, the donor stars are constrained to be either a WD, a semi-degenerate dwarf or a helium star \citep{1982ApJ...254..616R}.
UCXBs are not only excellent laboratories for testing binary-star evolution, but also important GW sources. Studies of their orbital parameters (mass, orbital period and eccentricity), chemical composition and spatial distribution may provide important information and clues to understand both the accretion processes of compact binaries (including spin-orbit and tidal interactions) and the long-term evolution of double compact object binaries.

Depending on the mass-transfer rate, the UCXBs are classified in two categories: persistent and transient sources \citep[e.g.][]{2013ApJ...768..184H}. Only about 14~UCXBs have been confirmed so far (9~persistent, 5~transient), and an additional $\sim 14$~candidates are known. 
Thus UCXBs are difficult to detect or represent a rare population. Earlier studies \citep[e.g.][]{2014A&A...571A..45I} have suggested the need for extreme fine tuning of initial parameters (stellar mass and orbital period of the LMXB progenitor systems) in order to produce an UCXB from an LMXB system.
UCXBs are detected with different chemical compositions in the spectra of their accretion discs \citep[e.g. H, He, C, O and Ne, see][]{2010MNRAS.401.1347N}. To explain this diversity requires donor stars which have evolved to different levels of nuclear 
burning and interior degeneracy, and therefore to different scenarios for the formation of UCXBs.
Since a large fraction of the UCXBs are found in globular clusters, some of these UCXB systems could also have formed via tidal captures, direct collisions or stellar exchange interactions \citep{1975MNRAS.172P..15F,1975A&A....44..227S,1983ApJ...268..319H}. 

Figure~\ref{fig:UCXB-AMCVn-detailed} displays the evolution of AM~CVns and UCXBs in the GW frequency vs dynamical chirp mass diagram. These systems undergo stable RLO and will start to widen their orbits again within a few Myr after the onset of the mass transfer. LISA will detect such Galactic systems continuously both during the inspiral phase for a few tens of Myr, while the systems are still detached, and after the onset of RLO on a timescale of up to 100~Myr (depending on their distance). 

The long-term stability of UCXBs has been a topic of debate. From an analytical investigation, \citet{2012A&A...537A.104V} argued that for a $1.4\;M_{\odot}$ NS accretor, only C/O-core~WDs with a mass of $\lesssim 0.4\;M_{\odot}$ lead to stable UCXB configurations. Subsequent hydrodynamical simulations suggested that this critical WD mass limit could be lower \citep{2017MNRAS.467.3556B}. The first successful numerical calculations of RLO from a WD to a NS were presented by \citet{2017MNRAS.470L...6S}, and they were able to follow the entire evolution until the low-mass He-core~WD donor star has become a $\sim 0.005\;M_\odot$ planet-like companion. These systems were further evolved \citep{2018PhRvL.121m1105T}, including the finite-temperature (entropy) effects of the WD donor stars, and the first evolutionary tracks of such sources across the LISA GW band were produced, see e.g. Figs~\ref{fig:UCXB_strain+data} and \ref{fig:UCXB-AMCVn-detailed}. Further independent studies on the detectability of UCXBs as LISA sources have been provided by e.g. \citet{2020ApJ...900L...8C,2021MNRAS.503.2776Y}.

It is also anticipated that LISA may detect interacting BH+WD systems \citep{2017MNRAS.467.2199B,2020arXiv201005974S}. It has been estimated in some studies \citep{2006A&A...454..559Y} that the Galaxy contains some $10^4$ of these systems. However, their formation process (especially those with low-mass WD companions) remains uncertain \citep{2003MNRAS.341..385P}.

\begin{figure*}
    \begin{center}
  \includegraphics[width=0.60\textwidth, angle=-90]{./img_ucb/UCXB_Mchirp_f-gw_3models.pdf}
\caption{GW frequency vs dynamical chirp mass for an UCXB and two AM~CVn systems, based on detailed mass transfer calculations (including finite-temperature effects of the WD donor star) using the MESA code \citep{2018PhRvL.121m1105T}. The end points of the first mass-transfer phases (LMXB and CV) are indicated by red triangles; the starting points of the second mass-transfer phases (UCXB and AM~CVn) are indicated by green circles. The time marks along the AM~CVn tracks are for the same values as indicated for the UCXB system, unless stated otherwise (in Myr). Time zero is defined at the onset of the second mass-transfer phase. The maximum GW frequencies (strongest LISA signal) in these three examples are 5.45~mHz (UCXB), 5.64~mHz (AM~CVn1), and 5.72~mHz (AM~CVn2) corresponding orbital periods of 6.12~min, 5.91~min and 5.83~min, respectively. The frequency at the onset of the RLO (green circles) depends on the temperature of the low-mass He~WD donor ($T_{\rm eff}$\,=\,10\,850~K, 9\,965~K and 8\,999~K, respectively).}
 \label{fig:UCXB-AMCVn-detailed}
  \end{center}
\end{figure*}




==> ucb_s2.4_OtherSources.tex <==
\subsubsection{Other potential sources}\label{subsubsec:other_sources}

\noindent \contr{Camilla Danielski(1.2.4.1-2), Silvia Toonen(1.2.4.2), Thomas Kupfer(1.2.4.4), Jan van Roestel (1.2.4.3), Nicola Tamanini (1.2.4.1), Valeriya Korol (1.2.4.1)}

\paragraph{Helium-star binaries}

\phantom{text}

Subdwarf B~stars (sdBs) are stars of spectral type B with luminosities below that of main-sequence stars. The formation mechanism and evolution of sdBs are still debated, although most sdBs are likely He--burning stars with masses $\sim 0.5\;M_\odot$, radii as small as $\sim 0.1\;R_\odot$ and thin hydrogen envelopes \citep{2016PASP..128h2001H}. A large fraction are found in binary systems and, due to their compact nature, the most compact ones have orbital periods $\lesssim\,1$\,hr \citep{2012ApJ...759L..25V,2013A&A...554A..54G,2017ApJ...851...28K,2020ApJ...891...45K,2020ApJ...898L..25K}, making them potentially detectable sources for LISA. 

The most compact systems have WD companions and as such they are prime progenitor systems for double detonation Type~Ia~SNe. In this scenario a WD is orbited by a core He-burning sdB~star in an ultra-compact orbit ($P_{\rm orb}<80\;{\rm min}$). Due to the emission of GWs, the binary shrinks until the sdB~star fills its Roche lobe and starts mass transfer. He-rich material is then transferred to the C/O-core WD companion which will lead to the accumulation of a He-layer on top of the WD. After accreting about $0.1\;M_\odot$, He-burning is predicted to be ignited in this shell. This in turn triggers the ignition of carbon in the core, even if the WD~mass is significantly lower than the Chandrasekhar limit \citep{2010A&A...514A..53F}. So far, the only known candidate for this scenario is the ultra-compact sdB+WD binary CD$-$30$^\circ$11223 with an orbital period of $P=71\;{\rm min}$ \citep{2012ApJ...759L..25V,2013A&A...554A..54G}. 
This system was also found to be detectable for LISA with an expected SNR of $\sim 5$ after four years of LISA observations \citep{2018MNRAS.480..302K}. More recently, the first members of ultra-compact sdB binaries which have started to transfer material to the WD companion were discovered. The most compact system, ZTF\,J2130+4420, consisting of a low-mass sdB~star with $M_{\rm sdB}=0.337\;M_\odot$ has an orbital period of 39~min. The system has well measured properties from EM observations and is expected to have a SNR of $\sim 3$ after four years of LISA observations, adding to the growing number of LISA detectable He-burning stars.

\citet{2020arXiv200607382G} modelled the Galactic population of stripped stars, which contain the low-mass sdB~stars as well as more massive He-core burning stars, in tight orbits with compact companions, focusing on those that will be detectable by LISA. Their analysis predicts up to 100 stripped star + WD binaries and up to 4 stripped star + NS binaries with ${\rm SNR}>5$ after 10 years of observations with LISA. Although the expected numbers are significantly smaller than for WD+WDs or AM~CVns, \citet{2020arXiv200607382G} finds that all of the LISA detectable sources are within 1~kpc and therefore bright in EM flux which makes them ideal targets for multi-messenger studies (see Section~\ref{subsec:synergies} for more details on multi-messenger opportunities). 

\paragraph{Period bouncing CVs} 

\phantom{text}

Period bouncing CVs are highly evolved cataclysmic variables where the donor has lost almost all of its mass and has become degenerate. These systems have reached the minimum orbital period for a hydrogen donor (70~min) and are evolving to longer orbital periods (up to 100~min). Model predictions are that 40--70\% of all CVs are period bouncers \citep{1993A&A...271..149K,2011ApJS..194...28K}. However, only a few have been identified so far because of the low accretion rate and low temperature of the WD and donor \citep[e.g.][]{2018MNRAS.481.2523P}. 
While the donor-mass is low and the orbital periods are relatively long, nearby period bouncers are detectable with LISA. Given their high space density, a dozen of these systems are close enough to be detected by LISA.


\paragraph{Exoplanets, brown dwarfs and substellar companions} %

\phantom{text}

In the Galaxy, due to the slope of the Salpeter-like initial mass function (IMF), more than 97\% of all stars will terminate their lives as a WD, meaning that the vast majority of the known 4000+ planet-hosting stars will end their lives as WDs. 
In the last couple of decades, most of the attention in exoplanetary searches has been focused on the formation and characterisation of exoplanets orbiting host stars on the main sequence, but very little is known on planetary systems in which the host star evolves off the main sequence, to become a red giant. 
Theoretical models indicate that, if planets avoid engulfment and evaporation throughout the red-giant or/and the asymptotic-giant branch phases of the host star, they can survive \citep[see e.g.][]{1984MNRAS.208..763L,1998Icar..134..303D,1998A&A...335L..85N}. This is expected to be the fate of the planet Mars, and other planets orbiting further out in our Solar System \citep{2008MNRAS.386..155S}.
Observational evidence, in the form of photospheric contamination by the accreted debris \citep{2010ApJ...722..725Z,2014A&A...566A..34K}, dusty \citep{2009ApJ...694..805F} and gaseous circumstellar discs \citep{2006Sci...314.1908G,2016MNRAS.455.4467M}, supports the existence of dynamically active planetary systems around WDs. Up to very recently, only two planetesimals had been observed orbiting a WD \citep{2015Natur.526..546V,2019Sci...364...66M}. However, within the last years, two giant planets have been detected orbiting single WDs \citep{2019Natur.576...61G,2020Natur.585..363V}, 
showing that planets can survive single host-star evolution. 

Today, over 1000 brown dwarfs (BDs) have been detected in the Solar neighbourhood \citep{2018haex.bookE.118B}. 
Some of them have been discovered also around single WDs, and examples of BDs orbiting at distances beyond the tidal radius of the asymptotic-giant branch progenitor \citep[but also within it, e.g.\,WD~0137$-$349~B,][]{2006Natur.442..543M}, show that BDs can survive stellar evolution of their host star, whether or not they are engulfed by its expanding envelope. \citet{2005ApJS..161..394F} predicted that few tenths of percent of Galactic single WDs hosts a BD.

The most straightforward way with which LISA could detect sub-stellar objects, such as planets or BDs, would be the direct detection of GWs emitted by a binary system composed of a sub-stellar object in an tight orbit around a single star. 
However, the absolute orbital period minimum for a hydrogen-rich body (i.e. a star, BD or a gas giant planet) in a binary system is about $P_{\rm orb}\simeq 37\;{\rm min}$ \citep{2021arXiv210412083R}. This corresponds to a GW frequency of at most $f_{\rm GW}\simeq 0.9\;{\rm mHz}$.
Such a system could be detected only at close distances (say, within 1~kpc) and only for relatively high sub-stellar masses ($M\gtrsim 13\;M_{\rm J}$), possibly excluding all exoplanets.  Furthermore, the mass of the sub-stellar object cannot be directly inferred from direct detection, and at best only the chirp mass of the binary system can be retrieved.
Further investigations and EM observations are necessary to better understand the detectability and the rates of these sub-stellar objects, although at the moment it seems unlikely that a large number of these systems will be observed by LISA \citep{2019MNRAS.483L..33W}.

Another option is to search for circumbinary planets around WD+WD through a modulation of the WD+WD signal \citep{2019NatAs...3..858T}, that can probe regions of parameter space not probed by EM observations (far away and not towards the Galactic Centre).
The discovery of evolved planetary systems will statistically increase the current sample of post-main-sequence planets, filling an area of the planetary Hertzsprung--Russell diagram that is currently not explored  \citep{2019NatAs...3..858T}. LISA will provide observational constraints on both planets that can survive two CE stellar evolution phases and on a possible second-generation planet population produced from CE ejecta material \citep{2014A&A...563A..61S}. 
Even in the case where LISA will prove no detection anywhere in the Milky Way, it will be possible to set strong unbiased constraints on planetary evolution and dynamical theories, and in particular on the fate of exoplanets bound to a binary that undergoes two CE phases.


\paragraph{Triples and multiples}\label{paragr:triples} 

\phantom{text}

LISA's stellar sources will also contain multiple body systems, such as triples and quadruples. 
Hierarchical systems that consist of nested orbits represent stable configurations that can remain intact for several Gyr and throughout (despite) the evolution of the stellar components, as evidenced by observations.  
Within 20~pc of the Sun, there are already two such systems that harbor close WD+WDs. These are 
WD~0326$-$273 \citep{1949ApJ...109..528L,1994RMxAA..28...43P,2005A&A...440.1087N,2012ApJS..199...29G,2017A&A...602A..16T} and 
WD~0101+048 \citep{1998ApJ...502..394S,2000MNRAS.319..305M,2009A&A...507..251C,2012ApJS..199...29G,2017A&A...602A..16T}. 
The former is a triple that consists of a close WD+WD with a period of $\sim 1.8\;{\rm d}$, and an M5 star in a wide orbit. The latter is a quadruple consisting of a close WD+WD (with a period of $\sim1.2\;{\rm d}$, but see \citep{2000MNRAS.319..305M} and a MS+MS binary. 
Two triple systems with \textit{three} WD components are known as well, J1953$-$1019 \citep{2019MNRAS.483..901P} and WD~1704+481 \citep{2000MNRAS.314..334M}. The inner binary of the latter system has a period of $\sim0.15\;{\rm d}$, just inside the LISA frequency range.  
Even millisecond pulsars have been found to be part of triple-architectures; 
the PSR~J0337+1715 system harbors a compact NS+WD (1.6~d orbital period) inner binary which is orbited by another (tertiary) WD every 327~d \citep{2014Natur.505..520R,2014ApJ...781L..13T}. The globular cluster (M4) pulsar B1620$-$26 has a WD companion in a half-year orbit, and a planetary companion in a 100-yr orbit \citep{1999ApJ...523..763T,2003Sci...301..193S}. 

Theory suggests that exoplanets (and BDs) also exist around WD+WDs in the Galactic disc, and that such objects are more likely to survive around evolving close binary stars than around evolving single stars \citep{2016ApJ...832..183K}. The eclipse timing variation technique allowed the detection of a few post-CE systems (that is WD+low-mass star), and a BD companion(s) \citep[see e.g.][]{2015MNRAS.448.1118G, 2012A&A...543A.138B, 2019AJ....157..150A}, nevertheless today no BDs or exoplanets orbiting WD+WDs have been observed yet. 

LISA will be able to detect outer companions to compact (inner) binaries when they impose eccentricity oscillations in the inner orbit due to three-body dynamics \citep{1910AN....183..345V,1962P&SS....9..719L,1962AJ.....67..591K,2016ARA&A..54..441N}. In particular \citet{2019ApJ...875L..31H} showed such oscillations would be observable with LISA to distances up to a few Mpc for compact binaries near supermassive BHs, which can also be considered a three-body system.  Furthermore, LISA can detect outer companions by exploiting the Doppler frequency modulation on the GW waveform due to their gravitational pull  \citep{2018PhRvD..98f4012R}. 
The acceleration imparted by the hierarchical companions can be detected in the GW signal for outer periods as large as 100~yr \citep{2018PhRvD..98f4012R, 2020PhRvD.101f3002T}. 
For systems with orbital periods that are shorter than, or comparable to, the mission lifetime, the perturbation allows for the determination of the orbital period, eccentricity, initial orbital phase and radial velocity parameter of the companion \citep{2018PhRvD..98f4012R,2019NatAs...3..858T}. 
On a general level, the sensitivity of LISA will be able to detect WD+WDs companions with masses down to $\sim M_{\rm J}$
\citep{2019A&A...632A.113D}, and therefore allow not only for the detection of stellar companion and compact objects, but also BDs and exoplanets. This being an indirect detection, i.e.\,the observation of a periodic Doppler shift modulation of an existing strong binary GW signal, we are able to probe a wider mass range, whose inferior limit also covers the giant planets range. The novelty of using LISA for the detection of planetary/low-mass companions is that GWs provide a much larger spatial coverage than the one provided by EM techniques, enabling us to probe regions of our Galaxy currently not accessible to other methods.
More specifically, \cite{2019A&A...632A.113D} showed that during a 4~yr nominal mission LISA will detect from 3 to 83 exoplanets, and from 14 to 2218 BDs everywhere in the Milky Way. The sensitivity of LISA is such that in the most optimistic cases exoplanets could be detected orbiting WD+WDs in the Milky Way's satellites, in particular in the Large Magellanic Cloud \citep[LMC,][]{2020arXiv200707010D}. Such an observation could represent the first detection of an extra-galactic bound exoplanetary system.


\paragraph{Capturing the inspiral of a CE system}\label{paragr:other-interacting} 

\phantom{text}

It has been suggested by \citet{2021arXiv210200078R} that LISA may be able to detect the inspiral of binaries undergoing a CE phase. Depending on various assumptions, they anticipate that LISA could detect between 0.1 and 100 such GW sources in the Galaxy during the mission duration. Detecting this GW signal would provide direct insight into the gas-driven physics of CE evolution.



==> ucb_s4_Rates.tex <==

\subsubsection{Binary's detectability}
{\color{blue}
The detectability of Galactic stellar binaries with LISA
primarily depends on the parameters involved in the GW amplitude:
\begin{equation} \label{eqn:amp}
    {\cal A} = \frac{2(G{\cal M})^{5/3}(\pi f)^{2/3}}{c^4 d},
\end{equation}
where $f$ is the binary's GW frequency, ${\cal M}={(m_1 m_2)^{3/5}}/{(m_1+m_2)^{1/5}}$ is the chirp mass (with $m_1$ and $m_2$ being the primary and secondary masses), $d$ is the luminosity distance, $G$ and $c$ are respectively the gravitational constant and the speed of light. This follows from the fact that the signal-to-noise ratio scales linearly with amplitude $\rho \propto {\cal A} \sqrt{T}$ with $T$ being the observation time \citep{2021arXiv210801167B}.
Besides, in contrast with electromagnetic observations, the observed GW signal scales as $1/d$, rather than $1/d^2$.

The GW frequency, defined as $f=2/P$ with $P$ being the binary's orbital period, has the strongest impact on the signal's detectability. Binaries emitting at $f>3\,$mHz fall in the most sensitive part of the LISA frequency band \citep{2017arXiv170200786A}. As a result, these high-frequency binaries -- even if consisting of the lowest mass WD components -- can be detected across the Milky Way also reaching satellite galaxies (cf. Figures~\ref{fig:horizons} and \ref{fig:MW}). At a set frequency, the maximum distance at which the binary can be detected increases with its chirp mass, as shown in Figure~1.1. In addition, the chirp mass defines how fast the GW frequency changes during the in-spiral phase. This so-called chirp is given by
\begin{equation} \label{eq:fdot}
\dot{f}=\frac{96}{5}  \pi^{8/3} \left( \frac{G{\cal M}}{c^3} \right)^{5/3} f^{11/3}.
\end{equation}
The chirping rate for stellar binaries in the LISA band is generally very slow ($\dot{f} < 10^{-15}$\,Hz$^2$ for typical WD+WD and NS+NS binaries emitting at frequencies lower than a few mHz).
Note that the frequency derivative (not the chirp mass) can be measured directly from GW data. The measurements is possible for binaries emitting at sufficiently large frequencies ($f > 3\,$mHz, \cite{2020ApJ...894L..15R}), such that during the observation time ($T$) with LISA the binary sweeps through at least a few frequency bins ($1/T$) . If $\dot{f}$ is measured and assuming that the inspiral is driven by radiation reaction only, the luminosity distance can be recovered by plugging in the measured value of the chirp mass into Eq.\eqref{eqn:amp}. At lower frequencies, binaries will be effectively ``seen'' by LISA as monochromatic. In which case, only measurements of $f$ and ${\cal A}$ will be possible, while the chirp mass estimate will be degenerate with that of the distance (cf. Eq.~\ref{eqn:amp}). 

Unlike circular binaries, eccentric ones emit GWs at multiple harmonics. Each signal can be thought as a collection of $n$ signals from circular binaries emitting at $f_n = n f/2$ and the amplitude ${\cal A}_n={\cal A}(2/n)^{5/3} g(n,e)^{1/2}$, where $g(n,e)$ is given in Peters \& Mathews (1963). The total signal-to-noise ratio can be estimated as the quadrature sum of the individual harmonics' signal-to-noise ratios. %Thus, under the assumption of the optimal GW signal recovery, the signal-to-noise of an eccentric binary is always greater than that of a circular one. 
Thus, to measure the chirp mass in case of the eccentric binary, in addition to $\dot{f}$, one needs to simultaneously measure the eccentricity. This is possible when at least two harmonics are detected \citep[e.g.][]{2016MNRAS.460L...1S}, otherwise only an upper limit on the chirp mass can be derived.

Another aspect of Galactic binaries' detectability is that they will be observed continuously during the course of the mission. However, it is likely that the measurements will undergo occasional interruptions due to communication antenna re-pointing or spacecraft housekeeping. Additionally, spurious disturbances may affect the interferometer signals, such as the transient glitches observed in LISA Pathfinder \citep{2022arXiv220511938L, 2022PhRvD.105d2002B}, leading to corrupted data spans. These operating conditions may impact the duty cycle of the mission, with a minimum requirement of 89\% at the time of writing. If the masking events are frequent, they could impact the detection of low-frequency sources (around 0.1 mHz and below). However, mitigation techniques have been developed and show promising results for restoring the optimal detectability \citep{2019PhRvD.100b2003B,2022MNRAS.509.5902B}.
}

\subsubsection{Detection and parameter estimation expectations}
{\color{blue}It is expected that the Galactic stellar binaries will dominate the number of individually detected GW sources at mHz frequencies (Table~\ref{tab:absolute_n_MWG}). Out of $\sim\mathcal{O}(10^7)$ stellar binaries emitting in the LISA frequency band, LISA is expected to deliver $\sim\mathcal{O}(10^4)$ individual detections \citep[e.g.][]{2020PhRvD.101l3021L, 2021PhRvD.104d3019K}.
Current estimates suggest that at frequencies $>3\,$mHz, Galactic WD+WD detectable by LISA will be counted in thousands, NS+NSs in few up to hundreds and BH+BHs in a few (see Tables \ref{tab:absolute_n_MWG} and \ref{tab:absolute_n_MWG_GC}). At frequencies $<3\,$mHz the number of stellar binaries is so large, that only a small fraction - the closest and more massive ones - will be individually detected, while the rest of the population will form an unresolved stochastic foreground (see Section~\ref{subsubsec:GWforeground}).

Amongst the resolvable systems, population synthesis simulations suggest that hundreds will be exceptionally strong LISA sources \citep[e.g.][]{2021PhRvD.104d3019K}. These binaries will be detectable within weeks from the start of mission operations, and over the full mission lifetime can accumulate SNRs up to $10^3$.
Based on an SNR evaluation via an iterative scheme for the estimate of the confusion foreground generated by Milky Way’s GW sources \citep[e.g.][]{2020PhRvD.101l3021L,2021PhRvD.104d3019K}, synthetic population analysis \citep[e.g.][]{2017MNRAS.470.1894K, 2019MNRAS.490.5888L} yields about up to $10^4$ binaries detectable with SNR$>20$, several $10^3$ with SNR$>100$, a few with SNR$>1000$. For all binaries, frequencies predicted be measured very accurately with $\sigma_{\rm f}/f < 10^{-5}$, which corresponds to $\sigma_{\rm P}<0.025$\,ms for a typical mHz WD+WD binary. Frequency derivative is estimated to be measured to better than 30\% for up to $10^4$ binaries, leading to the measurement of the chirp mass via Eq.~\eqref{eq:fdot}. Consequently, also distances can be derived to better than 30\% for several $10^3$ binaries. The sky localisation uncertainty depends strongly on the SNR and GW frequency ($\propto \rho^{-2}f^{-2}$). Additionally, it is also dependent on the ecliptic latitude: a source on the ecliptic has an order of magnitude more uncertainty than a source at the poles \citep{2020ApJ...894L..15R}. On average, sky localisation error for Galactic WD+WD systems is expected to be of several deg$^2$, improving with increasing GW frequency and SNR down to sub-square degree precision and below. These expectation are well supported by Bayesian-based data analysis exercises \citep{2020PhRvD.101l3021L} with mock data simulating observations over one year, and including 30 millions of injected Galactic sources. Consolidation of these results are expected once more realistic data simulations featuring mixed source types are analysed (see https://lisa-ldc.lal.in2p3.fr).}





Beyond the Milky Way, the Local Group galaxies are expected to harbour from a few to a few hundreds LISA sources (mainly WD+WDs and some NS+NSs) depending on the total mass and the distance of the galaxy \citep{2019MNRAS.489.4513S, 2020ApJ...892L...9A,2020A&A...638A.153K,2020MNRAS.492.3061L} (see Fig.~\ref{fig:horizons}). For instance, the number of WD+WDs and NS+NS in the largest Milky Way satellites, the Large and Small Magellanic Clouds, will be high enough to overcome Galactic foreground and to unambiguously identify these galaxies in the LISA data \citep{2020ApJ...894L..15R}. Even further away, with the total mass comparable to the Milky Way's mass, the Andromeda galaxy could also be visible on the LISA sky as a group of GW sources \citep{2018ApJ...866L..20K}. 

The outside limits of the Local Group, LISA can access distances up to $\sim 1\,$Gpc through GW signal from stellar-mass BH+BHs, which will ultimately be observable during merger to ground-based detectors (see Section~\ref{paragr:highFreqGW}).
Studies based on cosmological simulations of galaxies at $z=0$ find that the present-day dwarf galaxies can accommodate a larger BH+BH merger rate compared to massive galaxies \citep{2017MNRAS.464.2831O}. Specifically, for massive BH+BHs similar to GW150914, about $40\%$ of mergers are expected to be in galaxy progenitors of Milky Way-like systems and the rest in smaller satellite or isolated dwarf galaxies \citep{2019MNRAS.484.3219M}. This translates into a large number of potential hosts within the estimated LISA horizon distance. Not only BH+BHs formed from the evolution of isolated binaries, but also BH+BHs formed in extragalactic globular clusters may  be detectable by LISA, with initial studies predicting the number of such sources to be in the range of 1 -- $10^2$ \citep{2018PhRvL.120s1103K}.

{\color{blue} Given LISA's selection effects, extra-galactic LIGO-like BH+BH are expected to have quite low signal-to-noise ratios ($\sim 10$). For this class of stellar binaries, \cite{2021PhRvD.104d4065B} report sky localisation errors of a few tens of squared degrees and constrains on the detector-frame chirp mass down to $\pm 0.01$\,M$_\odot$. They also show
that at 10\,mHz the eccentricity for these binaries can be measured down to $10^{-3}$, while the merger time can be determined within a time window of 1\,hour.}


For sources that form through isolated binary evolution, the rates (such as those mentioned above and in Table~\ref{tab:absolute_n_MWG}) are often estimated with the population synthesis approach.
There are many uncertainties that affect the rate calculations. These uncertainties can be divided in five broad categories: (i) binary evolution physics (e.g., CE evolution, mass transfer stability, mass-accretion efficiency, etc.), (ii) stellar evolution physics (e.g., metallicity dependent stellar winds, core-collapse mechanisms, natal kicks, pair-instability SN and pulsational pair instability, etc.), (iii) initial stellar and binary properties (e.g., initial mass function, binary fraction, initial distribution of separation, mass ratio, eccentricity, etc.), (iv) different assumptions for the Galactic spacial distribution (thin/thick disc and bulge) and star-formation history  and (v) LISA selection effects (e.g., GW foreground, mission length, sensitivity curve and SNR detection threshold).



As discussed in Section~\ref{subsubsec:cluster-sources}, LISA sources may also form dynamically in dense stellar environments such as globular clusters (and may have markedly different features compared to sources that form through isolated binary evolution, Section~\ref{subsubsec:isolated-binaries}). In Table \ref{tab:absolute_n_MWG_GC}, we show the estimated number of sources expected to be found in globular clusters in a Milky Way-like galaxy \citep{2018PhRvL.120s1103K}. The number of detectable LISA BH+BHs originating from young massive clusters and open clusters is expected to be several tens to $\sim$100 \citep[or about $0.5\text{--}3$ times the density of those clusters in the local volume in units of Mpc$^{-3}$;][]{Banerjee2020}. Merger rate estimates for GW sources produced in dynamical environments from cluster simulations, can also be influenced by many uncertain physical processes, some of which are common to the ones outlined for sources formed via isolated binary evolution. For instance, natal kicks for compact objects have a direct impact on retention of those objects in stellar clusters \citep{2013ApJ...763L..15M,2018MNRAS.479.4652A,2018MNRAS.474.3835W,2018A&A...617A..69P,2020A&A...639A..41B} which influences the number of dynamically formed binary systems. The number of compact objects that form in dense environments also depends on their metallicity and the initial mass function of their stars which may vary with their formation environment  \citep{2009MNRAS.394.1529D,2013ApJ...771...29G,2014PhR...539...49K,2020A&A...636A..10C}. Additionally, dissolved or tidally disrupted open and globular clusters can also contribute to the number of GW sources that may have dynamically formed \citep{2010ApJ...718.1266M,2018ApJ...856...92F,2019MNRAS.487.2412G}.



Apart from population synthesis-like simulations, another approach to predict the expected LISA rates is to derive empirical estimates from the already observed population of sources. For NS+NSs for instance, one can use the inferred merger rate coming from the known Galactic NS+NS population, and accounting for survey selection effects \citep{1991ApJ...380L..17P, 2003ApJ...584..985K}, or the inferred merger rate from LIGO--Virgo \citep{2020arXiv201014533T}, to predict that LISA should be able to detect $50\text{--}300$ NS+NSs in the Milky Way \citep{2020ApJ...892L...9A}. In a similar manner, based on O1 LIGO--Virgo detections, it was estimated that LISA maybe able to detect up to $\sim 50$ BH+BHs \citep{2016PhRvL.116w1102S}, but the inferred BH+BH merger rate density decreased in the most recent O3 run by a factor of $\sim 2$. Empirical estimates of the Galactic NS+WD population have been derived, based on the observed pulsar population, with $100-150$ being predicted to be observable by LISA \citep{2018PhRvL.121m1105T}. 















\begin{table}
\centering                          % used for centering table
\begin{tabular}{c | c c }        % centered columns (4 columns)
\hline
%Source & $N \, \mathrm{[MW^{-1}]}$ & $N^\mathrm{detected} \, \mathrm{[MW^{-1}]}$ \\
Source & $N$ & $N^\mathrm{detected}$ \\
\hline
    WD+WD & $\sim 10^8$  & 6,000$-$10,000  \\
    %\cite{2012ApJ...758..131N}\cite{2017MNRAS.470.1894K,2019MNRAS.490.5888L,2018ApJ...866L..20K,2010ApJ...719.1546L,2010ApJ...717.1006R}
    NS+WD & $\sim 10^7$  & 100$-$300  \\
    %\cite{2020ApJ...898...71B}\cite{2018PhRvL.121m1105T,2020ApJ...898...71B}
    BH+WD & $ \sim 10^6$  & 0$-$3  \\
    %\cite{2020ApJ...898...71B}\cite{2020ApJ...898...71B}
    NS+NS & $\sim 10^5$  & 2$-$100  \\
    %\cite{2010ApJ...725..816B,2018MNRAS.481.1908K,2020ApJ...898...71B}\cite{2010ApJ...725..816B,2018MNRAS.481.1908K,2020MNRAS.492.3061L,2020ApJ...892L...9A,2020ApJ...898...71B}
    BH+NS & $\sim 10^4 - 10^5$  & 0$-$20  \\
    %\cite{2010ApJ...725..816B,2018MNRAS.481.1908K,2020ApJ...898...71B}\cite{2010ApJ...725..816B,2018MNRAS.481.1908K,2020ApJ...898...71B}
    BH+BH & $\sim 10^6$  & 0$-$70  \\
    %\cite{2010ApJ...725..816B,2018MNRAS.481.1908K,2020ApJ...898...71B,2018MNRAS.480.2704L}\cite{2010ApJ...725..816B,2018MNRAS.481.1908K,2020MNRAS.494L..75S,2020ApJ...898...71B}
\hline
\end{tabular}
\caption{Estimated absolute number of compact binaries from \textit{isolated binary evolution} in the Milky Way. The columns show the source type, the total number of binaries in the galaxy at any frequency and the total number of estimated sources detected by LISA. We report values from indipendent studies which assume different LISA mission lifetimes and SNR. WD+WD models assume a frequency range $0.5-10$~mHz while models for the other sources assume a frequency range $0.1-10$~mHz. At lower frequencies the total number of LISA sources is so high that it might become impossible to distinguish individual sources from the GW foreground. The ranges of the expected intrinsic number of each binary type are extracted from \cite{2012ApJ...758..131N, 2020ApJ...898...71B, 2010ApJ...725..816B, 2018MNRAS.481.1908K, 2001A&A...365..491N, 2014A&A...569A..42V, 2018MNRAS.480.2704L} while the ranges of the expected number of LISA sources are extracted from \cite{2001A&A...375..890N, 2017MNRAS.470.1894K, 2019MNRAS.490.5888L, 2018ApJ...866L..20K, 2010ApJ...719.1546L, 2010ApJ...717.1006R, 2018PhRvL.121m1105T, 2020ApJ...898...71B, 2010ApJ...725..816B, 2018MNRAS.481.1908K, 2020MNRAS.492.3061L, 2020ApJ...892L...9A, 2020MNRAS.494L..75S}.}
\label{tab:absolute_n_MWG}
\end{table}



\begin{table}
\centering                          % used for centering table
\begin{tabular}{c | c c }        % centered columns (4 columns)
\hline
% Source & $N \, \mathrm{[MWG^{-1}]}$ & $N^\mathrm{detected} \, \mathrm{[MWG^{-1}]}$ \\
 Source & $N$ & $N^\mathrm{detected}$ \\
\hline
    WD+WD & $\sim 2 \times 10^4$ & 4$-$20 \\
    NS+WD & $\sim 10^3$ & 3$-$6 \\
    BH+WD & $\sim 10^2$ & 2$-$4 \\
    NS+NS & $\sim 40$ & 1  \\
    BH+NS & $\sim 4$ & 0  \\
    BH+BH & $\sim 2 \times 10^2$ & 4$-$7 \\
\hline
\end{tabular}
 \caption{Estimated absolute number of compact binaries in \textit{globular clusters} in the Milky Way. The columns show the source type, the total number of binaries in the galaxy at any frequency and the total number of estimated sources detected by LISA assuming a frequency range of $10^{-5}-1$~Hz and a mission lifetime of 4 years with a SNR ranging between 2 and 7 \citep{2018PhRvL.120s1103K}. }
\label{tab:absolute_n_MWG_GC}
\end{table}




==> ucb_s5.1_InteractionPhysics.tex <==
\subsubsection{Constraining stellar and binary interaction physics}

\noindent \coord{Fritz Roepke, Alina Istrate}\\
\contr{Karel Temmink (1.7.1.1), Mike Lau (1.7.1.1, 1.7.1.7-8), Stephan Rosswog (1.7.1.2, 1.7.1.6), Vasileios Paschalidis (1.7.1.2), Alina Istrate (1.7.1.2), Fritz Roepke (1.7.1.3,1.7.1.6), Kinwah Wu (1.7.1.4-5), St\'ephane Mathis (1.7.1.4), Thomas Tauris (1.7.1.5), Stéphane Blondin (1.7.1.6), Ashley Ruiter(1.7.1.6, 1.7.1.8), Chris Fryer (1.7.1.7), Thierry Foglizzo (1.7.1.7) Manuel Arca Sedda (1.7.1.8), Kyle Kremer (1.7.1.8), Simone Bavera (1.7.1.8), Abbas Askar (1.7.1.8), Silvia Toonen (1.7.1.8), Gijs Nelemans (refs for 1.7.1.8),  Irina Dvorkin (refs for 1.7.1.8),  Valerya Korol (refs for 1.7.1.8), Astrid Lamberts (refs for 1.7.1.8)}\\


Throughout this Section we will highlight science questions related to LISA that can/should be addressed before the launch of the mission with the label \textbf{pre-LISA-launch objective}, while science questions that can only be addressed by using LISA data will be highlighted with the label \textbf{post-LISA-launch objective}.
{\color{blue}It should be emphasized, that in most cases LISA detection of individual binaries is limited to GW frequency and a somewhat poor sky location. For a fraction of these thousands of systems, however, high SNR and/or high frequency will enable the measurement of the GW frequency derivative, a good sky localization, and possibly constraining the eccentricity of the binary system. The GW frequency derivative will reveal the chirp mass of the binary and thus the distance. Although these cases will be exceptional systems in the overall global perspective, they will be the key science drivers that deliver deep insight and new breakthroughs in our understanding of binary compact object systems --- often because of the enhanced chances of finding the EM counterpart of these well-localized systems.}  

\paragraph{Dynamical stability and efficiency of mass transfer in the formation of LISA sources}

\phantom{text}

The formation of compact binary systems with two compact objects is still relatively poorly constrained. Typically, at least two phases of mass transfer are required to form a general observable stellar LISA system: one for each component star to lose their hydrogen envelope, and additional phases are possible to remove the helium-rich envelope. 
To explain the compactness of the orbit, typically one or more of these mass-transfer phases are considered to proceed in an unstable fashion in order to get the necessary amount of orbital shrinkage i.e. a CE phase \citep[e.g.][]{1972AcA....22...73P,1976IAUS...73...75P,1984ApJ...277..355W}. Hence, it is crucial to understand for which binary configurations mass transfer proceed stably, and for which it will be unstable.

\textbf{Pre-LISA-launch objective:} The precise value of the stability boundary (i.e. a critical mass ratio, $q$ between the two stellar components above which  no stable mass transfer is possible) remains under debate. Theoretical work has shown that mass transfer can proceed  significantly more stable than classical results  have previously implied \citep[e.g.][]{1987ApJ...318..794H,2008MNRAS.387.1416C, 2011ApJ...739L..48W, 2012ApJ...760...90P, 2015MNRAS.449.4415P, 2017MNRAS.471.4256V,2020A&A...642A.174M}. 
Similarly, the mass-retention fraction of the accreting companion remains relatively poorly understood \citep[e.g.][]{1972AcA....22...73P, 1999ApJ...513L..41K, 1999ApJ...522..487H, 2000ApJ...530L..93T, 2002MNRAS.329..897H, 2007ApJ...663.1269N, 2020MNRAS.498.4705V}.
These issues severely affect the predicted formation details of compact binaries, and determine which evolutionary pathways are dominating in the formation rate of LISA sources (Section~\ref{subsec:rates}), and hence would leave characteristic imprints on the numbers and properties (orbital periods, masses) of the resulting LISA population \citep[e.g.][]{2017MNRAS.470.1894K,2019MNRAS.484..698R}. 
For instance, whether or not the first phase of mass transfer in the formation of a WD+WD leads to a shrinkage or widening of the orbit (i.e. unstable or stable mass transfer) determines to which size the secondary star can evolve before filling its Roche lobe, which dictates the mass of its core at RLO, i.e. the mass of the resulting WD, and hence the mass ratio of the WD+WD \citep{2000A&A...360.1011N,2001A&A...365..491N,2006A&A...460..209V,2012AA...546A..70T}. 

Stability of mass transfer depends rather sensitively not only on the intricate details of the structure of the donor star, but also on the transfer and potential loss of mass and angular momentum \citep{1997A&A...327..620S}. 
\textbf{Pre-LISA-launch objective:} Hydrodynamical simulations can help settle the question of dynamical stability (see Fig.~\ref{fig:UCXB_hydro}).
The mass that is transferred to the companion can not always be fully accreted by the companion star: spin-up to critical rotation rates and/or strong optically thick winds or outflows (including jets) can result in significant fractions of transferred material being lost from the accreting star. Since mass that is not accreted leaves the binary system, carrying with it an amount of orbital angular momentum, the efficiency of accretion and the stability of mass transfer are linked. In the case of compact object accretors, it is expected that less conservative mass transfer is typically more stable than mass transfer where all mass is accreted \citep{1997A&A...327..620S}. 


\begin{figure*}
    \begin{center}
   \includegraphics[width=0.60\textwidth]{./img_ucb/UCXB_hydro.png}
\caption{Hydrodynamical investigation of dynamical stability in a UCXB with a $0.15\;M_\odot$ WD donor star and a $1.4\;M_\odot$ accreting NS, in an orbit with an initial eccentricity of 0.04. Plotted here is the mass density in the orbital plane after roughly 13 orbits of RLO. The density plot shows eccentric structures in the accretion disc, the complex character of the flow near the circularization radius and a strong density cusp near the NS. The envelope surrounding the binary is sparse but its total mass is significant compared to the disc. Figure from \citet{2017MNRAS.467.3556B}.}
 \label{fig:UCXB_hydro}
  \end{center}
\end{figure*}


\textbf{Post-LISA-launch objective:} Observed samples are required to reverse-engineer the progenitor evolution, and constrain the evolutionary pathways \citep[e.g.][]{2000A&A...360.1011N, 2006A&A...460..209V,2010A&A...520A..86Z,2011MNRAS.411.2277D,2013MNRAS.429L..45P}.
On the EM side, only relatively small samples exist currently, with relatively large biases towards the lower-mass and hotter WDs, since they have longer (observational) lifetimes and are brighter. 
However, LISA will be sensitive to WD+WDs throughout the whole Galaxy and will be able to provide properties of the entire WD+WD population with relatively few selection biases. This will allow for stronger and more meaningful statistical analyses. Additionally, LISA will be able to almost directly measure the Galactic rate and masses of merging WD+WDs, which is another useful tool in constraining progenitor evolution.


The detection of NS+NSs (and potentially NS+BH systems) with LISA allow for a direct view of their formation pathways through their eccentricity, that is induced by the supernova kick associated with the formation of the second NS \citep{2018MNRAS.481.4009V,2020MNRAS.492.3061L}. 
The population of eccentric LISA NS+NS binaries originate from NS+NS binaries born right in or near the sensitivity window of LISA, so that there is little time for GWs to circularise the orbit.  The tight orbit prior to the second SN, leading to NS+NS formation, is characterized by the last phase of mass transfer (see Section~\ref{subsec:1313} and Fig.~\ref{fig:1.9}). This is Case~BB mass RLO initiated by the expansion of the naked helium-star after core-helium depletion. The Case~BB mass transfer episode is believed to be predominantly stable from detailed simulations \citep{2015MNRAS.451.2123T} and in order to match the observed period distribution of Galactic NS+NS systems \citep{2018MNRAS.481.4009V}. However, unstable Case~BB RLO would lead to an additional CE phase that produces NS+NSs with sub-hour periods. Yet, because such NS+NSs that have gone through unstable Case~BB RLO prior to the second SN are formed with higher GW frequencies, they also have a more rapid GW frequency evolution ($f_{\rm GW}/\dot{f}_{\rm GW} \propto f_{\rm GW}^{-8/3}$), which disfavours their detection by LISA \citep{2020MNRAS.492.3061L,2020ApJ...892L...9A}. 
\textbf{Pre-LISA-launch objective:} A deeper understanding of whether or not mass transfer is stable or unstable in Case~BB RLO is needed, and should be investigated further.

\paragraph{Dynamical stability and efficiency of mass transfer in accreting LISA sources}

\phantom{text}


A remarkable property of Roche-lobe filling stars is that, for mass ratios $< 0.8$, their
average density is related to their orbital period \citep[see e.g.][]{2002apa..book.....F}. For mass ratios, $M_{\rm donor}/M_{\rm accretor}<0.8$ the relation is given by:
\begin{equation}
P_{\rm orb}= 10.5\;{\rm hr}\,\left( \frac{\bar{\rho}}{{\rm g\,cm}^{-3}}\right)^{-1/2},
\label{eq:P_rho}
\end{equation}
As an example, Roche-lobe filling stars with orbital frequencies of $0.1\;{\rm mHz}$ ($f_{\rm GW}=0.2\;{\rm mHz}$)  have
$\bar{\rho}\sim 10\;{\rm g\,cm}^{-3}$, while those at 1~Hz possess an average
density of $\bar{\rho}\sim 10^9\;{\rm g\,cm}^{-3}$.
In other words, mass-transferring WDs are located right inside LISA's frequency band. For NS donors, mass transfer only sets in at much smaller separations when the frequencies are already close to the kHz-regime \citep{2011LRR....14....6S}. 

For a LISA stellar source, there are at least two possible scenarios for the subsequent evolution after the onset of mass transfer: a) after an initial brief phase of continued orbital shrinkage after RLO is initiated \citep{2018PhRvL.121m1105T}, mass flows on a much longer timescale from the WD toward the accretor star while the binary separation increases. This process is commonly referred to as a form of stable mass transfer (see Fig.~\ref{fig:DWD-stability}); b) The WD becomes tidally disrupted by the accretor, resulting in the binary merger. This process occurs on a dynamical (orbital) timescale. \textbf{Pre-LISA-launch objective:} Whether the binary undergoes stable  mass transfer vs a merger may have important implications on the type of GW templates that are necessary to detect these binaries with LISA. 

The above discussion makes it clear that for WD+WD, NS+WD, and BH+WD binaries the onset of mass transfer marks a turning point
since the stability of mass transfer decides whether the binary
can survive or will inevitably merge. As mentioned in the previous Sections, its fate depends sensitively on
the internal structure of the mass-donating star, on the mass ratio
and on the involved angular momentum exchange mechanisms,  which here depend primarily on whether mass transfer takes place with or without an accretion disc around the accretor \citep{1982ApJ...254..616R,1984ApJ...284..675H,2004MNRAS.350..113M,2007ApJ...655.1010G,2007ApJ...670.1314M,2009PhRvD..80b4006P,2011ApJ...737...89D,2015ApJ...805L...6S}.
Since fully degenerate WDs possess an inverted mass-radius relation, i.e.\,they grow in size as mass is removed, the mass-donating star will expand
and thereby tend to speed up the mass transfer. However, since the
mass is transferred to the heavier star, the orbit will tend to widen, and therefore stabilize the mass transfer \citep{1997A&A...327..620S,1999A&A...350..928T}.


The way the transferred mass settles onto the accretor star has a
decisive impact on the orbital evolution. If the circularization radius
of the transferred matter is smaller than the radius of the accretor, it will
directly impact onto the stellar surface and spin up the accreting
star -- this scenario is referred to as direct impact accretion. That means that orbital angular momentum is not fed back into the orbit, and therefore the orbital separation shrinks and
mass transfer accelerates. If instead the circularization radius is
larger than the radius of the heavier WD accretor, a disc can form
and --- via its large lever arm --- the disc can feed back angular
momentum into the orbital motion, increase the orbital separation, and thus stabilize the binary system
\citep{1998ApJ...503..344I,2011ApJ...740L..53P,2009PhRvD..80b4006P}. 


\begin{figure*}
    \begin{center}
   \includegraphics[width=0.60\textwidth]{./img_ucb/DWD+UCXB-stability-RLO.png}
   \includegraphics[width=0.60\textwidth]{./img_ucb/DWD-stability-RLO.png}
\caption{Stability regions in the donor mass---accretor mass plane of WD+WDs and UCXBs. Donor star masses are on the vertical axes, accretor star mass on the horizontal axes. {\bf Upper panel}: analytical results of \citet{2004MNRAS.350..113M} where the solid line marks the transition between disc and direct impact accretion, and the other lines show how the strict stability limit of \citet{2001A&A...368..939N} is relaxed when dissipative torques feed angular momentum from the accretor back to the orbit. 
{\bf Bottom panel}: ballistic calculation approach by \citet{2017ApJ...846...95K} using zero-temperature mass--radius relations for the WD donor. Red systems are stable throughout their lifetimes, through stages of both direct-impact and disc accretion; black systems are unstable; and blue systems have an accretor that exceeds the Chandrasekhar limit during their evolution. The solid black line marks again the boundary between disc and direct-impact accretion for initially synchronous and circular binaries. The yellow region indicates systems with a total mass in excess of the Chandrasekhar limit, i.e. potential SN~Ia progenitors. 
It is evident from these figures that UCXBs with low-mass ($\lesssim 0.2\;M_\odot$) He~WD donor stars, and NS accretors, are always dynamically stable.} 
 \label{fig:DWD-stability}
  \end{center}
\end{figure*}

The majority of studies of mass-transfer stability to date assume that the mass-transferring WD is tidally locked. However, as pointed out by~\cite{WebbinkIben1988}, spinning up a WD while being tidally locked from some initial separation down to the Roche limit is accompanied by tremendous energy release that, depending on the dissipation mechanism, could potentially lift the degeneracy throughout the star. Given that the dissipation mechanisms in WD interiors are not well understood, this makes things even more complex: The tidal interaction between the stars can substantially heat up the
mass-donating WD, change its internal structure, and thereby its response response to mass loss.


For LISA this means that the measured chirp of a mass-transferring binary is not only set by the decay of the orbit due to GW, but also due to mass transfer and tidal interactions, and therefore the chirp mass can not be directly measured as in the case of  detached (chirping) binaries. 
However, for an assumed cold equation-of-state mass-radius relation of the donor star, both the mass of the donor star and the model mass-transfer rate can be derived, as these are fully set by the orbital period \citep[][see also Eq.\,\ref{eq:P_rho}]{1971ApJ...170L..99F, 1971ApJ...168..217V}. 
\textbf{Pre-LISA-launch objective:}  Future work should aim at including finite-temperature effects in the WD EOS consistently, e.g.\,by using detailed stellar structure calculations following the formation and evolution of the system --- from the detachment of the CV/LMXB phase until onset of the AM~CVn/UCXB phase (Fig.~\ref{fig:LMXB-UCXB-link}).

\textbf{Post-LISA-launch objective:}  We do not expect the second derivative ($\ddot{f}_{\rm GW}$) of the GW frequency an AM~CVn system to be measurable with LISA, as the low mass ratios required from mass transfer stability considerations ($M_{\rm donor}\ll M_{\rm accretor}$), imply a low-mass WD donor, whose large radius prevents the AM~CVn system from penetrating into the highest frequency range where the second derivate is large \citep{2004MNRAS.349..181N}.
The combination of LISA with EM surveys, such as Gaia, is particularly promising for AM~CVn sources. If their distance is known, the chirp mass can be constrained, which allows for the orbital chirp to be decoupled into its different components \citep{2018ApJ...854L...1B}.

Apart from determining the orbital evolution, mass transfer in a WD+WD also
leads to an accumulation of helium (possibly also carbon and oxygen) on the surface of the accreting WD. If (or when) nuclear fusion commences in this layer, rapid burning follows that causes a nova outburst or, in case of persistent fusion, X-ray emission may be observed as for supersoft X-ray sources \citep{1997ARA&A..35...69K}. Rapid accretion during the last tens of orbits before a merger and the
interaction with the incoming accretion stream can trigger surface
detonations that cause weak SN~Ia-like transients \citep{2010ApJ...709L..64G}. A (tidal) disruption of a WD by a NS or BH could potentially lead to nuclear-dominated accretion flows \citep{2012MNRAS.419..827M,2013ApJ...763..108F}. 

\textbf{Post-LISA-launch objective:} The probability of detecting a Galactic WD+WD merger during the LISA mission is small (since the Galactic WD+WD merger rate is of order one per century \citep{2001A&A...375..890N}, let alone that this number includes all the WD+WD ``mergers'' giving rise to stable RLO after contact, i.e. the AM~CVn systems). Yet, the case of merging WD+WD binaries deserves a separate mention, because of the exciting possibility of multiband and/or multiwavelength observations: the inspiral phase would be detectable by LISA or a similar mission, and the merger phase by a future observatory such as DECIGO \citep{2017JPhCS.840a2010S}. If the merger gives rise to an optical transient (e.g. a SN of Type~Ia/Iax), these can be observed by EM transients surveys such as ZTF and the Vera Rubin Observatory. For NS+WD, the post-merger phase would be detectable by ground-based high-frequency GW observatories, such as LIGO, Virgo, KAGRA and future facilities like Cosmic Explorer \citep{ 2017CQGra..34d4001A} and the Einstein Telescope \citep{ 2010CQGra..27h4007P}, due to either the eventual collapse of the NS core or post-merger oscillations of the remnant \citep{2017LRR....20....7P}. Therefore, NS+WD systems offer the unique opportunity not only to study the dynamics/stability of mass-transfer, but also the potential to place constraints on the nuclear equation of state. Nevertheless, once again, we emphasize the small probability for a Galactic WD+WD merger event during the lifetime of the LISA mission.

\textbf{Post-LISA-launch objective:} In summary, mass transfer is crucial for determining the final fate of interacting close binaries, but many details and many questions still remain unanswered related to e.g. formation and evolution of AM~CVn and UCXB systems and their ultimate fates, and for related questions such as the progenitor systems of Type~Ia/Iax supernovae. Observations with LISA may therefore bring a major leap forward in our understanding of the physics of this crucial evolutionary phase of close-orbit stellar binaries with compact objects. 





\paragraph{Common envelopes \label{paragr:CE}}

\phantom{text}

CE phases are one of the greatest uncertainties in binary stellar evolution theory \citep{2020cee..book.....I} and LISA will provide important measurements.
\textbf{Pre-LISA-launch objective:}  The inspiral of the secondary star into the envelope of the primary lacks obvious symmetries and is therefore not accessible to classical one-dimensional stellar evolution modelling approaches. At least some part of CE interaction takes place on a dynamical timescale. Therefore, parametrized prescriptions for CE evolution are used in stellar evolution modelling. Three-dimensional hydrodynamic simulations have been employed to study the process in more detail \citep{2012ApJ...744...52P,2018MNRAS.477.2349I, 2000ApJ...533..984S, 2012ApJ...746...74R,2015MNRAS.450L..39N,2016MNRAS.460.3992N,2016MNRAS.461..486K,2016ApJ...816L...9O,2016MNRAS.462L.121O,2018MNRAS.480.1898C,2019MNRAS.484..631R,1996ApJ...471..366R,2019MNRAS.486.5809P,2020arXiv200700019K, 2020arXiv200711000S,2020arXiv201106630L}, but they are numerically challenging due to the large dynamical range of spatial and temporal scales of the problem. Furthermore, most often three-dimensional hydrodynamic simulations do not incorporate modelling of physical processes like convection and radiation transport, which are thought to be important especially in the later phases of the inspiral. Complementing the global three-dimensional CE simulations with local, wind-tunnel type, simulations that study the details of the flow around the inspiraling object \cite[e.g.][]{2017ApJ...838...56M, 2020ApJ...897..130D, 2020ApJ...899...77E}, as well as one-dimensional but multi-physics hydrodynamic simulations \cite[e.g.][]{2017MNRAS.470.1788C, 2019ApJ...883L..45F} is a promising avenue to more physically accurate predictions of post-CE binary properties. Lastly, studies of post-CE binaries that are found observationally will provide insights into the CE phase. Valuable constraints on the CE mechanism have come from this method previously \citep{2000A&A...360.1011N,2006A&A...460..209V,2010A&A...520A..86Z,2013A&A...557A..87T}.

Because the actual interaction is short (up to about $10^3$ years), direct observations in optical astronomy are difficult. Some of the fainter optical transients  \citep[luminous red novae;][]{2003ApJ...582L.105S,2011A&A...528A.114T, 2007Natur.447..458K,2020MNRAS.492.3229H,2020A&A...639A.104S} have  been associated with CE events. The two fundamental, and to date unanswered, questions are: i) Which systems manage to eject the CE? ii) What is the final orbital separation of the two stellar cores in this case? \textbf{Post-LISA-launch objective:} The LISA mission is instrumental for clarifying many aspects of the physics of CE phases in two main directions:

\begin{enumerate}
\item \textbf{Direct observations of events related to CE interaction.}\\
The secondary star may be a compact object, but the primary (donor) is typically in a giant phase. Therefore, a generation of sufficiently strong GW signals during inspiral can only be expected if the core of the primary star is also relatively compact, and if the secondary (a compact object) comes close enough during the inspiral. 




The prospects to observe GW signals from the inspiral phase, however, do not seem very promising in current models. While based on a parametrized description of CE inspiral, \cite{2020MNRAS.493.4861G} predict about one detection in a few centuries with LISA. 
The full three-dimensional hydrodynamic CE simulations of \cite{2016PhDT........74O} find weaker signals. The rates for the slower self-regulated phase that proceeds on a thermal timescale are more promising, with a rate of $\approx 0.1-100$ events in the Galaxy during the LISA mission duration \citep{2021arXiv210200078R}.

The detectability, however, depends on how close the stellar cores come to one another during the evolution. This is uncertain and depends on the above questions i) and ii). Due to the inspiral of the secondary into the primary star's envelope, orbital energy and angular momentum are transferred to this (now) CE. Some material becomes unbound and is ejected from the system. Simulations, however, show that this process alone is inefficient and other energy sources (such as the ionization of envelope material, \citealt{2015MNRAS.450L..39N, 2019MNRAS.486.5809P,2020arXiv200711000S}) have to be tapped to achieve full envelope removal. The exact parameters allowing for such a successful CE ejection are still unknown, but it is likely that most initial configurations may fail. Such failed events, however, may produce stronger GW signals. Moreover, more exotic cases  in which, for instance, triple systems enter CE evolution \citep{2020MNRAS.498.2957C,2021MNRAS.500.1921G}, may potentially also be sources of detectable GW signals.

\item \textbf{Indirect information from detecting post-CE sources.}\\
Since all stellar mass LISA sources have presumably gone through a CE phase (disregarding here sources produced in dense clusters via dynamical interactions), comparison of LISA populations with model predictions naturally test CE physics. 
Specifically, the occurrence (and detection) rates of these binary populations depend critically on the orbital separation of the stellar cores after the CE phase. In this sense, the LISA mission will statistically sample the outcome of CE events and the results provide valuable information for answering the above question ii). Moreover, if CEs produce binaries with sufficiently short orbital periods, such that they are within the LISA band immediately at envelope ejection, they will act as a source term for the population of LISA binaries. In the absence of this injection of sources, evolution of the orbits due to GWs produce a predictable expectation for the orbital period distribution of binaries, any deviations from that expectation could be ascribed to an injected population of post-CE systems. By simultaneously modelling the LISA noise curve, the GW foreground from unresolved Galactic sources, and the effect of GWs on a binary population, the initial post-CE separations for the shortest period binaries can, in principle, be derived, and thereby deliver important insight into CE physics.
\end{enumerate}

Contributing to these two aspects, the LISA mission will help to constrain physics of the mysterious, and yet crucial, CE phase in binary stellar evolution. Its results will be used to validate hydrodynamic simulations and to develop new efficient prescriptions of CE interactions that are to be used in binary stellar evolution and population synthesis studies.

\paragraph{Tides and angular momentum transport}

\phantom{text}

The orbital evolution of detached binaries is practically determined by the loss of orbital angular momentum and the exchanges of angular momentum between the stars and the orbit, and also in some situations, the mass loss from the system. 
For binaries with only BH or NS components, tidal effects are completely insignificant (except for the few final orbits before a merger event) and the orbital evolution is entirely determined by GWs alone. 
An example of such a system is the radio pulsar binary PSR~B1913+16 \citep[see][]{2016ApJ...829...55W}.  
For binaries with non-degenerate stars, or tight systems with WDs, tides can be important, leading to measurable differences in the LISA signal. 
The orbital dynamics of the wide-orbit systems is relatively simple, as the orbital angular momentum is decoupled from the spin of the two stars. 
The orbital evolution of these binaries is therefore simply driven by the wind-mass loss of the stars and, in principle, GWs, which nevertheless is negligible in such wide systems.
The situation is very different for the systems with a sufficiently short orbital period. 
First of all, the timescale for the loss of orbital angular momentum via GWs \citep{1963PhRv..131..435P} could be comparable to or shorter than the evolution of the stars and the tidal evolution of the system \citep{1992ApJ...400..175B}. 
Secondly, the sizes of the stars are no longer negligible compared with the orbital separation, and torques can be exerted on the stars effectively \citep{1994ApJ...437..742L,1981A&A....99..126H}.  
Hence, the structures and the hydrodynamical properties of the stars would play an important role in determining the orbital dynamics and the orbital evolution of these systems \citep{2011ApJ...740L..54B,2012MNRAS.421..426F,2014ApJ...790..161S}. 
These have, at least, two immediate consequences on the LISA science: 
i) the number density of persistent GW sources associated with these binaries observable within the LISA band, and 
ii) the event rate of burst sources associated with coalescence or merging, resulting from the orbital decay of these binaries, although these bursts are very rare in our Galaxy.
  
The exchange of angular momentum between the binary orbit and the spin of the stars can be facilitated by the viscous torque \citep[][]{1977A&A....57..383Z}, but in the compact star binaries this coupling is less efficient than the coupling caused by a stellar bulge cause by the tidal deformation of the star \citep{1992ApJ...400..175B,2013MNRAS.428..518D,1992ApJ...398..234K}.  
The degree of tidal deformation of a star depends on its internal structure and dynamics \citep[e.g.][]{2008PhRvD..77b1502F,2014ARA&A..52..171O,2019EAS....82....5M}. 
Thus, even in the absolute absence of viscosity, WDs and NSs would respond differently to tidal deformations \cite[cf. the studies of][]{2019PhRvD.100f3001V,1995ApJ...443..705L,2013MNRAS.428..518D,1992ApJ...400..175B,2013MNRAS.428..518D,1992ApJ...398..234K}. 
The presence of the close companion will trigger a large-scale flow induced by the hydrostatic adjustment of the studied primary to the tidal perturbation, the equilibrium tide \citep[e.g.][]{1966AnAp...29..313Z,2012A&A...544A.132R,2013MNRAS.429..613O}, and a broad diversity of tidal waves (i.e.\,gravity waves, inertial waves, gravito-inertial waves), and the dynamical tide \citep[e.g.][]{2017PhRvD..96h3005X,2020MNRAS.496.5482Y}. 
Their dissipation and the quadrupolar moment they induce modify the inspiral and cause changes in orbital frequency and phase shifts \citep[e.g.][]{1992ApJ...400..175B,2020arXiv200908300W,2020MNRAS.491.3000M}.     
Thus, WD binaries and NS binaries will behave and evolve differently, which will manifest in the LISA GW background. 
Their orbital evolution will also imprint signatures in the GWs that they emit \citep{2019PhRvD.100f3001V,2020MNRAS.491.3000M,2013MNRAS.428..518D,2014MNRAS.443.1057D,2014ApJ...791...76S}. 
The situation can be more complicated  if the compact stars have a large magnetic moment, which is not uncommon among magnetic WDs \citep{2015SSRv..191..111F}. The magnetic moments of NSs may not be as large as those of WDs since NSs are more compact. 
Direct magnetic interactions between two magnetised components should be taken into account and may compete with tidal interactions in LISA sources. 

\textbf{Post-LISA-launch objective:} Our understanding of the interplay between tidal interaction, feedback magnetic-field amplification and orbital angular momentum extraction by GWs is currently very primitive. 
The observations of GWs from such systems will surely expand our knowledge on this subject substantially \citep[e.g.][]{1990MNRAS.244..731K,2012ApJ...755...80P,2002MNRAS.331..221W,2018ApJ...868...19W}.   


\paragraph{Irradiation of companion star }

\phantom{text}

Feedback irradiation effects on companion stars caused by the intense X-ray flux emitted from accreting compact objects may influence the evolution 
 of the orbits of binary stars \citep{1991Natur.350..136P,2014ApJ...786L...7B}. 
In detached systems, energetic millisecond pulsars  \citep[MSPs, recycled to high spin frequencies from a previous recycling phase;][]{1991PhR...203....1B} may irradiate their companion star with a pulsar wind of relativistic particles and hard photons \citep{1992Natur.356..320T}.
Observations have revealed a growing number of such MSPs with a non- or semi-degenerate companion star which is being ablated by the pulsar wind, the so-called black widows and redbacks \citep{2013IAUS..291..127R}. This is evidenced by the radio signal from the pulsar being eclipsed for some fraction of the orbit \citep{1988Natur.333..237F}.
Tidal dissipation of energy in the donor star envelope \citep{1994ApJ...436..312A} may cause the companion star to be thermally bloated and thereby evaporate more easily.
For LISA binaries, such mass loss via ablation/evaporation will modify their orbital evolution \citep[e.g.][]{2013ApJ...775...27C,2018ApJ...864...30H}, which is otherwise dictated by GWs and tides. For this reason, we may gain new insight on irradiation efficiency from LISA detections of such systems and precise measurements of their orbital frequency. \textbf{Pre-LISA-launch objective:} The impact and the modelling of this effect, often leading to cyclic accretion, is still unclear needs to be improved before LISA flies.

\textbf{Post-LISA-launch objective:} For accreting LISA sources, the irradiation will lead to disturbance of the thermal equilibrium of the companion star \citep{2004A&A...423..281B} and, in the extreme situation, geometrical deformation \citep{2002MNRAS.337..431P}, thereby affecting its mass-transfer rate and thus the orbital evolution of the binary. 
Such an effect may indeed be measured by LISA via its impact on the orbital frequency derivative, and thus the chirp mass of the system. 
Hence, detection of a number of mass-transferring UCXBs and AM~CVn systems by LISA could provide us with unique ways of probing the physics governing close compact object binaries \citep{2016ApJ...830..153J,2017ApJ...846...95K}. 



\paragraph{Type~Ia supernovae and other transients }\label{paragr:SNeIa}

\phantom{text}

Stellar interactions in binary systems containing at least one WD are thought to trigger Type~Ia supernovae  (SN~Ia)
and likely a variety of other transients \citep[see e.g.][for a review]{2012NewAR..56..122W}. SN~Ia were of paramount importance for the discovery of the accelerated expansion of the Universe 
and they significantly contribute to cosmic nucleosynthesis, but the lack of a clear observational connection between a progenitor
system and the observable phenomenon has made their understanding difficult. Without proper initial conditions their
modelling remains uncertain.

The properties of the ensuing explosion  are determined by the pre-explosion state of the WD, but is it triggered
when approaching the Chandrasekhar-mass limit, or well before? The occurrence rate, the delay time between binary 
formation and SN explosion, and the ignition process are all determined by the nature of the progenitor system, 
and they have a strong impact on the contribution of thermonuclear SNe to galactic chemical evolution. A traditional 
broad classification is to distinguish between single-degenerate systems, where the companion of the exploding WD is a 
non-degenerate star --- and the double degenerate systems --- where the interaction of two WDs (mergers, or in rare cases
collisions) triggers the SN explosion \cite[see][for a breakdown of binary star progenitor configurations]{2020IAUS..357....1R}. 

None of the progenitors and explosion mechanisms is established beyond doubt. The single-degenerate 
Chandrasekhar-mass model, that served as a reference for a long time, has several shortcomings, but it seems 
to be needed to explain observed abundance trends \citep{2013A&A...559L...5S}. 
However, both population synthesis models and observations indicate that single degenerate explosions fall short of explaining the observed SN~Ia rate.
GW signals were derived from explosion simulations of near-Chandrasekhar mass WDs \citep{2011PhRvL.106t1103F, 2015PhRvD..92l4013S}, but the prospect of measuring individual events is low.

The major competing double-degenerate scenario received increased attention over the past years 
and is of particular interest in the context of LISA. In this scenario, however, the process initiating the 
actual thermonuclear explosion is unclear. For massive WDs, the remnant can reach or exceed the 
Chandrasekhar-mass, but the explosion could also be triggered in the merger process itself while the more 
massive WD is well below the Chandrasekhar mass limit \citep{2010Natur.463...61P, 2012ApJ...747L..10P}. 
Apart from GW-driven (close-to-circular) mergers, {\em collisions} can also (likely to a much smaller extent) contribute to the SN~Ia rate \citep{2009ApJ...705L.128R, 2009MNRAS.399L.156R}. They may occur in locations with large
stellar number densities such as globular cluster cores or galactic centres, but they
are generally thought to occur too infrequently to explain the bulk of SN~Ia \citep[][but see \citealt{2013ApJ...778L..37K} for more optimistic claims]{2018A&A...610A..22T}.
Such collisions, however, have the advantage of a very robust and physically understood explosion
mechanism: WDs of the most common type ($\sim 0.6\;M_\odot$),
that collide with velocities given by their mutual gravitational attraction, cause
strong shocks in the collision and nuclear burning occurs in the right density regime,
so that the resulting explosions appear as rather common Type~Ia SNe
\citep{2009ApJ...705L.128R}. Before the final collision causes a thermonuclear explosion,
the two WDs may undergo several close encounters causing a sequence of
GW bursts in the LISA band of increasing amplitude.

Further clarification of the double-degenerate progenitor channel of Type~Ia SNe 
requires the determination of the exact demographics of WD merger events --- what is their
occurrence frequency for different WD masses? It is further crucial to understand whether
the explosion is triggered during the merger itself or, maybe, already during the inspiral 
phase when mass transfer between both WDs sets in. Even if only small amounts of
mass are exchanged, the re-distribution of angular momentum can have a substantial
impact on the orbital dynamics and therefore on the GW signal \citep{2011ApJ...737...89D}.   
\textbf{Post-LISA-launch objective:}  The LISA mission has great potential to contribute here and to provide important clues
to the mechanism of Type~Ia SN explosions. \citet{2010ApJ...717.1006R} found that on the order of $\sim 500$ WD+WD pairs --- whose total mass exceeds the Chandrasekhar mass limit and will 
merge within a Hubble time --- could be resolvable by LISA in our own Galaxy. 
While most likely no such systems will merge and give rise to a SN~Ia during LISA's operation, 
much can be learned about SN~Ia (and more generally transient) demographics from 
detecting these plausible progenitor systems.



\paragraph{Core-collapse and supernova kicks }\label{paragr:ccSNe}  

\phantom{text}

Observations of compact objects, from pulsar proper motions \citep{2005MNRAS.360..974H} to compact binary properties \citep{2005MNRAS.363L..71D, 2017NewAR..78....1M}, argue that many NSs and some BHs receive natal kicks during the collapse and explosion of the massive star that forms them. 
Asymmetries in the explosion mechanism, manifested either through asymmetries in the mass ejecta \citep{2013A&A...552A.126W} or neutrino emission, have been studied as a source of these kicks. The different mechanisms \citep{2001ApJ...549.1111L} produce different predictions for the distribution of their magnitude \citep{2006A&A...457..963S}, their orientation with respect to the orbital angular momentum \citep{1961BAN....15..265B}, to the stellar spin \citep{2006ApJ...639.1007W, 2012MNRAS.423.2736N, 2013A&A...552A.126W}, and to the distribution of heavy elements \citep{2013A&A...552A.126W,2014Natur.506..339G}.
The asymmetries produced by strongly magnetized explosions are generally aligned with the angular momentum in the collapsing star \citep{2008ApJ...672..465S, 2020MNRAS.492.4613O, 2020ApJ...896..102K} and these mechanisms will produce kicks with directions aligned with the rotation axis, which typically is also aligned with the orbital angular momentum axis. Mechanisms produced by the large-scale convective eddies in the neutrino driven mechanism can produce kicks that are distributed more isotropically \citep{2013A&A...552A.126W, 2019MNRAS.484.3307M}. 

Different kick mechanisms also predict different kick magnitudes as a function of the compact remnant mass \citep[][and references therein]{2017ApJ...846..170T,2020arXiv200608360M}. These kick distributions, in turn, predict different properties in compact object binaries \citep{2003MNRAS.342.1169V, 2020MNRAS.492.3061L}. The NS kick properties can thus affect the number of NS+NS, BH+NS and BH+BH binaries detectable by LISA and LIGO/Virgo \citep{2003MNRAS.342.1169V,2016ApJ...819..108B,2018MNRAS.481.4009V,2018MNRAS.481.1908K,2020ApJ...891..141G,2020MNRAS.492.3061L}, as well as EMRIs \citep{2019MNRAS.485.2125B}.

For example, it has been demonstrated \citep{2013ApJ...778L..23T,2015MNRAS.451.2123T} that ultra-stripped SNe are at work in close-orbit NS+NS and BH+NS systems that LISA and LIGO will eventually detect. The reason being that extreme stripping of the companion star by the accreting NS or BH during the last mass-transfer stage (Case~BB RLO), produces an almost naked metal core prior to the second SN. This has an important effect on the magnitude of the kick added onto the newborn (second) NS, which affects the survival probabilities. It was argued qualitatively and quantitatively \citep{2017ApJ...846..170T} that the resulting kicks are often, but not always, small --- depending on the mass of the collapsing metal core and thus on the resulting NS mass --- which enhances the survival probability.

\textbf{Post-LISA-launch objective:} The overall detection rate of Galactic NS+NS systems by LISA is thus directly affected by the magnitude of the kick, since a large kick can disrupt the binary during the SN. A large kick may also produce moderately more eccentric LISA NS+NS sources \citep{2020MNRAS.492.3061L}. The systemic velocity imparted by the two SN kicks displaces a binary from its birth position in the thin Galactic disc. LISA’s ability to localise Galactic NS+NS sources on the sky to within a few degrees \citep{2019MNRAS.483.2615K, 2020MNRAS.492.3061L} may therefore constrain the kick distribution by measuring the Galactic NS+NS scale height.
By increasing the sample of observed compact binaries, LISA can thus be used to constrain the kick mechanism. In turn, this constrains the nature of SN explosions in binary system \cite{2004ApJ...612.1044P}.


 \paragraph{Neutron star equation of state}
  
\phantom{text}

Matter in the interior of a NS is compressed to densities exceeding those in the centre of atomic nuclei, providing a unique possibility to probe the nature of the strong interaction and to determine the NS composition.  Via the EOS, matter properties determine the star's radius for a given mass \citep{2016PhR...621..127L, 2016ARA&A..54..401O}.  Candidate EOSs can be tested by measuring the mass and radius for a NS or via the accurate measurement of a NS with a high mass because each EOS has a corresponding maximum allowed mass.  Thus, finding a NS with a mass above the maximum allowed for an EOS rules out that EOS, and the radio measurement that PSR J0740+6620 has a mass of 2.14 solar masses rules out many EOSs \citep{2020NatAs...4...72C}.  In addition, the Neutron Star Interior Composition Explorer (NICER) has enabled the measurement of the mass and radius for PSR 0030+0451. In particular, M/R is measured to 5\%, but M and R separately are known to $\approx10$\,\% \citep{2019ApJ...887L..21R, 2019ApJ...887L..24M}, and the uncertainties still do not allow for the determination of a unique EOS. STROBE-X and eXTP could do the same work as NICER to even to a larger distance. Masses provided by GW measurements would help dramatically, since  for the pulsars observed using NICER the pulse profile fitting is mostly sensitive to M/R, and having data points with M and M/R measured well is much more valuable than just having M/R.  With GW measurements, the determination of the tidal deformability for merging NSs is another measurable parameter that can constrain the EOS, as has been shown for GW170817 \citep{2018PhRvL.121p1101A}.  Given the small number of constraining measurements to date, it is clear that additional EM measurements of pulsars and GW measurements of merging NSs are both necessary \citep{2020ApJ...893L..21R} to obtain conclusions that will affect our understanding of fundamental physics.

\textbf{Post-LISA-launch objective:} Many binary systems with NSs produce GWs that will be detectable by LISA, leading to NS mass distributions for various binary populations, and some of these populations may have high mass NSs to further constrain the EOS.  While NS+NSs are somewhat rare, binaries with a WD and a NS are expected to be plentiful.  LISA will also detect binaries that are approaching mergers, and predicting mergers will allow for EM observations to be planned at the time of the merger.  UV, optical, and near-IR observations to determine the remnant type and to constrain the mass and velocity of the ejecta will be very powerful for constraining the EOS \citep{2018MNRAS.480.3871C, 2019ApJ...880L..15M}, especially with a facility like STROBE-X.


\paragraph{Disentangling formation environments based on LISA data}
\label{ucb_dis_form}

\phantom{text}

One of the exciting prospects of LISA observations is the possibility to disentangle the formation channels from compact sources in different environments based on their distinctive properties/demographics; most importantly isolated binary evolution in the Galactic disc or dynamical interactions in dense environments (e.g.\,open, globular and nuclear star clusters) or isolated triple evolution (Section\,\ref{subsec:formation-binaries}). 
Whereas the majority of LISA binaries are expected to form in isolation (Section\,\ref{subsec:rates}), several key properties, in particular orbital eccentricity and component masses, can reveal deviating birth environments.
If LISA is able to constrain these source properties from the GW signal for a given resolved system, the formation channel for that particular system may be inferred. Here, we describe briefly ways these properties may differ between different formation channels and describe applications to particular classes of binaries.

In general, BH and WD binaries that form as isolated systems through standard binary evolution processes are expected to be nearly circular by the time they enter the LISA frequency band. This is a consequence of the various dissipative forces expected to operate throughout the binary evolution that circularize the binary orbit, namely CE \citep{2013A&ARv..21...59I,2016A&A...596A..58K,2018MNRAS.480.2011G,2020arXiv200109829V} and tidal interactions \citep{1977A&A....57..383Z,2014LRR....17....3P,2020A&A...636A.104B}.
In contrast, LISA binaries that formed dynamically in dense stellar environments may have relatively high eccentricities. In the dense star clusters, frequent dynamical encounters impart large eccentricities to binaries \citep{2003gmbp.book.....H}, whereas the formation of triple systems with an inner double compact object can reach high eccentricities via von Zeipel-Kozai-Lidov cycles \citep{2016ApJ...816...65A,2018arXiv180506458A,2019MNRAS.483.1233R,2020arXiv200908468M}, which induce a secular variation of the inner binary eccentricity \citep{1910AN....183..345V,1962AJ.....67..591K,1962P&SS....9..719L}.

Dynamically formed binaries are expected to feature several distinct sub-classes of formation channels that may also be distinguished by their eccentricities. In order of increasing characteristic formation frequency, these dynamical sub channels include: binaries dynamically {\em ejected} from their host cluster that merge as isolated binaries ($f_{\rm{GW}}\approx 10^{-5}\;{\rm Hz}$), binaries that merge {\em in cluster} between strong dynamical encounters ($f_{\rm GW}\approx 10^{-3}\;{\rm Hz}$), and finally binaries that merge in cluster through {\em GW capture} during single--single ($f_{\rm GW}\approx 10^{-1}\;{\rm Hz}$) or few-body dynamical encounters encounters ($f_{\rm GW}\approx 1\;{\rm Hz}$) 
\citep{2016ApJ...830L..18B,Banerjee2018,2018PhRvL.120s1103K,2018MNRAS.481.5445S,2018MNRAS.481.4775D, 2018arXiv180506458A,Samsing2019a, 2019PhRvD..99f3003K, 2019ApJ...871...91Z, Banerjee2020, 2020ApJ...894..133A}. 
\textbf{Post-LISA-launch objective:}  Binaries formed through the ejected and in-cluster merger channels are expected to have eccentricities at GW frequencies of $10^{-2}\;{\rm Hz}$ of roughly $10^{-3}$ and $10^{-2}$, respectively, which are expected to be measurable by LISA \citep{2016PhRvD..94f4020N}. Furthermore, the likelihood of an eccentric merger is dependent on the eccentricity and orbital separation of the outer perturber's orbit and the mutual orientation of the outer and inner orbit \citep{2018ApJ...863...68L,2018arXiv180506458A}.  
Since the typical binary architecture can be connected with the cluster structure, in terms of either mass and radius or velocity dispersion, the detection of binaries with given orbital properties can carry insights on the type of cluster that harboured the merger.


In nuclear star clusters and, more in general, galactic nuclei, the formation and evolution of compact binaries can be substantially affected by the presence of an MBH \citep{1995MNRAS.272..605L,2002ApJ...578..775B,2009ApJ...692..917M,2020ApJ...891...47A}. MBHs are not only a common occurrence in nuclear star clusters \citep[e.g.,][]{2007ApJ...655...77G, 2008AJ....135..747G}, but their masses are correlated \citep{2009MNRAS.397.2148G, 2013ApJ...763...76S, 2016IAUS..312..269G}. The binary can develop ZKL oscillations as a result of secular perturbations exerted by the MBH tidal field \citep{2012ApJ...757...27A,2018ApJ...856..140H,2019MNRAS.488...47F,2020ApJ...891...47A}. Up to 40\% of binaries undergoing ZKL oscillations in galactic nuclei transit into the LISA band with an eccentricity $> 0.1$ \citep{2020ApJ...891...47A}. LISA has the potential to measure the eccentricity oscillations driven by an MBH onto a stellar BH+BH binary out to a few~Mpc \citep{2019ApJ...875L..31H} thus offering a unique way to probe the KL mechanism in galactic nuclei and to disentangle this sub-channel of the dynamical formation scenario. \textbf{Post-LISA-launch objective:} Thus, if measurable by LISA, eccentricities (or lack thereof) may serve as a strong fingerprint pointing toward the specific formation channel \citep{2016ApJ...830L..18B,2017MNRAS.465.4375N,2019arXiv190702283R,2019PhRvD..99f3003K}.

In the case of NS binaries, NS natal kicks \citep[e.g.,][]{2005MNRAS.360..974H} may result in high-eccentricities for binaries that form through isolated binary evolution. In this case, eccentricity may no longer be useful for distinguishing between the dynamical and isolated formation channels. However, even in this case, dynamical and disc binary NSs may still have distinguishable eccentricity distributions that can potentially be differentiated with LISA \citep{2020ApJ...892L...9A}.

Although rare, dynamically-formed NS+BH systems represent a class of GW sources that potentially offer the widest range of peculiarities compared to the isolated channel in terms of total mass, primary mass, and high eccentricity at mHz frequencies \citep{2020CmPhy...3...43A}. Isolated NS+BH systems  \citep{2018MNRAS.481.1908K} are mostly characterised by BHs with masses of $6-10\;M_\odot$ at high, Milky Way-like metallicity ($Z=0.0088$), or BH masses of $10-25\;M_\odot$ at low metallicity, ($Z=0.0002$), and nearly zero eccentricity at merger \citep{2018MNRAS.480.2011G}. Dynamical formation of these systems is not generally relevant for isolated LISA sources in the Milky Way, but in globular and nuclear clusters up to 50\% of dynamically formed compact NS+BH feature BH masses $>10\;M_\odot$, and a large probability ($\sim 50\%$) will have an eccentricity $> 0.1$ when transiting into the mHz~frequency band of LISA \citep{2020CmPhy...3...43A}.

In general, GW sources forming through dynamical channels may contain compact objects with masses that differ or that are even not expected to form at all from isolated binary evolution of Galactic disc sources. 
For instance, BHs with masses between $\sim 55\;M_\odot - 120\;M_\odot$ are not expected to form from the evolution of single massive stars due to pair-instability SNe \citep{2007Natur.450..390W,2012ApJ...749...91F,2016Natur.534..512B,2017MNRAS.470.4739S,2019ApJ...887...53F, 2021arXiv210307933W}. This range has been described as the upper-mass-gap for BHs.
It may be possible to form binaries containing BHs in this mass range through dynamical processes in stellar clusters \citep{2020MNRAS.497.1043D}. One channel to form such BHs could be through hierarchical mergers of stellar-mass BHs in nuclear and globular clusters \citep{2002MNRAS.330..232C,2019PhRvD.100d3027R,2020ApJ...894..133A,2020ApJ...891...47A,2020arXiv200609744S,2020arXiv200715022M}. Hierarchical mergers are most likely to happen in the densest stellar clusters with the highest escape velocities, such as nuclear star clusters, as these clusters can retain the binary despite the GW recoil kick from the merger \citep{2018ApJ...856...92F,2019MNRAS.486.5008A,2020MNRAS.tmp.2017F, 2020A&ARv..28....4N,2020ApJ...891...47A}.  In these extreme environments, binaries at formation are tighter, on average, than in normal clusters, and the interactions with flyby stars and the possible long-term effect of a central MBH can boost stellar collisions and BH mergers, thus possibly inducing a significant modification of the BH mass spectrum. Another possibility to form more massive BHs could be through collisional runaway mergers of BH progenitors in dense star clusters \citep{2002ApJ...576..899P,2004Natur.428..724P,2006MNRAS.368..121F,2006MNRAS.368..141F,2015MNRAS.454.3150G,2016MNRAS.459.3432M,2020MNRAS.497.1043D,2020arXiv200610771K}. 

\textbf{Post-LISA-launch objective:} Such runaway mergers and collisions in dense clusters can also lead to the formation of IMBHs in the mass range $10^2-10^4 \; M_\odot$ \citep{2001ApJ...562L..19E,2006ApJ...641..319P,2006ApJ...640L..39G,2007CQGra..24R.113A,2016ApJ...819...70M,2019arXiv190605864A,2020arXiv200604922A,2020MNRAS.tmp.2099H, 2020ApJ...894..133A, 2020arXiv200715022M}, and mergers of IMBH+IMBH with component masses in the range $10^3-10^4\;M_\odot$ can be observed with LISA up to redshift $z\lesssim 3$ \citep{2019arXiv190605864A,2019arXiv190811375A,2020arXiv200713746A,2020NatAs...4..260J}. 
The number and characteristics of BHs in the upper mass-gap could shed a light on the relative contribution of dynamically-formed or isolated sources to the overall population of BH+BH mergers. 

Lastly, the evolution of isolated triples can also lead to a mass distribution that deviates from that of isolated binary evolution. This is mainly due to two effects. Firstly, to form a LISA source, isolated binary evolution relies on one or more mass-transfer phases that reduce the orbital period (Section~\ref{subsec:formation-binaries}) down to the range observable by LISA. Mass transfer can also occur in triples \citep[even a larger fraction of triples experiences RLO;][]{2020A&A...640A..16T} (Sections~\ref{paragr:triples} and \ref{subsubsec:triples_formation}), however orbital shrinkage can also be achieved by the combination of three-body dynamics with dissipative processes. The increased eccentricities during von Zeipel-Kozai-Lidov cycles reduce the GW inspiral time \citep[e.g.][]{2011ApJ...741...82T,2017ApJ...841...77A,2018ApJ...863....7R,2019MNRAS.486.4443F}. Moreover, if a star does not fill its Roche lobe, and does not lose its envelope prematurely, it typically will form a more massive remnant compared to the case of RLO mass stripping. Such triples will on average contain stars that are more massive than those formed through isolated binary evolution \citep{2013MNRAS.430.2262H, 2018A&A...610A..22T}, and will not contain He-core WDs (which have masses $\lesssim 0.45M_{\odot}$ which can only be formed in a Hubble time through mass stripping). Secondly, similar to the evolution in star clusters, sequential mergers in multiples give rise to higher stellar masses \citep{2020ApJ...888L...3S, 2020ApJ...898...99H, 2020arXiv200910082L}. In addition, the effect of a tertiary perturber can induce precession of the spins and lead to spin misalignment \citep{2018MNRAS.480L..58A,2018ApJ...863...68L,2018ApJ...863....7R}. 


==> ucb_s5.2_GalacticProbes.tex <==
\subsubsection{LISA sources as galactic probes} 

\noindent \coord{Valeriya Korol}\\
\noindent \contr{Valeriya Korol, Raffaella Schneider, Luca Graziani, Astrid Lamberts, Samuel Boissier, Martyna Chruslinska, Alberto Sesana, Katie Breivik, Shane Larson, Michela Mapelli}\\

Stellar binaries detectable by LISA bear the imprint of the properties of their native stellar environments (galaxies and stellar clusters) such as the total stellar mass, IMF, star formation history (SFH), age and metallicity ($Z$). These properties can be investigated by combining binary population synthesis (BPS) models (Section~\ref{subsubsec:codes}) with models of galaxy formation and evolution.
Several methods have been developed to achieve this goal. The combination of BPS models with theoretical semi-analytic or observationally inferred cosmic star formation rate densities  provides a fast way of predicting the evolution of the overall birth and merger rates with redshift \citep{2001MNRAS.324..797S, 2011RAA....11..369R, 2011PhRvD..84l4037M,2013ApJ...779...72D,2016Natur.534..512B,2016MNRAS.461.3877D,2016MNRAS.463L..31L,2018MNRAS.473.1186E,2019MNRAS.488.5300C,2019ApJ...881..157B}.
In particular, observation-based approaches allow one to account for the current observational uncertainties on the birth metallicity distribution of stars forming over the cosmic history and evaluate the related uncertainty on the predicted properties of mergers \citep[e.g.][]{2019MNRAS.488.5300C}.
A detailed understanding of the properties of galaxies hosting GW sources can be gained from cosmological simulations, which provide a detailed description of the cosmic star formation in a more accurate context of the galaxy evolution. Galaxy catalogues from the Illustris \citep{2014MNRAS.444.1518V}, GASOLINE \citep{2001PhDT........21S,2004NewA....9..137W}, 
EAGLE \citep{2015MNRAS.446..521S} simulations have been used for predicting NS+NS and BH+BH mergers  \citep[e.g.][]{2017MNRAS.472.2422M,2017MNRAS.464.2831O,2019MNRAS.487.1675A}. Similarly, the Latte simulation of Milky Way-like galaxies of the FIRE hydrodynamical simulation project \citep{2014MNRAS.445..581H,2016ApJ...827L..23W} was adopted to study the properties of Galactic WD+WDs and BH+BHs accessible to LISA \citep{2018MNRAS.480.2704L,2019MNRAS.490.5888L}. Alternative hybrid pipelines  such as \texttt{GAMESH} \citep{2015MNRAS.449.3137G,2017MNRAS.469.1101G,2019Physi...1..412G}, combining a dark matter simulation with semi-analytic star formation, chemical enrichment and numerical radiative transfer, represent an advantageous alternative to study the redshift evolution of compact binaries along the assembly of a Milky Way-like galaxy and in its local volume dwarf satellites \citep{2017MNRAS.471L.105S,2019MNRAS.484.3219M,2020MNRAS.495L..81G}.




{\it Effect of the IMF.} The IMF is one of the key ingredients in the BPS that sets the distribution of initial masses and the relative proportions of stars forming in different mass ranges. Therefore it has a direct impact on the observed merger rates and properties of the LISA sources. Studies often adopt the IMF inferred from the observations of stars in the local Galactic neighborhood \citep[e.g.][]{2001MNRAS.322..231K,2003PASP..115..763C}. However the universality of this assumption is one of the fundamental open questions in astronomy and is still debated \citep[e.g.][]{2010ARA&A..48..339B}. Theoretical studies
show that with the assumption of the Milky Way-like IMF one may underestimate the number of WD and NS progenitors forming at redshifts $\lesssim$ 1, especially at low metallicities \citep{2020A&A...636A..10C}, and,
therefore,  underestimate  the  predicted  number  of  individual  LISA  detections  and  background/foreground  noise. 

\textbf{Post-LISA-launch objective:} LISA's observations of stellar remnants --- invisible to EM observatories --- will offer us an alternative way of probing the IMF. For instance, hundreds of Galactic WD+WDs with measured chirp mass \citep{2019MNRAS.482.3656R} can be used to constrain the low-mass end of the IMF in different Galactic habitats. In addition, numerous LISA detections in the Magellanic Clouds will enable the studies of the IMF with GWs in alternative environments \citep{2020A&A...638A.153K}. 


{\it Effect of metallicity.}
The metallicity is another important assumption of the models that affects different types of stellar binaries in different ways \citep{2019MNRAS.482.5012C}. 
The predicted metallicity dependence of the formation efficiency of merging BH/NS binaries is a complex function of numerous poorly constrained phases of binary evolution. 
Specifically, BH+BH mergers resulting from isolated stellar evolution are typically found to form much more efficiently at low metallicity ($\lesssim 0.1-0.3\;$Z$_\odot$) than at solar metallicity \citep{2010ApJ...715L.138B, 2016MNRAS.462.3302E, 2017NatCo...814906S,2017MNRAS.471L.105S, 2018A&A...619A..77K, 2018MNRAS.474.2959G}. The differences in formation efficiency reach up to two orders of magnitude and consequently, the size of the observable BH+BH population is sensitive to the amount of star formation happening at low metallicity
\citep{2013ApJ...779...72D,2017MNRAS.472.2422M, 2019MNRAS.484.3219M, 2019MNRAS.482.5012C, 2019MNRAS.490.3740N,2020MNRAS.495L..81G, 2020ApJ...898..152S,2020arXiv200903911S}.
Furthermore, the most massive BH+BH are expected to form at low metallicity
and their mass distribution could potentially be linked to the metallicity distribution
of their progenitors.
Metallicity dependence of the formation efficiency of NS+NS mergers is typically found to be much weaker than for BH+BH, with the mixed systems falling in between.
For the case of WD+WD, the metallicity mainly changes the total number of WD+WDs by allowing lower masses for a star to reach the WD stage in a Hubble time with decreasing metallicity. This results in a moderate increase (few tens of percents) in the number of resolved LISA sources  \citep{2010A&A...521A..85Y,2020A&A...638A.153K}. 


 {\it Effect of star formation histories.} The merger rate of compact stellar binaries across cosmic time is a direct consequence of the SFH \citep{2017ApJ...840...39M,2019MNRAS.487.1675A,2013ApJ...779...72D,2017MNRAS.472.2422M,2018MNRAS.479.4391M,2019ApJ...886L...1V,2019MNRAS.490.3740N,2020ApJ...898..152S}. Together with BPS models, SFH regulates the content of stellar binaries in the LISA band at a given time. Galactic WD+WDs can be used as a tool to study the SFHs of the MW components: due to the different timescales to reach the mHz frequencies, WD+WDs of different core composition dominate different parts of the Galaxy due to their distinct SFHs. Specifically, double He-core WDs with formation times that can exceed 10~Gyr populate the Galactic bulge, thick disc and stellar halo; double C/O-core WDs, typically form on timescales shorter than 2~Gyr and are associated with a much younger populations present in the thin disc; mixed He-C/O-core binaries present an intermediate distribution \citep{2010A&A...521A..85Y,2019MNRAS.490.5888L}. In addition, SFH has significant effects on the LISA detection rates in the Milky Way satellites \citep{2020A&A...638A.153K}. 
 

    
{\it Structure of the Milky Way with resolved and unresolved sources.} It is expected that the Galactic GW population at mHz frequencies will be largely dominated by WD+WDs and will have two components in the LISA data: population of high-frequency individually resolved binaries and unresolved stochastic foreground from low-frequency binaries (Section~\ref{paragr:foreground}). Both resolved and unresolved WD+WDs encode global properties of Galactic stellar populations, and can thus be used as a tool to study the Milky Way’s stellar content and shape. 

\textbf{Post-LISA-launch objective:} Affected by different selection biases than EM observatories, LISA can probe the entire volume of the Milky Way and therefore will facilitate detailed studies of its the far side (Fig.\,~\ref{fig:MW}). Moreover, unaffected by the dust extinction and stellar crowding, LISA can also probe the inner Galaxy at all latitudes. For several thousands WD+WDs measurements of the sky positions and distances will enable the mapping of the Galaxy. Reconstructed density profiles of WD+WDs will provide unbiased constraints on the scale length parameters of Galactic bulge/bar and disc that are both accurate and precise, with statistical errors of a few \% to 10\% level \citep{2012PhRvD..86l4032A,2019MNRAS.483.5518K,2020arXiv200311074W}. The Galactic stellar halo is also expected to host up to a few thousand WD+WDs, and therefore can potentially be studied with WD+WDs in a similar way \citep{2009ApJ...693..383R,2010A&A...521A..85Y,2019MNRAS.490.5888L}. Furthermore, the LISA sample is found to be sufficient to disentangle between different commonly used disc density profiles, by well covering the disc out to sufficiently large radii. The stellar bar will also clearly appear in the GW map of the bulge. LISA's WD+WDs can accurately characterise the bar's physical parameters: length, axis ratio and orientation angle with respect to the Sun's position \citep{2020arXiv200311074W}. However, because of the low density contrast compared to the background disc, the spiral arms will be elusive to LISA. Finally, building upon the analogy with simple stellar population models used for inferring stellar masses of galaxies based on their total light, the total stellar mass of the Galaxy can be estimated from the number of LISA events. Using a simplified example of Milky Way satellites, \citet{2021MNRAS.502L..55K} showed that based on BPS models of LISA sources satellite masses can be recovered within 1) a factor two if the SFH of the satellite is known and 2) within an order of magnitude even when marginalising over alternative SFHs. When also accounting for the unresolved Galactic foreground, this method could be extended for measuring the total stellar mass of the Milky Way.


\textbf{Post-LISA-launch objective:} The power of constraining the overall properties of the Galactic potential will be significantly enhanced by using LISA detections in combination with EM observations of binaries motions. BPS studies forecast up to 150 detached and interacting WD+WDs detectable through both EM and GW radiation \citep[e.g.][see also Section~\ref{subsec:rates}]{2017MNRAS.470.1894K,2018ApJ...854L...1B}. For these multi-messenger binaries 3D positions provided by LISA can be combined with proper motions --- for example provided by Gaia or Vera Rubin Observatory --- into the rotation curve, which allows the derivation of the stellar masses of the Galactic baryonic components \citep{2019MNRAS.483.5518K}.

                
The unresolved Galactic foreground will provide complementary constraints on the Galactic structure. For example, the Galactic foreground will show whether the WD+WD population traces the spatial distribution of young, bright stars (and thus do experience significant kicks), or traces a vertically heated spatial distribution associated with Galaxy's oldest stellar populations.
This can be understood from the shape of Galactic power spectral density that depends on the characteristic scale height of the WD+WD population \citep{2006ApJ...645..589B}. 
\textbf{Post-LISA-launch objective:}  In addition, using the spherical harmonic decomposition of the LISA data streams, the structure of the disc population of Galactic WD+WDs can be constrained with an accuracy of 300~pc \citep{2020ApJ...901....4B}. The relative poor resolution compared with the resolved sources is a direct consequence of LISA's poor spatial resolution at low frequencies. Nevertheless, an independent measurement at low frequencies will either help to confirm the structure of the resolved sources or point to frequency-dependent Galactic structure.





\begin{figure*}
    \begin{center}
  \includegraphics[width=0.60\textwidth]{./img_ucb/MW.pdf}
\caption{Numerous WD+WDs detectable by LISA will enable the mapping of our Galaxy. In the background the artist impression of our current view of the MW. Over-plotted in colour WD+WD with SNR$>7$ from \citet{2020arXiv200311074W}. LISA's position is at $(0,0)$. The selection effect due to GW frequency in visible in colour. Figure credit: Valeriya Korol.}
 \label{fig:MW}
  \end{center}
\end{figure*}


==> ucb_s6.1_EMSynergies.tex <==
\subsubsection{Synergies with EM observations}\label{subsec:synergies}

\noindent \coord{Thomas Kupfer}\\
\noindent \contr{Thomas Kupfer, John Tomsick, Nicole Lloyd-Ronning, John Quenby, Thomas Tauris, Thomas J. Maccarone}
 

%\noindent \contr{Thomas Kupfer, Astrid Lamberts, John Tomsick, Stephan Rosswog, Marica Branchesi, Albert Kong, Nicole Lloyd-Ronning, Samaya Nissanke,  Daryl Haggard, Ashley Ruiter, Fritz Roepke, Shane Larson, Shenghua Yu, Dongliang Liu, Naoki Seto, Jeremy Schnittman, John Tomsick, Gijs Nelemans, Sylvain Chaty,  John Tomsick, John Quenby, Silvia Zane, Kinwah Wu, Matthew Mumpower, Thomas Tauris, Thomas J. Maccarone}\\

Many new verification binaries are expected to be discovered before the launch of LISA, in particular with wide-field optical surveys such as ZTF, BlackGEM and LSST on the Rubin Observatory. Once flying, LISA will be complemented with surveys across different frequency bands (radio to gamma-rays). New sources discovered by LISA can be studied with the next generation of follow-up facilities such as ESO/ELT, CTA, SKA, ngVLA or even Athena as well as smaller space missions which could be approved, built and launched in the early 2030s (eXTP or STROBE-X). This provides a plethora of large-scale follow-up resources for detailed multi-messenger studies but it requires a well planned follow-up strategy to generate the most useful results. 

The large number of facilities running in the 2020s and 2030s will provide a bright future for the research on compact Galactic binaries, with hundreds of additional EM discovered systems ready to be studied in detail through EM+GW observations as soon as LISA is operational. A significant sample of binaries, observed with EM+GW observations, will open up possibilities to explore and study astrophysical phenomena which are crucial to our understanding of the Universe. This includes the long-standing questions of the progenitors of SNe Ia, the formation and evolution of compact objects in binaries and accretion physics under extreme conditions.



\paragraph{UV/Optical/IR observations}

\phantom{text}


Previous studies predict that we will be able to observe several thousand Galactic binaries in both GW and optical emission \citep{2013MNRAS.429.2361L,2017MNRAS.470.1894K}. A subset of the known UCBs have orbital periods that lie in the LISA band and these will be individually detected by LISA due to their strong GW signals, some on a timescale of weeks or a few months. Combined GW and EM multi-messenger studies of UCBs will allow us to derive population properties of these systems such as masses, radii, orbital separations, and inclination angles but in many cases EM observations are required to complement GWs and break degeneracies in the GW data. \citet{2012A&A...544A.153S, 2013A&A...553A..82S, 2014ApJ...791...76S, 2018MNRAS.480..302K} present several studies on how EM observations can complement LISA GW data and vice versa. The GW amplitude and inclination is strongly correlated, but the GW amplitude can be improved by a factor of six when including EM constraints on the inclination and the sky position and inclination can reduce the uncertainty in amplitude by up to a factor of 60 \citep{2014ApJ...791...76S}. 

Additionally, knowing the distance from EM, e.g. from parallaxes measured by Gaia, will help to derive a chirp mass from GWs even for non-chirping sources because for many LISA sources only the frequency and amplitude will be measured. This leaves a degeneracy between chirp mass and distance and inclination, since a more massive binary further away can have the same amplitude as a lower mass one that is closer by and inclined systems closer by look like face on systems further away \citep{2012A&A...544A.153S,2014ApJ...790..161S}. 

If the chirp mass has been measured from GWs using e.g.\,Gaia parallaxes and the mass ratio has been measured from EM, through radial velocities or ellipsoidal deformation of one component, both measurements can be combined to the measure the masses of both components with a few percent precision. Comparing the measured orbital decay with the predicted orbital decay from general relativity will allow us to measure the effects of tides compared to GWs. Tides are predicted to contribute up to $10\,\%$ of the orbital decay \citep{2011ApJ...740L..53P} but has not been measured so far and is very difficult with GW and EM alone. Some of the known AM\,CVn and detached WD+WD binaries have well constrained distances from Gaia \citep{2018MNRAS.480..302K, 2018A&A...620A.141R}. Measuring the distance from EM constrains the uncertainty in chirp mass to 20\%, whereas adding the period derivative $\dot{P}$ reduces it to 0.1\% (see e.g.\,Fig.~\ref{fig:f-dot}). A GW chirp mass measurement would provide the first detection of tidal heating in a merging pair of WDs from the deviations in predicted $\dot P$ \citep{2014ApJ...791...76S}. With a large enough sample of WD+WD binaries whose chirp masses can be determined, we can plausibly extract constraining information about CE phase evolution physics. In studying massive WD+WD binaries that are likely progenitors of merger-induced collapse NSs \citep{2019MNRAS.484..698R}, chirp mass distributions had different shapes depending on the adopted CE phase prescription in the binary evolution population synthesis model. 


Several studies have shown that spectral and photometric analysis of detached WD+WD can provide precise sky positions, orbital periods and in some cases mass ratios, inclinations, and the rate of orbital period decay \citep[e.g.][]{2002MNRAS.332..745M,2011ApJ...737L..23B, 2012ApJ...757L..21H, 2019Natur.571..528B}. All of the known verification binaries have precise sky positions and orbital periods and five systems have a measured orbital decay from photometric monitoring \citep{2018MNRAS.480..302K}.  SDSSJ0651, a 12 min orbital period detached WD+WD \citep{2011ApJ...737L..23B}, and ZTFJ1539, a 7 min orbital period detached WD+WD \citep{2019Natur.571..528B}, are prime example of what can be accomplished. Using only one year of eclipse timing measurements, \citet{2012ApJ...757L..21H} found an orbital decay of $\dot{P} = (-9.8\pm 2.8)\times 10^{-12}$\,s\,s$^{-1}$ in SDSSJ0651 which has not been updated since then. \citet{2019Natur.571..528B} used photometric data from PTF/iPTF and ZTF covering a total of ten years and measured a very precise orbital decay of  $\dot P = (-2.373\pm0.005)\times 10^{-11}$\,s\,s$^{-1}$. However, neither of the two systems has a precision of WD component masses good enough from optical observations to see if their $\dot{P}$ differs from the predictions of the theory of General Relativity (GR). GW observations can solve that. Tidal theory predicts a 10\% deviation from GR if the WDs are tidally heating up.  Which means that combining EM+GW observations from LISA will allow a measurement of the amount of tidal heating in these merging pairs of WDs for the first time.

Combined EM+GW observations of the Galactic WD+WD population will help to solve another major problem in astrophysics: the SNe\,Ia progenitor problem. Although only the thermonuclear explosion of a WD following the interaction with a binary companion can explain the observed features in the SN light, much less is known about their progenitors. Recent results have shown that SN\,Iae show a large range of explosion energies and decay times, photometric and spectroscopic signatures indicating different progenitor systems \citep{2019NatAs...3..706J}. Several different explosion scenarios are under discussion, including the merger and subsequent explosion of an ultra-compact WD+WD system (double-degenerate model) or the explosion triggered by ignition of an helium shell accreted from a helium star in a UCB (double-detonation scenario). However, the number of known progenitor systems is limited. \citet{2019MNRAS.482.3656R} studied the probability of finding WD+WD progenitors of SNe\,Ia using a binary population synthesis approach, and found that the chance of identifying such progenitors purely in EM data is $\sim10^{-5}$. These include both double-lined spectroscopic binaries and the eclipsing systems. Even with the next generation of 30\,m class telescopes, the probability for detection only goes up by a factor of $\sim10$. \citet{2017MNRAS.470.1894K} predicts that LISA will individually resolve $\sim25,000$ detached WD+WD systems including the most massive systems. EM follow-up observations in combination with GW measurements will allow us to measure masses of individual systems and find and characterize the population of double degenerate SN\,Ia progenitors. 

Kilonovae \citep[see][]{2019LRR....23....1M} are optical/IR emission accompanying the merger of NS+NS, possibly NS+BH, and in special cases, WD+WD mergers \citep{2019JCAP...03..044R}. Although LISA is not sensitive to the actual merger that can produce a kilonova, it is sensitive to the GW emission from their progenitors. Therefore it is worthwhile to consider kilonova events in the nearby universe because they allow constraints on these degenerate stellar populations. 

\paragraph{X-ray observations}

\phantom{text}


Many of the LISA sources also emit X-rays, thus allowing for a number of joint LISA + X-ray investigations. The donor stars in UCXBs appear to be a mixture of C/O-core and He-core WDs and abundance measurements can help identify their formation scenario \citep{2010MNRAS.401.1347N}. In the oxygen-rich systems, oxygen is the dominant coolant in the accretion discs, and the iron emission lines are suppressed; the strength of the iron lines is broadly in agreement with the thermonuclear burst properties of the sources, strengthening the case that this donor classification process works reasonably well even in its simplest form \citep{2020arXiv200100716K}. However, in some cases, the abundances of the WD inferred from X-ray data are at odds with those inferred from Type I burst properties. In a few cases, the inference has been made from neon-to-oxygen rations \citep{2001ApJ...560L..59J}, and for this scenario, it has been shown that there is a channel of binary evolution that allows a He-core WD to have such neon-to-oxygen ratios \citep{2005A&A...441..675I}.  Alternatively, \citet{1992ApJ...384..143B} show that spallation of CNO elements in a NS atmosphere is quite likely. The combination of LISA measurements with X-ray (and optical) abundance measurements thus opens a window to determining which of these scenarios is correct.  If the apparent C/O-core WD donors are paired with high mass NSs, then the spallation scenario is strongly preferred. 

More detailed X-ray spectroscopy should potentially be able to make detailed abundance estimates for the donor stars, allowing, e.g., identification of systems in which the CNO processing may not have gone to completion, and perhaps estimating the time of formation through estimates of the abundances of non-CNO elements, which could yield the initial metallicity of the star. The X-ray measurements are essential given that a large fraction of the UCXBs are located in globular clusters, or deep in the Galactic Plane where ultraviolet and optical spectroscopy are more challenging. Substantive work has also been done in the optical wavebands \citep[see e.g.][]{2004MNRAS.348L...7N, 2006MNRAS.370..255N}.  Furthermore, when combined with LISA data the UCBs then may provide a means of testing how conservative accretion onto NSs is; C/O-core WD donors must start at masses of at least $\approx0.5 M_\odot$, but are generally observed with masses of $0.1\,M_\odot$ or less.  If the early stages of mass transfer in these systems are conservative, the NSs should typically be about $1.8\,M_\odot$, while if they show much lower masses, this implies that the mass transfer was strongly non-conservative.

Additionally, for 4U~1820$-$30, X-ray measurements provide a straightforward way to monitor the source's period derivative \citep{1991ApJ...374..291T}, as the source is deep in the potential well of a globular cluster whose gravitational acceleration leads to its negative period derivative.  It is easy to track the source's orbital period in the X-ray band \citep{1987ApJ...312L..17S,1991ApJ...374..291T}, and hard in other bands, due to the crowding in the cluster. With more intensive X-ray data, the period derivative of 47~Tuc~X-9, the best candidate BH+WD binary in the Milky Way \citep{2017MNRAS.467.2199B}, could be tracked.  Imposing these constraints, which are likely to lie outside the range of normal templates, can help improve the quality of the LISA GW detection.  Globular clusters are likely good hosts for LISA sources, but the globular cluster sources' periods have come from ultraviolet photometry \citep{2005ApJ...634L.105D,2009ApJ...699.1113Z} and the best non-cluster source's period comes from optical spectroscopy \citep{2013MNRAS.429.2986M}. Additional intensive monitoring campaigns would be required for the period derivative to be estimated.


For the AM~CVn systems, X-ray emission is also valuable.  The same abundance issues can be studied in the X-ray band in AM~CVn systems, although primarily from the emission lines from the boundary layer of the accretor, rather than disc reflection.  Relatively short period AM~CVn systems will be detectable to large distances, where reddening may be important, and in these cases, restricting the set of sources to those which are in a reasonable range of fluxes.  For the faintest AM~CVn sources with periods less than half an hour, the X-ray luminosities are typically about $10^{31}$ erg\,s$^{-1}$ \citep[e.g.][]{2004MNRAS.349..181N,2004ApJ...614..358S, 2005A&A...440..675R, 2006A&A...457..623R, 2016MNRAS.460.3660Z}, meaning that eROSITA should detect them to distances of about 3~kpc.  Combining with radio surveys to remove background Active Galactic Nuclei (AGN), and optical surveys to remove foreground stars and CVs should then yield a much more manageable list of candidates for high time resolution optical follow-up (which usually has limited fields of view) than without the X-ray data and  potentially add more LISA verification sources.

X-rays are also likely to provide the best EM distance estimators for many of these UCXBs (see Fig.\,\ref{fig:LMXB-UCXB-link})  complementing LISA data. Some are located in globular clusters, where the cluster distance can be used. None of the Galactic field UCXBs is bright enough for Gaia in the optical, and most are also too faint for radio parallaxes with current facilities.  Thermonuclear bursts with radius expansion can be used to estimate the Eddington luminosities \citep{2003A&A...399..663K}, and these can then be used in conjunction with the GW estimates of the masses to establish self-consistent properties for the sources.  For the persistent sources that burst in an appropriate manner, these data are already in hand, but obtaining such data for transients would require instruments with large collecting area and small deadtime \citep[e.g.\,NICER, STROBE-X, eXTP][]{2016SPIE.9905E..1HG, 2019arXiv190303035R, 2019SCPMA..6229502Z}.\footnote{most imaging X-ray telescopes will not be able to make such measurements because of pile-up or deadtime issues.}  The other approach that can be used to estimate distances is that of dust-scattering halos \citep{1973A&A....25..445T}, something that requires good angular resolution, good collecting area, and the ability to observe bright sources; while Chandra has done some work in this area, Athena should be able to help dramatically \citep{2019ApJ...874..155C}.

Some UCXBs may contain BHs as well. The first strong globular cluster BH candidate \citep{2007Natur.445..183M} in NGC~4472 is an ultracompact system \citep{2008ApJ...683L.139Z}, probably with an orbital period near 5 minutes, and 47~Tuc~X-9 \citep{2015MNRAS.453.3918M,2017MNRAS.467.2199B} is also a strong candidate ultracompact BH X-ray binary.  At the shortest orbital periods, BH+WD binaries should be detectable by LISA to distances of a few megaparsecs.  For these cases, imaging X-ray data would be needed, along with follow-up optical spectroscopy to look for [O III] nebulae as well as hydrogen emission similar to that in the globular cluster RZ~2109 in NGC~4472 \citep{2008ApJ...683L.139Z,2014ApJ...785..147S,2019MNRAS.489.4783D}.  In the Milky Way, UCXBs with BH accretors at relatively long orbital periods could be quite faint X-ray sources in quiescence (being considerably fainter than accreting NSs at the same mass transfer rate due to advection dominated accretion, \citealt{1994ApJ...428L..13N}). They could also exhibit only rare outbursts, meaning that sensitive X-ray observations would be needed to detect their counterparts.  Furthermore, these objects may be preferentially in globular clusters, meaning that excellent angular resolution, from Chandra or a Chandra successor mission like Lynx or AXIS would be needed to find their counterparts.  If some new BH UCXBs are discovered with X-ray outbursts, they may become bright enough to make BH spin estimates using reflection and/or disc continuum modelling.

For most of the topics related to accretion, there is a need for developing better spectral models that treat unusual abundances.  Development of reflection models that include both the reflection from the surface of the WD, and discs made from hydrogen-poor material is thus vital. It has already been found that details of how atomic physics is incorporated into the disc models can affect inferred spins and abundances \citep{2016MNRAS.462..751G,2018ApJ...855....3T}.

X-ray observations are also vital for understanding the detached systems with NS members.  In most of these systems, the older NS will have experienced significant spin-up, and will be a millisecond pulsar.  Pulsar beam opening angles are larger at high energy than at radio wavelengths (a phenomenon exhibited by objects like Geminga \citep{1992Natur.357..222H} and many of the Fermi-discovered pulsars), meaning that some fraction of these objects will be radio-quiet pulsars \citep{2015ApJ...802...78M}.   X-ray observations will then provide the most comprehensive means for estimating the spins of these systems and determining what fraction of them have become recycled.  Furthermore, in combination with radio searches for pulsations, having a gravitationally-selected sample will allow a clean determination of the ratio of pulsars with radio and X-ray emission, allowing an important constraint for developing a full picture of the pulsar beam geometry.  In an ideal case we may identify an object with thermal cap emission from the NS, such that pulse-profile measurement and modelling could be done to estimate its radius.  If this comes in conjunction with sufficiently good LISA GW measurements to provide an independent, precise, estimate of the NS's mass, this would give a constraint on the equation of state for NSs, even from a single object \citep{2019AIPC.2127b0008W}.






\begin{figure*}
    \begin{center}
   \includegraphics[width=0.60\textwidth]{./img_ucb/GW_freq_freq_dot_UCXB.png}
   \includegraphics[width=0.60\textwidth]{./img_ucb/DWD-RLO-details-LISA+Gaia.png}
\caption{{\bf Upper panel}: GW frequency derivative, $|\dot{f}_{\rm GW}|$ as a function of GW frequency, $f_{\rm GW}$ for the UCXB shown in Figs.~\ref{fig:UCXB_strain+data} and \ref{fig:UCXB-AMCVn-detailed}. The black coloured points correspond to the inbound leg (orbital shrinking) and the blue points correspond to the outbound leg (orbital expansion, after reaching the orbital period minimum) including mass transfer/loss from the system and finite-temperature effects of the WD donor. Each point represents a binary stellar MESA model. The green solid circle indicates the onset of the UCXB stage. (Before this point, the system is a detached NS+WD binary). Figure from \citet{2018PhRvL.121m1105T}. 
{\bf Bottom panel}: pure general relativistic (GR, blue) and astrophysical (orange) chirps as a function of GW frequency for WD+WD (AM~CVn) systems \citet [Figure from][]{2018ApJ...854L...1B}. The astrophysical contribution from mass transfer and tides leads to a significant deviation from the contribution from GR alone and will cause the systems to widen their orbit upon mass transfer. The decoupling of the astrophysical chirp from the GR chirp will be possible with {\em combined measurements} from LISA and Gaia. The error bars show the anticipated 1$\sigma$ measurement errors. On average, \citet{2018ApJ...854L...1B} find that about 50 AM~CVn systems in the Mikly Way with $P_{\rm orb}<800\;{\rm s}$ have resolvable GR and astrophysically driven chirps.} 
 \label{fig:f-dot}
  \end{center}
\end{figure*}


\paragraph{Radio observations}


\phantom{text}



The synergies from joint, multi-messenger observations of radio pulsar binaries entering the LISA band are very promising and will provide significantly more information than observations in the EM or GW bands alone (see Fig.\,\ref{fig:LMXB-UCXB-link}). Such benefits include better measuring the orbital inclination angle \citep{2012A&A...544A.153S} and sky position \citep{2013A&A...553A..82S} and potentially even constraining the NS mass-radius relation to within $\sim 0.2$\% \citep{2020MNRAS.493.5408T}. Additionally, radio astrometry can give parallax distances out to a few kpc already, and with ngVLA \citep{2018ASPC..517....3M}, that should increase dramatically. Most LISA sources would be nearby enough that with ngVLA, one would be able to get 10\% or better geometric parallaxes over about 3/4 of the sky. 

Binary NSs in NS+NS and NS+WD systems enter the LISA band at a GW frequencey of order $1\;{\rm mHz}$ (depending on their distance), corresponding to orbital periods of about $30\;{\rm min}$.
Doppler smearing of radio pulsations from pulsars in such tight binary orbits \citep{2013MNRAS.431..292E} could cause a selection bias against detection of e.g., rapidly spinning millisecond radio pulsars in many previous and present day acceleration searches (at least for dispersion measures, $< 100\;{\rm cm}^{-3}\,{\rm pc}$). However, using neural networks, \citet{2020arXiv201004151P} develop accurate modelling of the observed binary pulsar population and argue for a $\sim 50$--$80$\% chance of detecting at least one of these systems with $P_{\rm orb}\le 15\;{\rm min}$ using data from surveys with the Arecibo radio telescope, and
$\sim 80$-$95$\% using optimal integration times of $\sim 50\;{\rm s}$ in the next several years. The chances of a radio detection of a binary pulsar in the LISA GW band is expected to be significantly enhanced by the completion of the Square-Kilometre-Array \citep{2015aska.confE..40K}. 

It has been argued \citep{2020arXiv201004151P} that unequal mass NS+WD systems are easier to detect compared to the usually near-equal mass NS+NS systems. It should be kept in mind that RLO from these (often bloated) WD companions begins when $P_{\rm orb}$ has decreased to $25-15\;{\rm min}$, depending on their temperature \citep{2018PhRvL.121m1105T} (see also Figs.~\ref{fig:UCXB_strain+data} and \ref{fig:UCXB-AMCVn-detailed}). This will exclude radio detection of such pulsar binaries once accreted plasma enters the NS magnetosphere.

\paragraph{Particle observations }

\phantom{text}


For high-frequency GW detections, there are prospects for detection of neutrino's or cosmic rays, from jets produced in mergers or from supernovae \citep{2016PhRvD..9312010A}. For LISA, the prospects are not so clear, even though associations of LISA GW sources with AGN jets and tidal disruption events could be possible.


\begin{comment} 
\paragraph{Particle observations }

\paragraph{Neutrino emission}
   
Sufficient rest mass energy is available to allow observable neutrino secondary production, arising from cosmic ray acceleration in relativistic jets, in the coalescence of stellar mass binaries.
Lack of X-ray and gamma-ray signatures from current GW observation
of SMBH merger has highlighted the problem of finding enough mass transfer in accretion flows to make the neutrinos \citep{2016PhRvD..9312010A}.
There is a possibility of neutrino production by cosmic rays in an extreme magnetic field jet, without significant photon flux \citep{2019PhLB..795..425Y}. However, tidal disruption in WD+WDs, NS+WD binaries or if a He poor star is involved is a more promising scenario. The presence of a UCXB would also indicate supply of accretion material at the time of merger. Total WD+WD galactic
merger rate  estimates of $\leq 0.05$\,yr$^{-1}$ means we would be looking for rare events while the predicted small GW amplitudes would require retrospective search for discovering the inspiral history.

Core collapse of massive stars are a source of neutrinos in an energy range detectable by Hyper-kamiokande. After the implosion either the core density increases, making it opaque to thermonuclear neutrinos or MHD processes. This causes an outward bounce, which gives time differences between the GW and neutrino signatures 
of  $\leq0.5$ s \citep{2013NuPhs.235..3810}. With GW power mainly above 1 Hz and a strain  $  \leq 6 \times 10^{-21}$ for an event at 10 kpc,  LISA data would be secondary to second generation detectors for these rare events. Cosmic ray acceleration occurs chiefly in the SN remnant shock wave, but if the collapse results in a magnetar, an initial burst of acceleration is possible.
    

Tidal disruption of a star passing close to a SMBH may produce GW-neutrino association. Optical/UV/X-ray observations have
identified candidate events but the GW are likely to be below the LISA threshold. Evidence of such an event 100 years ago at the
Galactic centre \citep{2017MNRAS.471.3293C} provides a chance of a further, unique observation.

\paragraph{Cosmic ray emission} 

Association of cosmic ray and GW production can only be indirect since the time delay between particle acceleration and arrival in the solar system is determined by magnetic scattering induced diffusion. For example, GW from the birth of the Galactic Geminga pulsar arrived $\sim 100$ years before the $10^{14}$\,eV positrons contributing to this primary cosmic ray flux. The signature of the likely dominant source of $\leq10^{15}$ eV particles is the X-ray flux in expanding supernovae envelopes, but although they are known a few hundred years post-explosion, no similar feature appeared immediately in the case of SN1987a. Particle composition data showing a mixture of interstellar plus SNR material also point to envelope shock origin. SgA* appears to have produced a galactic CR wind in the past.
    
Extragalactic origin of particles $\geq10^{15}$ eV is satisfied energetically by AGN emitting $\sim10^{46}$ erg/s. However, lack of anisotropy in the UHECR flux as seen by the AUGER array leads to the possibility that starburst galaxies in the $\leq10^{41}$ erg/s range are the main source. Discovery of GW and $10^{15}$\,eV neutrinos from identifiable sources would aid the elucidation of extragalactic cosmic ray origin. The blazar TXS 0506+056 is the known example. The remaining $10^{15}$ eV neutrino flux seems too large to correspond to CR secondary production. GWs are expected only in the merger stage of IMBH/SMBHs. The suggestion that gamma ray bursts could also be an important CR source is reinforced since, in common with AGN, their relativistic jets are seats of acceleration at shocks or in large scale electric fields. Long-lived GRB produce higher gamma--ray energies and are related to core collapse SN while short
time scale GRB are attributed to NS merger and X-ray temperatures.
The GW170817 event was correlated with a low luminosity
($10^{46}$ erg rather than the typical $10^{52}$ erg) short lived burst identified as an NS+NS merger. With ejecta moving at only $\sim 0.3$c and a temperature $\sim2$ keV, such events will
only contribute to galactic scale CR fluxes. However, there is the prospect of GW-led searches uncovering significant numbers of similar low luminosity GRB.


\paragraph{Kilonova Emission as a constrain for binary populations} 

We often think about EM observations of GW sources as meaning direct EM observations of LISA observable sources, whether they are synchronous or follow-up. However, it is also important to consider observations in the EM band that are relevant to LISA (and LISA observations that are relevant to EM observers who are planning what to observe) even if we aren't talking about simultaneous observations or observations of the same source.

An example of this important synergy is observations of kilonovae. Emission from ejecta that is heated due to radioactive decay of elements formed in compact object mergers - a kilonova - can provide us with a wealth of information about these systems \cite{2019LRR....23....1M}.  The spectrum and colour of this emission reflects the nucleosynthetic processes in the ejecta, and is related to the the amount of mass ejected, its velocity, and the presence of a wind from the nascent disc. For neutron rich ejecta (in which the electron fraction is low), the r-process can  operate effectively and lanthanides \citep{2016ApJ...833..282M, 2020arXiv200604322V} as well as actinides \citep{2018ApJ...869...14M, 2019JPhG...46f5202V, 2019ApJ...881....5H} are produced. Lanthanide-rich ejecta is opaque to higher energy photons (in the UV/optical continuum) and therefore emission from this ejecta has a redder spectrum \citep{2013ApJ...774...25K, 2013ApJ...775...18B, 2017Natur.551...80K}.  Alternatively, when the electron fraction is high, the synthesis of the elements via the rapid neutron capture (r-process) is suppressed and the bluer photons can escape.  If the event is close by, concurrent observations of X-rays and $\gamma$-rays can point to the distinct composition of nucleosynthesis \cite{2020ApJ...889..168K, 2020ApJ...899...24E, 2020arXiv200803335W}. In particular, an enhancement in an observed light curve around 60 to 100 days provides smoking-gun evidence of the production of $^{254}$Cf \citep{2018ApJ...863L..23Z}.  The details of the processes that play a role in the emission spectrum of kilonova - from atomic opacities to accurate determinations of the electron fraction based and properly accounting for weak interactions in the system as a whole - are yet to be determined. 

Although LISA is not sensitive to the actual merger that can produce a kilonova (NS+NS, NS+BH, and in special cases, WD+WD mergers \citep{2019JCAP...03..044R}), it is sensitive to the GW emission from their progenitors. Therefore it is worthwile to consider kilonova events in the nearby universe because they allow constraints on these degenerate stellar populations. 







    
\end{comment}





==> ucb_s6.2_GWSynergies.tex <==
\subsubsection{Synergies with other GW  detectors}


\noindent \coord{Lijing Shao; Paul Groot} \\
\noindent \contr{Ilya Mandel (1.5.2.1), Alberto Sesana, Emanuele Berti, Lijing Shao (1.5.2.4), Davide Gerosa (1.5.2.1), Pau Amaro Seoane, Paul Groot, Thomas Tauris (1.5.2.2), Valeriya Korol (1.5.2.3)}

\paragraph{High-frequency GW merger precursors seen by LISA \label{paragr:highFreqGW}}


\phantom{text}



LISA has a unique capability of covering the full frequency spectrum for stellar-mass binary BHs and NSs when combined with the higher-frequency ground-based GW  detectors 
advanced LIGO \citep{AdvLIGO} and Virgo \citep{AdvVirgo}, and their third generation successors such  as the proposed Einstein Telescope \citep{2010CQGra..27h4007P} and Cosmic Explorer \citep{2017CQGra..34d4001A}. 


Some individual sources can be tracked on human timescales from the LISA band to the $\gtrsim$ few Hz ground-based detector sensitive frequency band \citep{2016PhRvL.116w1102S}.  The GW  driven merger timescale for a circular binary with components of equal mass $m$ from a starting frequency $f$ is~\citep{1964PhRv..136.1224P}
\begin{equation}
\tau_\mathrm{GW} \simeq 5 \left( \frac{f}{0.01\ \mathrm{Hz}} \right)^{-8/3} \left( \frac{m}{68\ M_\odot} \right)^{-8/3}\ \mathrm{yr}.
\end{equation}
Thus, a signal like GW190521 \citep{2020PhRvL.125j1102A} could be tracked from 10 mHz to merger across the the full range of frequencies with the combination of LISA and ground-based detectors. Rate estimates have been presented by \citet[][]{2015Sci...349.1522S,2016MNRAS.462.2177K,2016PhRvL.116w1102S,2017JPhCS.840a2018S,2019PhRvD..99j3004G,2019MNRAS.488L..94M}, with predictions ranging from  0 to roughly a dozen detections during the LISA mission.

The high mass and correspondingly rapid orbital evolution of IMBHs with masses in the $100$--$1000\ M_\odot$ range makes them particularly appealing targets for tracking across the LISA and ground-based detector frequency bands.  IMBHs with these masses are a challenge for EM observations: their dynamical signature is relatively insignificant, while their X-ray emission can be confused with that of super-Eddington accretors \citep[e.g.,][]{MillerColbert:2004,2011NewAR..55..166F, 2019arXiv191109678G}.  On the other hand, IMBH mergers have been proposed in the context of both isolated binary evolution of very massive stars \citep{Belczynski:2014VMS} and globular cluster dynamics \citep{Amaro:2006imbh}.  The latter can also be responsible for intermediate-mass ratio inspirals of stellar-mass compact objects into IMBHs \citep{Mandel:2008,2016ApJ...832..192H}.  Meanwhile, hierarchical mergers of few-hundred $M_\odot$ seeds have been proposed as seeds of today's massive BHs \citep[][see Chapter~\ref{MBH_chapter}]{2003ApJ...582..559V}. Joint observations with LISA and third-generation ground-based detectors \citep{2011PhRvD..83d4036S,2011GReGr..43..485G} would provide the perfect tools for studying these elusive IMBHs.   

Observations of the same individual source across a broad range of frequencies can improve the accuracy of source parameter measurement. Some parameters are likely to be best measured at low frequencies.  For example, sky localisation accuracy depends on timing precision \citep{Fairhurst:2009,2010PhRvD..81h2001W,Grover:2013}.  The sky localization accuracy can be estimated as the timing accuracy divided by the light travel time across the detector baseline \citep{Mandel:2017}, which is $\sim$ astronomical unit (AU) for LISA, yielding a relative position error of:
\begin{equation}
\sigma_\theta \sim 0.025 \;\left(\frac{0.01\ \mathrm{Hz}}{f}\right) \,\left(\frac{8}{\rho}\right),
\end{equation}
where $\rho$ is the detection signal-to-noise ratio. For heavier sources that can evolve faster than the LISA observing duration, the LISA frequency bandwidth $f_\mathrm{bandwidth}$ should be used in place of $f$.  The angular resolution scales inversely with baseline.  Therefore, despite the lower observing frequency (lower bandwidth), for high SNR sources, LISA sky localisation is likely to be superior to the capabilities of ground-based detectors, whose baseline, even in a network, is limited by the size of the Earth (unless the signal is sufficiently long-lived to allow the effective baseline to be extended by the detector motion over the duration of the observation).

On the other hand, some source parameters will be better measured at higher frequencies, allowing ground-based detectors to provide complementary information to LISA observations.   These include measurements of the ringdown of the post-merger BH, which yield the final mass and spin, and the tidal effects for NSs.  

Yet other measurements could benefit from the joint constraints placed by low-frequency and high-frequency observations.  These include measurements of spin magnitudes and spin-orbit misalignment angles, which could carry information about formation scenarios \citep[e.g.,][]{2013PhRvD..87j4028G,Vitale:2015,Stevenson:2017spin,Zevin:2017,Farr:2017,2018PhRvD..98h4036G}.   Spin-orbit and spin-spin coupling enter the waveform at higher post-Newtonian orders in an expansion in the orbital frequency \citep{PoissonWill:1995}, and so may be better measured at higher frequencies by ground-based detectors.  On the other hand, massive binaries like GW190521 may spend a million cycles in the LISA band (only 4 cycles were observed in the LIGO band when this signal was detected in 2019; \citealt{2020PhRvL.125j1102A}).  Further analysis is necessary to explore the quantitative benefits of LISA for parameter estimation of such signals \citep[but see e.g.][]{2016PhRvL.117e1102V,2019MNRAS.488L..94M,2019PhRvD..99f4056M,2019BAAS...51c.109C}

Lower-mass GW  sources such as double NSs \citep{2020MNRAS.492.3061L,2020ApJ...892L...9A} will not be individually trackable on a human timescale from the LISA band to the band of ground-based detectors.  However, they may still benefit from tracking the entire population of sources as the sources evolve from the LISA frequency band to the frequency band of ground-based detectors.  For example, binaries circularise through GW emission (very roughly, the eccentricity scales inversely with the increase in frequency), making eccentricity challenging to observe with ground-based detectors \citep[e.g.,][]{RomeroShaw:2019,2020MNRAS.497.1966L}.  Thus, LISA observations at lower frequencies, where eccentricities are still significant, could help to distinguish compact binary formation scenarios \citep{2016ApJ...830L..18B,2016PhRvD..94f4020N,2017MNRAS.465.4375N}.  

This can be further aided by the detection of a stochastic  background from a superposition of GWs emitted by multiple individually unresolvable binaries (see Section~\ref{subsec:SGWB}) .  For circular binaries, the stochastic background should be a simple power-law in frequency, and any deviations from that could indicate the emergence of new binaries, particularly eccentric binaries, at high frequencies.  Moreover, the combined low-frequency and high-frequency stochastic background observations may make it easier to subtract the astrophysical background and reveal a possible GW  background of cosmological origin  \citep[e.g.][]{Mandic:2012,Lasky:2016,Callister:2016}.

LISA precursors to ground-based detector mergers could also have important repercussions in fundamental physics, allowing stringent tests of the BH no-hair theorems, as well as more stringent bounds on low-Post-Newtonian deviations from GR \citep{2020PhRvD.101j4038T,2016PhRvL.116x1104B,2019PhRvD..99l4043T,2019PhRvD.100f4024G,2020CQGra..37bLT01C,2017PhRvX...7d1025S}.


\paragraph{Dual-line GW sources}

\phantom{text}


A possibility in upcoming GW astronomy will be the potential discovery of a {\em dual-line} Galactic GW source \citep{2018PhRvL.121m1105T}, where ground-based detectors detect the continuous high-frequency GW emission from the rapid spinning (recycled) NS \citep{2019gwa..book.....A} and LISA simultaneously detects the gravitational damping of the system's orbital motion via continuous low-frequency GW emission. Such a system could very well be a UCXB \citep[e.g.][]{2012A&A...537A.104V,2013ApJ...768..184H}.
Combining the expressions for the strain amplitudes of the ground-based and LISA observations ($h_{\rm spin}$ and $h_{\rm orb}$ respectively) yields \citep{2018PhRvL.121m1105T}:
\begin{equation}
    I_{zz}\,\varepsilon = \sqrt{\frac{2}{5}}\,\left(\frac{\sqrt{G}}{2\pi}\right)^{4/3} \left(\frac{f_{\rm orb}^{1/3}}{f_{\rm spin}}\right)^2\,\mathcal{M}^{5/3}\,\left(\frac{h_{\rm spin}}{h_{\rm orb}}\right).
\end{equation}
Once the right-hand-side of this equation is determined observationally, and assuming that the NS mass, $M_{\rm NS}$ can be determined from the chirp mass, $\mathcal{M}$ \citep[see required assumptions on component mass determinations in][]{2018PhRvL.121m1105T}, constraints can be made on the NS moment of inertia, $I_{zz}$, and thus the NS radius \citep{1994ApJ...424..846R}. \citet{2021MNRAS.503.5495S} recently examined the dual-line detectability of tight Galactic binaries, and found that at least two of the known systems (4U 1820-30 and 4U 1728-34) may be visible to both ground-based and space-based instruments simultaneously. Although only measuring the moment of inertia in combination with the ellipticity, $\varepsilon$, it will still help in pinning down the long sought-after equation of state (EOS) of NS matter. The maximum spin rate and $\varepsilon$ for accreting NSs \citep[][]{2019gwa..book.....A} remain to be constrained firmly. 


\paragraph{TianQin}

\phantom{text}


TianQin is a space-based GW observatory conceived as an equilateral triangle constellation of three drag-free satellites with frequency sensitivity at $10^{-3} - 10^{-1}\,$Hz \citep{2016CQGra..33c5010L}, between LISA and DECIGO. 
Unlike LISA, TianQin will follow a geocentric orbit with a radius of about $10^5$\,km \citep{2018CQGra..35i5008H,2019IJMPD..2850121Y}. Its constellation plane will be nearly perpendicular to the ecliptic plane and will have a fix orientation pointing toward RX J0806.3+1527 \citep{2005ApJ...627..920S}, a $5\,$min orbital period Galactic binary that is expected to be the strongest GW source among currently known systems \citep{2018MNRAS.480..302K}. Planned for the launch around 2035, TinQin will see the same GW sources as LISA \citep{2020arXiv200810332M}. Consequently, many synergies can be envisioned between the two missions. For instance, TianQin and LISA will simultaneously detect several thousand Galactic WD+WD binaries, which will improve the parameters estimation including the amplitude, inclination and sky localisation for these binaries \citep{2020arXiv200507889H}. 

\paragraph{Mid-band observatories, e.g. DECIGO}

\phantom{text}


After the discovery of GW150914~\citep{2016PhRvL.116f1102A}, it was realized that massive stellar-mass BHs will be detectable in both LISA and LIGO/Virgo bands~\citep{2016PhRvL.116w1102S,2010ApJ...722.1197A}. However, the SNRs are not expected to be large in the mHz band, and because of the use of template bank searching, in order to claim a confident detection, BH+BH signals in LISA require a larger SNR threshold than 15~\citep{2019MNRAS.488L..94M}. Fortunately, these sources will have large SNRs if they are seen in the decihertz band~\citep{2018PTEP.2018g3E01I, 2019arXiv190811375A, 2020MNRAS.496..182L}. DECihertz laser Interferometer Gravitational wave Observatory (DECIGO) is a representative GW detector in the relevant frequency band~\citep{2011PhRvD..83d4011Y, 2011CQGra..28i4011K, 2020arXiv200613545K}. Studies showed that, not only will observations in the decihertz band provide profound insights to astrophysics \citep[see][for a comprehensive discussion]{2019arXiv190811375A}, they will also provide unprecedented playgrounds for fundamental physics (e.g. testing the dipolar radiation~\citep{2016PhRvL.116x1104B, 2020MNRAS.496..182L}. The mid-band observations of decihertz frequency are natural means to bridge the gap between LISA and LIGO/Virgo observatories.





==> ucb_s7_Technical.tex <==
\noindent \coord{Irina Dvorkin}\\
\noindent \contr{Emanuele Berti, Sylvain Chaty, Astrid Lamberts, Alberto Sesana, Kinwah Wu (1.6.3), Shenghua Yu, Shane Larson, Irina Dvorkin (1.6.1, 1.6.3, 1.6.5), Kinwah Wu \textcolor{blue}{already cited above}, Pau Amaro Seoane, Giuseppe Lodato, Xian Chen, Valeriya Korol (1.6.2), Silvia Toonen (1.6.5)}

\subsubsection{How to distinguish between different compact binaries? } 


One of the outstanding challenges of LISA will be to analyze a datastream that consists of multiple overlapping signals from astrophysical and possibly cosmological sources as well as instrumental noise. Since many LISA sources will remain in band for multiple orbits, from several days or months up to the entire duration of the mission, there will be an overlap between multiple sources in any given data stretch. Data analysis techniques suitable for this unique problem are currently under development, including in the context of the LISA Data Challenge \citep{2010CQGra..27h4009B,2020PhRvD.101l4008C,2020PhRvD.101l3021L}.
A standard procedure that allows us to extract WD+WD signals from a noisy datastream uses waveform templates that span a large parameter space \citep{1996PhRvD..53.6749O}. The most studied case (and the only class detected so far by LIGO-Virgo) is that of isolated compact binaries (see Section~\ref{subsubsec:detached-binaries}), which are characterized by the component masses, the distance to the binary, its position on the sky and the orbital eccentricity, as well as the orbital frequency. Contrary to the case of ground-based interferometers, these binaries are long-lived LISA sources. In other words their orbital evolution timescale due to the emission of GW is very slow compared to the mission duration. This will allow us to collect data from many cycles of each binary, increasing the SNR, but also puts stringent requirements on the accuracy of the template waveform. The waveform of quasi-monochromatic sources, such as WD+WD binaries, is relatively simple and can be quite accurately described by the leading order terms in the orbital dynamics \citep{2020PhRvD.101l3021L}. On the other hand, binaries that evolve in the LISA band (such as BH+BH) require a more detailed computation to higher Post-Newtonian order  \citep{2019PhRvD..99f4056M}. Accurate waveform templates are crucial for measuring the source parameters and distinguishing between various source classes since any error in the predicted phase of the template waveform will accumulate over the many cycles the binary stays in band.

The main parameter that can help to distinguish the different classes of isolated compact binaries is the chirp mass of the system. In order to establish the class of a quasi-monochromatic source one may use the fact that the chirp mass distribution of WD+WD binaries peaks around $\simeq 0.25M_{\odot}$ \citep{2017MNRAS.470.1894K} with the tail up to 1 M$_\odot$, while the chirp mass of NS+NS systems is expected to lie around $\simeq 1.2 M_{\odot}$. 
BH+NS and BH+BH systems will have higher chirp masses. However, high-mass WD+WD systems at the tail of the distribution with chirp masses of up to $\simeq 1.2M_{\odot}$ may be confused for a NS+NS or a NS+WD binary. Similarly, BH+NS binaries may be confused with NS+NS if the NS has an extremely high mass, or the BH has an extremely low mass. Indeed, the discovery by LIGO-Virgo of GW190814, a binary consisting of a $23M_{\odot}$ BH and a $2.6M_{\odot}$ compact object \citep{2020ApJ...896L..44A} is very difficult to interpret: the secondary component is either the lightest BH or the heaviest NS discovered to date. 

Additional clues as to the identity of the source are somewhat model-dependent, although priors from copious ground-based observations will help with NS+NS, NS+BH, BH+BH scale events. Thus, it may be possible to use eccentricity measurements to distinguish between WD+WDs and NS+NSs \citep{2020MNRAS.492.3061L}. Since WD+WDs are expected to have  formed  via  isolated  binary  evolution, their progenitors are expected to have circularised via multiple mass transfer episodes (see Sec.~\ref{paragr:DWD-formation}). This assumption is supported by the lack of observed eccentric galactic WD+WD binaries. On the other hand, NS+NSs in the LISA band could have measurable eccentricities: e.g. in the fiducial model by \citet{2020MNRAS.492.3061L} half of LISA NS+NS sources have eccentricities $e>0.1$. Thus, a detection of an eccentric source with chirp mass of around $\simeq 1.2M_{\odot}$ can be interpreted as a likely NS+NS. Nevertheless,  some rare eccentric WD+WD can be produced in globular clusters of the Milky Way, or via triple interactions \citep[e.g.][]{2018PhRvL.120s1103K}. 


The case of interacting binaries (see Sec.\,\ref{subsubsec:interacting-binaries}) is potentially even more complex, since their orbital evolution is influenced not only by gravity, but also mass transfer and magnetic braking, which lead to  qualitatively different waveforms (such as anti-chirping phases) depending on the evolution stage of the binary \citep[e.g.][]{2017ApJ...846...95K, 2018PhRvL.121m1105T}. For example, as discussed in Sec.\,\ref{paragr:UCXBs} and \ref{paragr:AM-CVns}, AM CVns and UCXBs can be detectable by LISA either during their inspiral phase (when the binary components are detached and the orbits shrinks) or during mass transfer (when the orbit expands). The upside of this complexity is that anti-chirping signals are easier to distinguish from isolated compact binaries. 


Clearly, an EM counterpart to a GW detection will help to identify the source. Indeed, as discussed in Sec.\,\ref{subsec:synergies}, EM observations can help in distinguishing between interacting and isolated sources, as well as identifying NS+NS or BH+NS binaries. For the technical aspects of EM synergies, see Sec.\,\ref{subsec:synergies}. 






\subsubsection{Foreground sources}\label{paragr:foreground} 

\label{subsubsec:GWforeground}

    The Milky Way hosts a large variety of stellar binaries (Section~\ref{subsec:classes-binaries}), numbering in the millions below mHz frequencies (Table~\ref{tab:absolute_n_MWG}). 
    They will appear as nearly monochromatic (constant frequency) sources emitting over the whole duration of the mission (continuous GW sources). Up to tens of thousands - those with frequencies larger than a few mHz and/or located closer than a few kpc -  will be individually resolvable. The rest of Galactic binaries will blend together into the confusion-limited foreground that is expected to affect the LISA data stream at frequencies below 3 mHz \citep[e.g.][]{1997CQGra..14.1439B,2005PhRvD..71l2003E,2010ApJ...717.1006R,2017JPhCS.840a2024C}. 
    The optimal detection, characterization, and subtraction of Galactic binaries from the data stream has been recognized as one of the fundamental tasks for the LISA analysis. Over-fitting the population of Galactic binaries can result in a large contamination fraction in the catalogue of detected sources, while under-fitting it can degrade the analyses of extra-galactic GW sources in the data due to the excess residual.
    
    The waveforms for Galactic binaries are well predicted using only leading order terms for the orbital dynamics of the binary \citep{1963PhRv..131..435P} and can be computed at low computational cost using a fast/slow decomposition of the waveform combined with the instrument response \citep{2007PhRvD..76h3006C}. Nevertheless, their identification in the LISA data will be laborious due to the sheer number of sources expected to be in the measurement band ($\sim 10^4$) and the large number of parameters required to model each source (between 5 and 10, depending on if the source is chirping and if spins are important in the modelling of one or both of the components). In addition, the high density of Galactic binaries in the LISA band (to the extent that sources are overlapping) and the modulation effects caused by LISA’s orbital motion, which spreads a source’s spectral power across multiple frequency bins, makes the true number of signals at a given frequency difficult to identify. Several techniques have been developed to address this challenge.
    
    {\it A hierarchichal/iterative scheme}. The detectable binaries can be identified by using an iterative process that utilizes a median smoothing of the power spectrum to estimate the effective noise level at each iteration, regresses binaries from the data with signal-to-noise ratios above the established threshold as detected sources, repeating the process until the convergence \citep[]{2003PhRvD..67j3001C,2006PhRvD..73l2001T,2012ApJ...758..131N}.
    {\color{blue} However, each iteration can leave behind some residual due to ``imperfect subtraction'' that can affect further analysis and bias parameter estimation.  In practice, the stochastic signal is not actually subtracted but rather included in the covariance matrix during the likelihood calculation. }
     
    {\it Global fit}. A number of studies show that a global fit to the resolvable binaries, while simultaneously fitting a model for the residual confusion or instrument noise and using Bayesian model selection to optimize the number of detectable sources can provide an effective solution to the Galactic {\color{blue}binaries challenge 
    \citep{2005PhRvD..72d3005C,2005PhRvD..72b2001U}. These} global fit methods have been demonstrated on the Galactic binaries using data from the LISA Data Challenges \citep{2020PhRvD.101l3021L}, but work still needs to be done to extend this into a fully-developed analysis pipeline with the full variety of overlapping LISA sources.

It should be noted that there will possibly be SGWBs of unresolved extragalactic sources or of cosmological origin (see Section~\ref{subsec:SGWB}). Such backgrounds will similarly be a broadband confusion signal, and similar considerations to identify and characterize SGWB in LISA data may be needed in order to reveal some of the fainter signals from astrophysical and cosmological sources. Techniques to identify and subtract the SGWB in LISA data are currently being developed by several groups  \citep{2019arXiv190609027K,2019JCAP...11..017C,2020JCAP...07..021P}.







\subsubsection{Tools}
\label{subsubsec:codes}



\paragraph{Modelling isolated binary evolution and populations}

\phantom{text}


The long-term evolution of stars and binaries is typically modelled in either of two methods; by solving the stellar structure equations, i.e. referred to as detailed calculations, or by faster approximate methods typically aimed at the population synthesis approach.
The latter either interpolates in a grid of detailed calculations or uses parametrised stellar evolution tracks which are fitted to detailed calculations. The advantage of this method is the highly boosted  computational speed (the simulation of the evolution of a single binary takes a fraction of a second in stead of hours or days), at the cost of detail; one only has access to those parameters included in the grid of tracks. Due to the speed,  the effect of different assumptions for poorly understood stellar physics (e.g., stellar mass-loss, interaction physics, supernova kick physics) can be tested in a statistical way, which leads to a deeper understanding of the underlying physical processes involved. The population synthesis approach has proven to work  well in retrieving the general characteristics of large binary populations \citep{2014A&A...562A..14T} and has led to many insights in binary evolution. 







Population synthesis codes are crucial for LISA science, both in order to make forecasts for source rates, but also to develop data analysis pipelines. Indeed, ongoing work on building fast and reliable waveforms relies on the knowledge of the expected properties of the sources (masses, spins, eccentricities) and the accuracies required to detect them and measure these properties. The codes currently in use by the LISA community are listed in Table\,\ref{table:pop-synth}. 
 Further development of these codes, in particular the inclusion of additional physical processes as well as cross-checks between the codes will help to prepare for LISA observations. 


\begin{table}
\caption{Population synthesis codes used by the community at the time of writing. Binary\_c, COSMIC, MOBSE are based on the BSE code \citep{2002MNRAS.329..897H}. \label{tbl:table:pop-synth}}

\begin{tabular}{ |c|c|c| } 
 \hline
 Code name & Reference & Publicly available  \\ 
 \hline
Binary\_c & \citet{2004PhDT........45I,2006AA...460..565I,2009AA...508.1359I}  & No  \\
%  Binary$_$C & \citet{2004PhDT........45I,2006A&A...460..565I,2009A&A...508.1359I} & No \\ 
 BSE & \citet{2002MNRAS.329..897H} & Yes  \\ 
 %BPASS\footnote{https://bpass.auckland.ac.nz/} & \citet{2018MNRAS.479...75S}  & No &  \\ 
 BPASS & \citet{2018MNRAS.479...75S}  & No \\
 ComBinE & \citet{2018MNRAS.481.1908K} & No \\
% COMPAS\footnote{https://compas.science/} & \citet{2017NatCo...814906S,2018MNRAS.481.4009V} & Yes & \\  % one ref. per code
%  COMPAS\footnote{https://compas.science/} & \citet{2017NatCo...814906S} & Yes & \\ 
 COMPAS & \citet{2017NatCo...814906S} & Yes  \\
%  COSMIC\footnote{https://cosmic-popsynth.github.io/docs/stable/index.html} & \citet{2020ApJ...898...71B} & Yes & \\ 
  COSMIC & \citet{2020ApJ...898...71B} & Yes  \\ 
 %MESA\footnote{http://mesa.sourceforge.net/} & \citet{2011ApJS..192....3P} & No & \\ 
 MOBSE & \citet{2018MNRAS.474.2959G} & No  \\ 
 POSYDON & \citet{2020arXiv201016333B, 2020arXiv201202274R} & No \\
Scenario Machine & \citet{1996smbs.book.....L,2009ARep...53..915L} & No \\
 SEVN & \citet{2015MNRAS.451.4086S} & Yes  \\ 
% SeBa\footnote{https://github.com/amusecode/SeBa} & \citet{1996A&A...309..179, 2012A&A...546A..70T} & Yes & \\
SeBa & \citet{1996AA...309..179P,2012AA...546A..70T} & Yes  \\
 
 StarTrack & \citet{2008ApJS..174..223B} & No   \\ 
TRES & \citet{2016ComAC...3....6T} & Yes   \\  
 \hline
\end{tabular}
\label{table:pop-synth}
\end{table}


\paragraph{Modelling binary evolution in dense environments}

\phantom{text}


Stellar-origin LISA GW sources can also be formed in dense stellar environments through dynamical interactions. Hence simulation codes that follow the evolution of dense stellar systems, either by direct integration or using Monte-Carlo techniques, are crucial for their study. Many of these codes follow simultaneously the evolution of single and binary stars within the dense stellar system, using one of the tools described in the previous Section. A list of stellar dynamics codes currently used in the community for the study of the formation of stellar-origin LISA GW sources can be fount in Table~\ref{table:dynamics-codes}.

\begin{table}
\caption{N-body and few-body dynamics codes used by the community at the time of writing. }

\begin{tabular}{ |c|p{4.5cm}|c| } 
 \hline
 Code name & Reference & Publicly available  \\ 
 \hline
NBODY6/NBODY6++GPU/NBODY7 & \citet{2012MNRAS.422..841A, 2012MNRAS.424..545N, 2015MNRAS.450.4070W}  & Yes  \\
phiGRAPE/phiGPU & \citet{2013hpc..conf...52B, 2011hpc..conf....8B} & No \\
HiGPU & \citet{2013JCoPh.236..580C} & No \\
CMC & \citet{2020ApJS..247...48K, 2019PhRvD..99f3003K, 2018PhRvL.120s1103K} & Yes \\
MOCCA & \citet{2013MNRAS.429.1221H, 2013MNRAS.431.2184G} & No\\
clusterBH & \citet{2020MNRAS.492.2936A} & No \\
 \hline
\end{tabular}
\label{table:dynamics-codes}
\end{table}

\paragraph{GW signal tools}

\phantom{text}


In order to calculate the GW signal of Galactic binary systems there are a number of approaches that can be used, ranging from detailed TDI based methods, e.g. via codes from the LISA Data Challenges (LDC, \url{https://lisa-ldc.lal.in2p3.fr}) to (more) analytic methods to calculate the signal and SNR of specific objects  \citep[e.g.][]{2003PhRvD..67j3001C,2019CQGra..36j5011R,2017MNRAS.470.1894K, 2018MNRAS.480..302K,2019PhRvD.100j4055S}. There are also some web-based tools to explore sensitivity of different GW detectors, including LISA and also detectability of sources in LISA, such as \url{https://gwplotter.com} \citep{2015CQGra..32a5014M} and the Gravitational Wave Universe Toolbox (\url{https://www.gw-universe.org}, \citealt{2021arXiv210613662Y})




